Replanning in Planar Pushing with Learned Dynamics: Frequency, Timing, and Search Effort

Choosing when to replan trades off access to new observations against search cost. We compare four signal-triggered rules on simulated planar pushing (PushT) using a curve of fixed periods and two controls: random replans matched to each rule's overall rate, and schedules shuffled across tasks to preserve the rule's replan frequency at each episode step. Across 10 state-input training seeds and 64 tasks, replanning every step succeeded on 33.7 tasks on average versus 16.8 for every four steps (difference +16.9, 95% interval +11.6 to +22.2). With the same nominal computation per step, eight search rounds every four steps reached 34.2 successes in a post hoc comparison with an interval for the difference that included zero; increasing candidates instead still favoured every-step replanning. At the prespecified settings, no rule showed a clear success advantage over its rate-matched control. Some rules did better at lower thresholds. Across the tested settings, no rule showed a clear success advantage over its schedule-shuffled control. The shuffled control itself outperformed the rate-matched control in 7 of 13 settings after correction. Under milder changes to simulator damping, every-step successes fell to 4.0-23.0 of 64 while the simulator-scored planner finished 44-56. The comparison separates replanning rate from the pairing of replanning times with individual tasks.

==> numbers.tex <==
% Generated by build_paper_assets.py from the result files. Do not edit by hand.
\makeatletter
\newcommand{\R}[1]{\@ifundefined{R@#1}{\textbf{??#1??}}{\csname R@#1\endcsname}}
\expandafter\def\csname R@checks\endcsname{66}
\expandafter\def\csname R@coast.0.0\endcsname{4.6}
\expandafter\def\csname R@coast.0.25\endcsname{86.3}
\expandafter\def\csname R@coast.0.85\endcsname{130.1}
\expandafter\def\csname R@commands\endcsname{47}
\expandafter\def\csname R@data.episodes\endcsname{6,000}
\expandafter\def\csname R@data.explore\endcsname{2,400}
\expandafter\def\csname R@data.transitions\endcsname{192,000}
\expandafter\def\csname R@dev0.fixed1.calls\endcsname{72,000}
\expandafter\def\csname R@dev0.fixed1.callsk\endcsname{72.0}
\expandafter\def\csname R@dev0.fixed1.cov\endcsname{0.81}
\expandafter\def\csname R@dev0.fixed1.exh\endcsname{0}
\expandafter\def\csname R@dev0.fixed1.n\endcsname{16}
\expandafter\def\csname R@dev0.fixed1.prog\endcsname{0.98}
\expandafter\def\csname R@dev0.fixed1.replans\endcsname{31.2}
\expandafter\def\csname R@dev0.fixed1.succ\endcsname{2}
\expandafter\def\csname R@dev0.fixed1.trig\endcsname{0}
\expandafter\def\csname R@dev0.fixed1.worse\endcsname{0}
\expandafter\def\csname R@dev0.fixed4.calls\endcsname{17,136}
\expandafter\def\csname R@dev0.fixed4.callsk\endcsname{17.1}
\expandafter\def\csname R@dev0.fixed4.cov\endcsname{0.83}
\expandafter\def\csname R@dev0.fixed4.exh\endcsname{0}
\expandafter\def\csname R@dev0.fixed4.n\endcsname{16}
\expandafter\def\csname R@dev0.fixed4.prog\endcsname{0.99}
\expandafter\def\csname R@dev0.fixed4.replans\endcsname{7.4}
\expandafter\def\csname R@dev0.fixed4.succ\endcsname{4}
\expandafter\def\csname R@dev0.fixed4.trig\endcsname{0}
\expandafter\def\csname R@dev0.fixed4.worse\endcsname{0}
\expandafter\def\csname R@dev1.fixed1.calls\endcsname{68,256}
\expandafter\def\csname R@dev1.fixed1.callsk\endcsname{68.3}
\expandafter\def\csname R@dev1.fixed1.cov\endcsname{0.88}
\expandafter\def\csname R@dev1.fixed1.exh\endcsname{0}
\expandafter\def\csname R@dev1.fixed1.n\endcsname{16}
\expandafter\def\csname R@dev1.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@dev1.fixed1.replans\endcsname{29.6}
\expandafter\def\csname R@dev1.fixed1.succ\endcsname{3}
\expandafter\def\csname R@dev1.fixed1.trig\endcsname{0}
\expandafter\def\csname R@dev1.fixed1.worse\endcsname{0}
\expandafter\def\csname R@dev1.fixed4.calls\endcsname{20,736}
\expandafter\def\csname R@dev1.fixed4.callsk\endcsname{20.7}
\expandafter\def\csname R@dev1.fixed4.cov\endcsname{0.85}
\expandafter\def\csname R@dev1.fixed4.exh\endcsname{0}
\expandafter\def\csname R@dev1.fixed4.n\endcsname{16}
\expandafter\def\csname R@dev1.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@dev1.fixed4.replans\endcsname{9.0}
\expandafter\def\csname R@dev1.fixed4.succ\endcsname{0}
\expandafter\def\csname R@dev1.fixed4.trig\endcsname{0}
\expandafter\def\csname R@dev1.fixed4.worse\endcsname{0}
\expandafter\def\csname R@dev2.fixed1.calls\endcsname{63,216}
\expandafter\def\csname R@dev2.fixed1.callsk\endcsname{63.2}
\expandafter\def\csname R@dev2.fixed1.cov\endcsname{0.90}
\expandafter\def\csname R@dev2.fixed1.exh\endcsname{0}
\expandafter\def\csname R@dev2.fixed1.n\endcsname{16}
\expandafter\def\csname R@dev2.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@dev2.fixed1.replans\endcsname{27.4}
\expandafter\def\csname R@dev2.fixed1.succ\endcsname{5}
\expandafter\def\csname R@dev2.fixed1.trig\endcsname{0}
\expandafter\def\csname R@dev2.fixed1.worse\endcsname{0}
\expandafter\def\csname R@dev2.fixed4.calls\endcsname{18,144}
\expandafter\def\csname R@dev2.fixed4.callsk\endcsname{18.1}
\expandafter\def\csname R@dev2.fixed4.cov\endcsname{0.85}
\expandafter\def\csname R@dev2.fixed4.exh\endcsname{0}
\expandafter\def\csname R@dev2.fixed4.n\endcsname{16}
\expandafter\def\csname R@dev2.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@dev2.fixed4.replans\endcsname{7.9}
\expandafter\def\csname R@dev2.fixed4.succ\endcsname{4}
\expandafter\def\csname R@dev2.fixed4.trig\endcsname{0}
\expandafter\def\csname R@dev2.fixed4.worse\endcsname{0}
\expandafter\def\csname R@dev3.fixed1.calls\endcsname{51,840}
\expandafter\def\csname R@dev3.fixed1.callsk\endcsname{51.8}
\expandafter\def\csname R@dev3.fixed1.cov\endcsname{0.90}
\expandafter\def\csname R@dev3.fixed1.exh\endcsname{0}
\expandafter\def\csname R@dev3.fixed1.n\endcsname{16}
\expandafter\def\csname R@dev3.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@dev3.fixed1.replans\endcsname{22.5}
\expandafter\def\csname R@dev3.fixed1.succ\endcsname{7}
\expandafter\def\csname R@dev3.fixed1.trig\endcsname{0}
\expandafter\def\csname R@dev3.fixed1.worse\endcsname{0}
\expandafter\def\csname R@dev3.fixed2.calls\endcsname{28,656}
\expandafter\def\csname R@dev3.fixed2.callsk\endcsname{28.7}
\expandafter\def\csname R@dev3.fixed2.cov\endcsname{0.91}
\expandafter\def\csname R@dev3.fixed2.exh\endcsname{0}
\expandafter\def\csname R@dev3.fixed2.n\endcsname{16}
\expandafter\def\csname R@dev3.fixed2.prog\endcsname{1.00}
\expandafter\def\csname R@dev3.fixed2.replans\endcsname{12.4}
\expandafter\def\csname R@dev3.fixed2.succ\endcsname{7}
\expandafter\def\csname R@dev3.fixed2.trig\endcsname{0}
\expandafter\def\csname R@dev3.fixed2.worse\endcsname{0}
\expandafter\def\csname R@dev3.fixed3.calls\endcsname{19,728}
\expandafter\def\csname R@dev3.fixed3.callsk\endcsname{19.7}
\expandafter\def\csname R@dev3.fixed3.cov\endcsname{0.88}
\expandafter\def\csname R@dev3.fixed3.exh\endcsname{0}
\expandafter\def\csname R@dev3.fixed3.n\endcsname{16}
\expandafter\def\csname R@dev3.fixed3.prog\endcsname{1.00}
\expandafter\def\csname R@dev3.fixed3.replans\endcsname{8.6}
\expandafter\def\csname R@dev3.fixed3.succ\endcsname{6}
\expandafter\def\csname R@dev3.fixed3.trig\endcsname{0}
\expandafter\def\csname R@dev3.fixed3.worse\endcsname{0}
\expandafter\def\csname R@dev3.fixed4.calls\endcsname{16,128}
\expandafter\def\csname R@dev3.fixed4.callsk\endcsname{16.1}
\expandafter\def\csname R@dev3.fixed4.cov\endcsname{0.88}
\expandafter\def\csname R@dev3.fixed4.exh\endcsname{0}
\expandafter\def\csname R@dev3.fixed4.n\endcsname{16}
\expandafter\def\csname R@dev3.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@dev3.fixed4.replans\endcsname{7.0}
\expandafter\def\csname R@dev3.fixed4.succ\endcsname{5}
\expandafter\def\csname R@dev3.fixed4.trig\endcsname{0}
\expandafter\def\csname R@dev3.fixed4.worse\endcsname{0}
\expandafter\def\csname R@dev3.fixed6.calls\endcsname{11,232}
\expandafter\def\csname R@dev3.fixed6.callsk\endcsname{11.2}
\expandafter\def\csname R@dev3.fixed6.cov\endcsname{0.88}
\expandafter\def\csname R@dev3.fixed6.exh\endcsname{0}
\expandafter\def\csname R@dev3.fixed6.n\endcsname{16}
\expandafter\def\csname R@dev3.fixed6.prog\endcsname{1.00}
\expandafter\def\csname R@dev3.fixed6.replans\endcsname{4.9}
\expandafter\def\csname R@dev3.fixed6.succ\endcsname{4}
\expandafter\def\csname R@dev3.fixed6.trig\endcsname{0}
\expandafter\def\csname R@dev3.fixed6.worse\endcsname{0}
\expandafter\def\csname R@mix.d0eps\endcsname{793}
\expandafter\def\csname R@mix.fixed1.calls\endcsname{80,640}
\expandafter\def\csname R@mix.fixed1.callsk\endcsname{80.6}
\expandafter\def\csname R@mix.fixed1.cov\endcsname{0.44}
\expandafter\def\csname R@mix.fixed1.exh\endcsname{0}
\expandafter\def\csname R@mix.fixed1.n\endcsname{16}
\expandafter\def\csname R@mix.fixed1.prog\endcsname{0.91}
\expandafter\def\csname R@mix.fixed1.replans\endcsname{35.0}
\expandafter\def\csname R@mix.fixed1.succ\endcsname{0}
\expandafter\def\csname R@mix.fixed1.trig\endcsname{0}
\expandafter\def\csname R@mix.fixed1.worse\endcsname{0}
\expandafter\def\csname R@mix.fixed4.calls\endcsname{20,736}
\expandafter\def\csname R@mix.fixed4.callsk\endcsname{20.7}
\expandafter\def\csname R@mix.fixed4.cov\endcsname{0.37}
\expandafter\def\csname R@mix.fixed4.exh\endcsname{0}
\expandafter\def\csname R@mix.fixed4.n\endcsname{16}
\expandafter\def\csname R@mix.fixed4.prog\endcsname{0.85}
\expandafter\def\csname R@mix.fixed4.replans\endcsname{9.0}
\expandafter\def\csname R@mix.fixed4.succ\endcsname{0}
\expandafter\def\csname R@mix.fixed4.trig\endcsname{0}
\expandafter\def\csname R@mix.fixed4.worse\endcsname{0}
\expandafter\def\csname R@n01.p0.contact.fixed4\endcsname{10}
\expandafter\def\csname R@n01.p0.contact.random\endcsname{9}
\expandafter\def\csname R@n01.p0.error.fixed4\endcsname{9}
\expandafter\def\csname R@n01.p0.fixed1.fixed4\endcsname{7}
\expandafter\def\csname R@n01.p0.geom.fixed4\endcsname{7}
\expandafter\def\csname R@n01.p0b.contact.fixed4\endcsname{10}
\expandafter\def\csname R@n01.p0b.contact.random\endcsname{8}
\expandafter\def\csname R@n01.p0b.error.fixed4\endcsname{9}
\expandafter\def\csname R@n01.p0b.fixed1.fixed4\endcsname{6}
\expandafter\def\csname R@n01.p0b.geom.fixed4\endcsname{7}
\expandafter\def\csname R@n01.s0.contact.fixed4\endcsname{10}
\expandafter\def\csname R@n01.s0.contact.random\endcsname{15}
\expandafter\def\csname R@n01.s0.error.fixed4\endcsname{10}
\expandafter\def\csname R@n01.s0.fixed1.fixed4\endcsname{3}
\expandafter\def\csname R@n01.s0.geom.fixed4\endcsname{9}
\expandafter\def\csname R@n01.s0b.contact.fixed4\endcsname{10}
\expandafter\def\csname R@n01.s0b.contact.random\endcsname{14}
\expandafter\def\csname R@n01.s0b.error.fixed4\endcsname{10}
\expandafter\def\csname R@n01.s0b.fixed1.fixed4\endcsname{4}
\expandafter\def\csname R@n01.s0b.geom.fixed4\endcsname{9}
\expandafter\def\csname R@n10.p0.contact.fixed4\endcsname{4}
\expandafter\def\csname R@n10.p0.contact.random\endcsname{3}
\expandafter\def\csname R@n10.p0.error.fixed4\endcsname{6}
\expandafter\def\csname R@n10.p0.fixed1.fixed4\endcsname{16}
\expandafter\def\csname R@n10.p0.geom.fixed4\endcsname{9}
\expandafter\def\csname R@n10.p0b.contact.fixed4\endcsname{4}
\expandafter\def\csname R@n10.p0b.contact.random\endcsname{3}
\expandafter\def\csname R@n10.p0b.error.fixed4\endcsname{6}
\expandafter\def\csname R@n10.p0b.fixed1.fixed4\endcsname{15}
\expandafter\def\csname R@n10.p0b.geom.fixed4\endcsname{9}
\expandafter\def\csname R@n10.s0.contact.fixed4\endcsname{11}
\expandafter\def\csname R@n10.s0.contact.random\endcsname{5}
\expandafter\def\csname R@n10.s0.error.fixed4\endcsname{12}
\expandafter\def\csname R@n10.s0.fixed1.fixed4\endcsname{22}
\expandafter\def\csname R@n10.s0.geom.fixed4\endcsname{11}
\expandafter\def\csname R@n10.s0b.contact.fixed4\endcsname{10}
\expandafter\def\csname R@n10.s0b.contact.random\endcsname{4}
\expandafter\def\csname R@n10.s0b.error.fixed4\endcsname{12}
\expandafter\def\csname R@n10.s0b.fixed1.fixed4\endcsname{16}
\expandafter\def\csname R@n10.s0b.geom.fixed4\endcsname{11}
\expandafter\def\csname R@or0.fixed1.calls\endcsname{14,016}
\expandafter\def\csname R@or0.fixed1.callsk\endcsname{14.0}
\expandafter\def\csname R@or0.fixed1.cov\endcsname{0.96}
\expandafter\def\csname R@or0.fixed1.exh\endcsname{0}
\expandafter\def\csname R@or0.fixed1.n\endcsname{8}
\expandafter\def\csname R@or0.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@or0.fixed1.replans\endcsname{18.2}
\expandafter\def\csname R@or0.fixed1.succ\endcsname{6}
\expandafter\def\csname R@or0.fixed1.trig\endcsname{0}
\expandafter\def\csname R@or0.fixed1.worse\endcsname{0}
\expandafter\def\csname R@or25.fixed1.calls\endcsname{24,480}
\expandafter\def\csname R@or25.fixed1.callsk\endcsname{24.5}
\expandafter\def\csname R@or25.fixed1.cov\endcsname{0.87}
\expandafter\def\csname R@or25.fixed1.exh\endcsname{0}
\expandafter\def\csname R@or25.fixed1.n\endcsname{8}
\expandafter\def\csname R@or25.fixed1.prog\endcsname{0.99}
\expandafter\def\csname R@or25.fixed1.replans\endcsname{31.9}
\expandafter\def\csname R@or25.fixed1.succ\endcsname{1}
\expandafter\def\csname R@or25.fixed1.trig\endcsname{0}
\expandafter\def\csname R@or25.fixed1.worse\endcsname{0}
\expandafter\def\csname R@p.p0.contact.fixed4\endcsname{0.180}
\expandafter\def\csname R@p.p0.contact.random\endcsname{0.146}
\expandafter\def\csname R@p.p0.error.fixed4\endcsname{0.607}
\expandafter\def\csname R@p.p0.fixed1.fixed4\endcsname{0.093}
\expandafter\def\csname R@p.p0.geom.fixed4\endcsname{0.804}
\expandafter\def\csname R@p.p0b.contact.fixed4\endcsname{0.180}
\expandafter\def\csname R@p.p0b.contact.random\endcsname{0.227}
\expandafter\def\csname R@p.p0b.error.fixed4\endcsname{0.607}
\expandafter\def\csname R@p.p0b.fixed1.fixed4\endcsname{0.078}
\expandafter\def\csname R@p.p0b.geom.fixed4\endcsname{0.804}
\expandafter\def\csname R@p.s0.contact.fixed4\endcsname{1.000}
\expandafter\def\csname R@p.s0.contact.random\endcsname{0.041}
\expandafter\def\csname R@p.s0.error.fixed4\endcsname{0.832}
\expandafter\def\csname R@p.s0.fixed1.fixed4\endcsname{0.0002}
\expandafter\def\csname R@p.s0.geom.fixed4\endcsname{0.824}
\expandafter\def\csname R@p.s0b.contact.fixed4\endcsname{1.000}
\expandafter\def\csname R@p.s0b.contact.random\endcsname{0.031}
\expandafter\def\csname R@p.s0b.error.fixed4\endcsname{0.832}
\expandafter\def\csname R@p.s0b.fixed1.fixed4\endcsname{0.012}
\expandafter\def\csname R@p.s0b.geom.fixed4\endcsname{0.824}
\expandafter\def\csname R@p0.contact.calls\endcsname{25,380}
\expandafter\def\csname R@p0.contact.callsk\endcsname{25.4}
\expandafter\def\csname R@p0.contact.cov\endcsname{0.89}
\expandafter\def\csname R@p0.contact.exh\endcsname{0}
\expandafter\def\csname R@p0.contact.n\endcsname{64}
\expandafter\def\csname R@p0.contact.prog\endcsname{1.00}
\expandafter\def\csname R@p0.contact.replans\endcsname{11.0}
\expandafter\def\csname R@p0.contact.rps\endcsname{0.34}
\expandafter\def\csname R@p0.contact.steps\endcsname{32.1}
\expandafter\def\csname R@p0.contact.succ\endcsname{8}
\expandafter\def\csname R@p0.contact.trig\endcsname{24}
\expandafter\def\csname R@p0.contact.worse\endcsname{0}
\expandafter\def\csname R@p0.disagreement.calls\endcsname{18,036}
\expandafter\def\csname R@p0.disagreement.callsk\endcsname{18.0}
\expandafter\def\csname R@p0.disagreement.cov\endcsname{0.88}
\expandafter\def\csname R@p0.disagreement.exh\endcsname{0}
\expandafter\def\csname R@p0.disagreement.n\endcsname{64}
\expandafter\def\csname R@p0.disagreement.prog\endcsname{1.00}
\expandafter\def\csname R@p0.disagreement.replans\endcsname{7.8}
\expandafter\def\csname R@p0.disagreement.rps\endcsname{0.25}
\expandafter\def\csname R@p0.disagreement.steps\endcsname{30.9}
\expandafter\def\csname R@p0.disagreement.succ\endcsname{10}
\expandafter\def\csname R@p0.disagreement.trig\endcsname{13}
\expandafter\def\csname R@p0.disagreement.worse\endcsname{0}
\expandafter\def\csname R@p0.error.calls\endcsname{18,576}
\expandafter\def\csname R@p0.error.callsk\endcsname{18.6}
\expandafter\def\csname R@p0.error.cov\endcsname{0.89}
\expandafter\def\csname R@p0.error.exh\endcsname{0}
\expandafter\def\csname R@p0.error.n\endcsname{64}
\expandafter\def\csname R@p0.error.prog\endcsname{1.00}
\expandafter\def\csname R@p0.error.replans\endcsname{8.1}
\expandafter\def\csname R@p0.error.rps\endcsname{0.26}
\expandafter\def\csname R@p0.error.steps\endcsname{30.7}
\expandafter\def\csname R@p0.error.succ\endcsname{11}
\expandafter\def\csname R@p0.error.trig\endcsname{15}
\expandafter\def\csname R@p0.error.worse\endcsname{0}
\expandafter\def\csname R@p0.fixed1.calls\endcsname{58,824}
\expandafter\def\csname R@p0.fixed1.callsk\endcsname{58.8}
\expandafter\def\csname R@p0.fixed1.cov\endcsname{0.92}
\expandafter\def\csname R@p0.fixed1.exh\endcsname{0}
\expandafter\def\csname R@p0.fixed1.n\endcsname{64}
\expandafter\def\csname R@p0.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@p0.fixed1.replans\endcsname{25.5}
\expandafter\def\csname R@p0.fixed1.rps\endcsname{1.00}
\expandafter\def\csname R@p0.fixed1.steps\endcsname{25.5}
\expandafter\def\csname R@p0.fixed1.succ\endcsname{23}
\expandafter\def\csname R@p0.fixed1.trig\endcsname{0}
\expandafter\def\csname R@p0.fixed1.worse\endcsname{0}
\expandafter\def\csname R@p0.fixed2.calls\endcsname{33,300}
\expandafter\def\csname R@p0.fixed2.callsk\endcsname{33.3}
\expandafter\def\csname R@p0.fixed2.cov\endcsname{0.90}
\expandafter\def\csname R@p0.fixed2.exh\endcsname{0}
\expandafter\def\csname R@p0.fixed2.n\endcsname{64}
\expandafter\def\csname R@p0.fixed2.prog\endcsname{1.00}
\expandafter\def\csname R@p0.fixed2.replans\endcsname{14.5}
\expandafter\def\csname R@p0.fixed2.rps\endcsname{0.52}
\expandafter\def\csname R@p0.fixed2.steps\endcsname{28.0}
\expandafter\def\csname R@p0.fixed2.succ\endcsname{18}
\expandafter\def\csname R@p0.fixed2.trig\endcsname{0}
\expandafter\def\csname R@p0.fixed2.worse\endcsname{0}
\expandafter\def\csname R@p0.fixed3.calls\endcsname{23,616}
\expandafter\def\csname R@p0.fixed3.callsk\endcsname{23.6}
\expandafter\def\csname R@p0.fixed3.cov\endcsname{0.89}
\expandafter\def\csname R@p0.fixed3.exh\endcsname{0}
\expandafter\def\csname R@p0.fixed3.n\endcsname{64}
\expandafter\def\csname R@p0.fixed3.prog\endcsname{1.00}
\expandafter\def\csname R@p0.fixed3.replans\endcsname{10.2}
\expandafter\def\csname R@p0.fixed3.rps\endcsname{0.34}
\expandafter\def\csname R@p0.fixed3.steps\endcsname{29.8}
\expandafter\def\csname R@p0.fixed3.succ\endcsname{14}
\expandafter\def\csname R@p0.fixed3.trig\endcsname{0}
\expandafter\def\csname R@p0.fixed3.worse\endcsname{0}
\expandafter\def\csname R@p0.fixed4.calls\endcsname{18,036}
\expandafter\def\csname R@p0.fixed4.callsk\endcsname{18.0}
\expandafter\def\csname R@p0.fixed4.cov\endcsname{0.88}
\expandafter\def\csname R@p0.fixed4.exh\endcsname{0}
\expandafter\def\csname R@p0.fixed4.n\endcsname{64}
\expandafter\def\csname R@p0.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@p0.fixed4.replans\endcsname{7.8}
\expandafter\def\csname R@p0.fixed4.rps\endcsname{0.26}
\expandafter\def\csname R@p0.fixed4.steps\endcsname{30.1}
\expandafter\def\csname R@p0.fixed4.succ\endcsname{14}
\expandafter\def\csname R@p0.fixed4.trig\endcsname{0}
\expandafter\def\csname R@p0.fixed4.worse\endcsname{0}
\expandafter\def\csname R@p0.fixed6.calls\endcsname{12,960}
\expandafter\def\csname R@p0.fixed6.callsk\endcsname{13.0}
\expandafter\def\csname R@p0.fixed6.cov\endcsname{0.87}
\expandafter\def\csname R@p0.fixed6.exh\endcsname{0}
\expandafter\def\csname R@p0.fixed6.n\endcsname{64}
\expandafter\def\csname R@p0.fixed6.prog\endcsname{1.00}
\expandafter\def\csname R@p0.fixed6.replans\endcsname{5.6}
\expandafter\def\csname R@p0.fixed6.rps\endcsname{0.17}
\expandafter\def\csname R@p0.fixed6.steps\endcsname{32.6}
\expandafter\def\csname R@p0.fixed6.succ\endcsname{7}
\expandafter\def\csname R@p0.fixed6.trig\endcsname{0}
\expandafter\def\csname R@p0.fixed6.worse\endcsname{0}
\expandafter\def\csname R@p0.geom.calls\endcsname{17,028}
\expandafter\def\csname R@p0.geom.callsk\endcsname{17.0}
\expandafter\def\csname R@p0.geom.cov\endcsname{0.90}
\expandafter\def\csname R@p0.geom.exh\endcsname{0}
\expandafter\def\csname R@p0.geom.n\endcsname{64}
\expandafter\def\csname R@p0.geom.prog\endcsname{1.00}
\expandafter\def\csname R@p0.geom.replans\endcsname{7.4}
\expandafter\def\csname R@p0.geom.rps\endcsname{0.26}
\expandafter\def\csname R@p0.geom.steps\endcsname{28.1}
\expandafter\def\csname R@p0.geom.succ\endcsname{16}
\expandafter\def\csname R@p0.geom.trig\endcsname{13}
\expandafter\def\csname R@p0.geom.worse\endcsname{0}
\expandafter\def\csname R@p0.random.calls\endcsname{21,384}
\expandafter\def\csname R@p0.random.callsk\endcsname{21.4}
\expandafter\def\csname R@p0.random.cov\endcsname{0.87}
\expandafter\def\csname R@p0.random.exh\endcsname{0}
\expandafter\def\csname R@p0.random.n\endcsname{64}
\expandafter\def\csname R@p0.random.prog\endcsname{1.00}
\expandafter\def\csname R@p0.random.replans\endcsname{9.3}
\expandafter\def\csname R@p0.random.rps\endcsname{0.31}
\expandafter\def\csname R@p0.random.steps\endcsname{29.7}
\expandafter\def\csname R@p0.random.succ\endcsname{14}
\expandafter\def\csname R@p0.random.trig\endcsname{24}
\expandafter\def\csname R@p0.random.worse\endcsname{0}
\expandafter\def\csname R@p0b.contact.calls\endcsname{20,592}
\expandafter\def\csname R@p0b.contact.callsk\endcsname{20.6}
\expandafter\def\csname R@p0b.contact.cov\endcsname{0.89}
\expandafter\def\csname R@p0b.contact.exh\endcsname{20}
\expandafter\def\csname R@p0b.contact.n\endcsname{64}
\expandafter\def\csname R@p0b.contact.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.contact.replans\endcsname{8.9}
\expandafter\def\csname R@p0b.contact.succ\endcsname{8}
\expandafter\def\csname R@p0b.contact.trig\endcsname{22}
\expandafter\def\csname R@p0b.contact.worse\endcsname{0}
\expandafter\def\csname R@p0b.disagreement.calls\endcsname{17,028}
\expandafter\def\csname R@p0b.disagreement.callsk\endcsname{17.0}
\expandafter\def\csname R@p0b.disagreement.cov\endcsname{0.88}
\expandafter\def\csname R@p0b.disagreement.exh\endcsname{8}
\expandafter\def\csname R@p0b.disagreement.n\endcsname{64}
\expandafter\def\csname R@p0b.disagreement.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.disagreement.replans\endcsname{7.4}
\expandafter\def\csname R@p0b.disagreement.succ\endcsname{10}
\expandafter\def\csname R@p0b.disagreement.trig\endcsname{13}
\expandafter\def\csname R@p0b.disagreement.worse\endcsname{0}
\expandafter\def\csname R@p0b.error.calls\endcsname{17,532}
\expandafter\def\csname R@p0b.error.callsk\endcsname{17.5}
\expandafter\def\csname R@p0b.error.cov\endcsname{0.89}
\expandafter\def\csname R@p0b.error.exh\endcsname{9}
\expandafter\def\csname R@p0b.error.n\endcsname{64}
\expandafter\def\csname R@p0b.error.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.error.replans\endcsname{7.6}
\expandafter\def\csname R@p0b.error.succ\endcsname{11}
\expandafter\def\csname R@p0b.error.trig\endcsname{15}
\expandafter\def\csname R@p0b.error.worse\endcsname{0}
\expandafter\def\csname R@p0b.fixed1.calls\endcsname{23,868}
\expandafter\def\csname R@p0b.fixed1.callsk\endcsname{23.9}
\expandafter\def\csname R@p0b.fixed1.cov\endcsname{0.92}
\expandafter\def\csname R@p0b.fixed1.exh\endcsname{41}
\expandafter\def\csname R@p0b.fixed1.n\endcsname{64}
\expandafter\def\csname R@p0b.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.fixed1.replans\endcsname{10.4}
\expandafter\def\csname R@p0b.fixed1.succ\endcsname{23}
\expandafter\def\csname R@p0b.fixed1.trig\endcsname{0}
\expandafter\def\csname R@p0b.fixed1.worse\endcsname{0}
\expandafter\def\csname R@p0b.fixed2.calls\endcsname{23,256}
\expandafter\def\csname R@p0b.fixed2.callsk\endcsname{23.3}
\expandafter\def\csname R@p0b.fixed2.cov\endcsname{0.90}
\expandafter\def\csname R@p0b.fixed2.exh\endcsname{47}
\expandafter\def\csname R@p0b.fixed2.n\endcsname{64}
\expandafter\def\csname R@p0b.fixed2.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.fixed2.replans\endcsname{10.1}
\expandafter\def\csname R@p0b.fixed2.succ\endcsname{17}
\expandafter\def\csname R@p0b.fixed2.trig\endcsname{0}
\expandafter\def\csname R@p0b.fixed2.worse\endcsname{0}
\expandafter\def\csname R@p0b.fixed3.calls\endcsname{23,616}
\expandafter\def\csname R@p0b.fixed3.callsk\endcsname{23.6}
\expandafter\def\csname R@p0b.fixed3.cov\endcsname{0.89}
\expandafter\def\csname R@p0b.fixed3.exh\endcsname{0}
\expandafter\def\csname R@p0b.fixed3.n\endcsname{64}
\expandafter\def\csname R@p0b.fixed3.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.fixed3.replans\endcsname{10.2}
\expandafter\def\csname R@p0b.fixed3.succ\endcsname{14}
\expandafter\def\csname R@p0b.fixed3.trig\endcsname{0}
\expandafter\def\csname R@p0b.fixed3.worse\endcsname{0}
\expandafter\def\csname R@p0b.fixed4.calls\endcsname{18,036}
\expandafter\def\csname R@p0b.fixed4.callsk\endcsname{18.0}
\expandafter\def\csname R@p0b.fixed4.cov\endcsname{0.88}
\expandafter\def\csname R@p0b.fixed4.exh\endcsname{0}
\expandafter\def\csname R@p0b.fixed4.n\endcsname{64}
\expandafter\def\csname R@p0b.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.fixed4.replans\endcsname{7.8}
\expandafter\def\csname R@p0b.fixed4.succ\endcsname{14}
\expandafter\def\csname R@p0b.fixed4.trig\endcsname{0}
\expandafter\def\csname R@p0b.fixed4.worse\endcsname{0}
\expandafter\def\csname R@p0b.fixed6.calls\endcsname{12,960}
\expandafter\def\csname R@p0b.fixed6.callsk\endcsname{13.0}
\expandafter\def\csname R@p0b.fixed6.cov\endcsname{0.87}
\expandafter\def\csname R@p0b.fixed6.exh\endcsname{0}
\expandafter\def\csname R@p0b.fixed6.n\endcsname{64}
\expandafter\def\csname R@p0b.fixed6.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.fixed6.replans\endcsname{5.6}
\expandafter\def\csname R@p0b.fixed6.succ\endcsname{7}
\expandafter\def\csname R@p0b.fixed6.trig\endcsname{0}
\expandafter\def\csname R@p0b.fixed6.worse\endcsname{0}
\expandafter\def\csname R@p0b.geom.calls\endcsname{16,920}
\expandafter\def\csname R@p0b.geom.callsk\endcsname{16.9}
\expandafter\def\csname R@p0b.geom.cov\endcsname{0.90}
\expandafter\def\csname R@p0b.geom.exh\endcsname{3}
\expandafter\def\csname R@p0b.geom.n\endcsname{64}
\expandafter\def\csname R@p0b.geom.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.geom.replans\endcsname{7.3}
\expandafter\def\csname R@p0b.geom.succ\endcsname{16}
\expandafter\def\csname R@p0b.geom.trig\endcsname{14}
\expandafter\def\csname R@p0b.geom.worse\endcsname{0}
\expandafter\def\csname R@p0b.random.calls\endcsname{20,808}
\expandafter\def\csname R@p0b.random.callsk\endcsname{20.8}
\expandafter\def\csname R@p0b.random.cov\endcsname{0.87}
\expandafter\def\csname R@p0b.random.exh\endcsname{8}
\expandafter\def\csname R@p0b.random.n\endcsname{64}
\expandafter\def\csname R@p0b.random.prog\endcsname{1.00}
\expandafter\def\csname R@p0b.random.replans\endcsname{9.0}
\expandafter\def\csname R@p0b.random.succ\endcsname{13}
\expandafter\def\csname R@p0b.random.trig\endcsname{24}
\expandafter\def\csname R@p0b.random.worse\endcsname{0}
\expandafter\def\csname R@p25.contact.calls\endcsname{25,560}
\expandafter\def\csname R@p25.contact.callsk\endcsname{25.6}
\expandafter\def\csname R@p25.contact.cov\endcsname{0.77}
\expandafter\def\csname R@p25.contact.exh\endcsname{0}
\expandafter\def\csname R@p25.contact.n\endcsname{64}
\expandafter\def\csname R@p25.contact.prog\endcsname{0.58}
\expandafter\def\csname R@p25.contact.replans\endcsname{11.1}
\expandafter\def\csname R@p25.contact.succ\endcsname{1}
\expandafter\def\csname R@p25.contact.trig\endcsname{21}
\expandafter\def\csname R@p25.contact.worse\endcsname{20}
\expandafter\def\csname R@p25.disagreement.calls\endcsname{41,292}
\expandafter\def\csname R@p25.disagreement.callsk\endcsname{41.3}
\expandafter\def\csname R@p25.disagreement.cov\endcsname{0.78}
\expandafter\def\csname R@p25.disagreement.exh\endcsname{0}
\expandafter\def\csname R@p25.disagreement.n\endcsname{64}
\expandafter\def\csname R@p25.disagreement.prog\endcsname{0.49}
\expandafter\def\csname R@p25.disagreement.replans\endcsname{17.9}
\expandafter\def\csname R@p25.disagreement.succ\endcsname{2}
\expandafter\def\csname R@p25.disagreement.trig\endcsname{49}
\expandafter\def\csname R@p25.disagreement.worse\endcsname{25}
\expandafter\def\csname R@p25.error.calls\endcsname{71,208}
\expandafter\def\csname R@p25.error.callsk\endcsname{71.2}
\expandafter\def\csname R@p25.error.cov\endcsname{0.75}
\expandafter\def\csname R@p25.error.exh\endcsname{0}
\expandafter\def\csname R@p25.error.n\endcsname{64}
\expandafter\def\csname R@p25.error.prog\endcsname{0.18}
\expandafter\def\csname R@p25.error.replans\endcsname{30.9}
\expandafter\def\csname R@p25.error.succ\endcsname{0}
\expandafter\def\csname R@p25.error.trig\endcsname{88}
\expandafter\def\csname R@p25.error.worse\endcsname{31}
\expandafter\def\csname R@p25.fixed1.calls\endcsname{79,560}
\expandafter\def\csname R@p25.fixed1.callsk\endcsname{79.6}
\expandafter\def\csname R@p25.fixed1.cov\endcsname{0.76}
\expandafter\def\csname R@p25.fixed1.exh\endcsname{0}
\expandafter\def\csname R@p25.fixed1.n\endcsname{64}
\expandafter\def\csname R@p25.fixed1.prog\endcsname{0.16}
\expandafter\def\csname R@p25.fixed1.replans\endcsname{34.5}
\expandafter\def\csname R@p25.fixed1.succ\endcsname{1}
\expandafter\def\csname R@p25.fixed1.trig\endcsname{0}
\expandafter\def\csname R@p25.fixed1.worse\endcsname{27}
\expandafter\def\csname R@p25.fixed2.calls\endcsname{40,968}
\expandafter\def\csname R@p25.fixed2.callsk\endcsname{41.0}
\expandafter\def\csname R@p25.fixed2.cov\endcsname{0.78}
\expandafter\def\csname R@p25.fixed2.exh\endcsname{0}
\expandafter\def\csname R@p25.fixed2.n\endcsname{64}
\expandafter\def\csname R@p25.fixed2.prog\endcsname{-0.73}
\expandafter\def\csname R@p25.fixed2.replans\endcsname{17.8}
\expandafter\def\csname R@p25.fixed2.succ\endcsname{1}
\expandafter\def\csname R@p25.fixed2.trig\endcsname{0}
\expandafter\def\csname R@p25.fixed2.worse\endcsname{35}
\expandafter\def\csname R@p25.fixed3.calls\endcsname{27,288}
\expandafter\def\csname R@p25.fixed3.callsk\endcsname{27.3}
\expandafter\def\csname R@p25.fixed3.cov\endcsname{0.77}
\expandafter\def\csname R@p25.fixed3.exh\endcsname{0}
\expandafter\def\csname R@p25.fixed3.n\endcsname{64}
\expandafter\def\csname R@p25.fixed3.prog\endcsname{0.10}
\expandafter\def\csname R@p25.fixed3.replans\endcsname{11.8}
\expandafter\def\csname R@p25.fixed3.succ\endcsname{1}
\expandafter\def\csname R@p25.fixed3.trig\endcsname{0}
\expandafter\def\csname R@p25.fixed3.worse\endcsname{31}
\expandafter\def\csname R@p25.fixed4.calls\endcsname{20,736}
\expandafter\def\csname R@p25.fixed4.callsk\endcsname{20.7}
\expandafter\def\csname R@p25.fixed4.cov\endcsname{0.77}
\expandafter\def\csname R@p25.fixed4.exh\endcsname{0}
\expandafter\def\csname R@p25.fixed4.n\endcsname{64}
\expandafter\def\csname R@p25.fixed4.prog\endcsname{0.53}
\expandafter\def\csname R@p25.fixed4.replans\endcsname{9.0}
\expandafter\def\csname R@p25.fixed4.succ\endcsname{0}
\expandafter\def\csname R@p25.fixed4.trig\endcsname{0}
\expandafter\def\csname R@p25.fixed4.worse\endcsname{22}
\expandafter\def\csname R@p25.fixed6.calls\endcsname{13,680}
\expandafter\def\csname R@p25.fixed6.callsk\endcsname{13.7}
\expandafter\def\csname R@p25.fixed6.cov\endcsname{0.77}
\expandafter\def\csname R@p25.fixed6.exh\endcsname{0}
\expandafter\def\csname R@p25.fixed6.n\endcsname{64}
\expandafter\def\csname R@p25.fixed6.prog\endcsname{0.33}
\expandafter\def\csname R@p25.fixed6.replans\endcsname{5.9}
\expandafter\def\csname R@p25.fixed6.succ\endcsname{1}
\expandafter\def\csname R@p25.fixed6.trig\endcsname{0}
\expandafter\def\csname R@p25.fixed6.worse\endcsname{24}
\expandafter\def\csname R@p25.geom.calls\endcsname{21,852}
\expandafter\def\csname R@p25.geom.callsk\endcsname{21.9}
\expandafter\def\csname R@p25.geom.cov\endcsname{0.76}
\expandafter\def\csname R@p25.geom.exh\endcsname{0}
\expandafter\def\csname R@p25.geom.n\endcsname{64}
\expandafter\def\csname R@p25.geom.prog\endcsname{0.47}
\expandafter\def\csname R@p25.geom.replans\endcsname{9.5}
\expandafter\def\csname R@p25.geom.succ\endcsname{0}
\expandafter\def\csname R@p25.geom.trig\endcsname{16}
\expandafter\def\csname R@p25.geom.worse\endcsname{22}
\expandafter\def\csname R@p25.random.calls\endcsname{24,840}
\expandafter\def\csname R@p25.random.callsk\endcsname{24.8}
\expandafter\def\csname R@p25.random.cov\endcsname{0.78}
\expandafter\def\csname R@p25.random.exh\endcsname{0}
\expandafter\def\csname R@p25.random.n\endcsname{64}
\expandafter\def\csname R@p25.random.prog\endcsname{0.45}
\expandafter\def\csname R@p25.random.replans\endcsname{10.8}
\expandafter\def\csname R@p25.random.succ\endcsname{1}
\expandafter\def\csname R@p25.random.trig\endcsname{24}
\expandafter\def\csname R@p25.random.worse\endcsname{26}
\expandafter\def\csname R@p85.contact.calls\endcsname{25,848}
\expandafter\def\csname R@p85.contact.callsk\endcsname{25.8}
\expandafter\def\csname R@p85.contact.cov\endcsname{0.78}
\expandafter\def\csname R@p85.contact.exh\endcsname{0}
\expandafter\def\csname R@p85.contact.n\endcsname{64}
\expandafter\def\csname R@p85.contact.prog\endcsname{-0.27}
\expandafter\def\csname R@p85.contact.replans\endcsname{11.2}
\expandafter\def\csname R@p85.contact.succ\endcsname{3}
\expandafter\def\csname R@p85.contact.trig\endcsname{23}
\expandafter\def\csname R@p85.contact.worse\endcsname{38}
\expandafter\def\csname R@p85.disagreement.calls\endcsname{50,760}
\expandafter\def\csname R@p85.disagreement.callsk\endcsname{50.8}
\expandafter\def\csname R@p85.disagreement.cov\endcsname{0.78}
\expandafter\def\csname R@p85.disagreement.exh\endcsname{0}
\expandafter\def\csname R@p85.disagreement.n\endcsname{64}
\expandafter\def\csname R@p85.disagreement.prog\endcsname{0.04}
\expandafter\def\csname R@p85.disagreement.replans\endcsname{22.0}
\expandafter\def\csname R@p85.disagreement.succ\endcsname{2}
\expandafter\def\csname R@p85.disagreement.trig\endcsname{62}
\expandafter\def\csname R@p85.disagreement.worse\endcsname{28}
\expandafter\def\csname R@p85.error.calls\endcsname{69,588}
\expandafter\def\csname R@p85.error.callsk\endcsname{69.6}
\expandafter\def\csname R@p85.error.cov\endcsname{0.79}
\expandafter\def\csname R@p85.error.exh\endcsname{0}
\expandafter\def\csname R@p85.error.n\endcsname{64}
\expandafter\def\csname R@p85.error.prog\endcsname{-0.15}
\expandafter\def\csname R@p85.error.replans\endcsname{30.2}
\expandafter\def\csname R@p85.error.succ\endcsname{4}
\expandafter\def\csname R@p85.error.trig\endcsname{90}
\expandafter\def\csname R@p85.error.worse\endcsname{33}
\expandafter\def\csname R@p85.fixed1.calls\endcsname{75,456}
\expandafter\def\csname R@p85.fixed1.callsk\endcsname{75.5}
\expandafter\def\csname R@p85.fixed1.cov\endcsname{0.77}
\expandafter\def\csname R@p85.fixed1.exh\endcsname{0}
\expandafter\def\csname R@p85.fixed1.n\endcsname{64}
\expandafter\def\csname R@p85.fixed1.prog\endcsname{0.08}
\expandafter\def\csname R@p85.fixed1.replans\endcsname{32.8}
\expandafter\def\csname R@p85.fixed1.succ\endcsname{5}
\expandafter\def\csname R@p85.fixed1.trig\endcsname{0}
\expandafter\def\csname R@p85.fixed1.worse\endcsname{30}
\expandafter\def\csname R@p85.fixed2.calls\endcsname{40,464}
\expandafter\def\csname R@p85.fixed2.callsk\endcsname{40.5}
\expandafter\def\csname R@p85.fixed2.cov\endcsname{0.78}
\expandafter\def\csname R@p85.fixed2.exh\endcsname{0}
\expandafter\def\csname R@p85.fixed2.n\endcsname{64}
\expandafter\def\csname R@p85.fixed2.prog\endcsname{-0.39}
\expandafter\def\csname R@p85.fixed2.replans\endcsname{17.6}
\expandafter\def\csname R@p85.fixed2.succ\endcsname{2}
\expandafter\def\csname R@p85.fixed2.trig\endcsname{0}
\expandafter\def\csname R@p85.fixed2.worse\endcsname{40}
\expandafter\def\csname R@p85.fixed3.calls\endcsname{26,352}
\expandafter\def\csname R@p85.fixed3.callsk\endcsname{26.4}
\expandafter\def\csname R@p85.fixed3.cov\endcsname{0.79}
\expandafter\def\csname R@p85.fixed3.exh\endcsname{0}
\expandafter\def\csname R@p85.fixed3.n\endcsname{64}
\expandafter\def\csname R@p85.fixed3.prog\endcsname{-0.15}
\expandafter\def\csname R@p85.fixed3.replans\endcsname{11.4}
\expandafter\def\csname R@p85.fixed3.succ\endcsname{4}
\expandafter\def\csname R@p85.fixed3.trig\endcsname{0}
\expandafter\def\csname R@p85.fixed3.worse\endcsname{34}
\expandafter\def\csname R@p85.fixed4.calls\endcsname{19,980}
\expandafter\def\csname R@p85.fixed4.callsk\endcsname{20.0}
\expandafter\def\csname R@p85.fixed4.cov\endcsname{0.78}
\expandafter\def\csname R@p85.fixed4.exh\endcsname{0}
\expandafter\def\csname R@p85.fixed4.n\endcsname{64}
\expandafter\def\csname R@p85.fixed4.prog\endcsname{0.02}
\expandafter\def\csname R@p85.fixed4.replans\endcsname{8.7}
\expandafter\def\csname R@p85.fixed4.succ\endcsname{3}
\expandafter\def\csname R@p85.fixed4.trig\endcsname{0}
\expandafter\def\csname R@p85.fixed4.worse\endcsname{31}
\expandafter\def\csname R@p85.fixed6.calls\endcsname{13,248}
\expandafter\def\csname R@p85.fixed6.callsk\endcsname{13.2}
\expandafter\def\csname R@p85.fixed6.cov\endcsname{0.78}
\expandafter\def\csname R@p85.fixed6.exh\endcsname{0}
\expandafter\def\csname R@p85.fixed6.n\endcsname{64}
\expandafter\def\csname R@p85.fixed6.prog\endcsname{-0.03}
\expandafter\def\csname R@p85.fixed6.replans\endcsname{5.8}
\expandafter\def\csname R@p85.fixed6.succ\endcsname{4}
\expandafter\def\csname R@p85.fixed6.trig\endcsname{0}
\expandafter\def\csname R@p85.fixed6.worse\endcsname{33}
\expandafter\def\csname R@p85.geom.calls\endcsname{24,048}
\expandafter\def\csname R@p85.geom.callsk\endcsname{24.0}
\expandafter\def\csname R@p85.geom.cov\endcsname{0.77}
\expandafter\def\csname R@p85.geom.exh\endcsname{0}
\expandafter\def\csname R@p85.geom.n\endcsname{64}
\expandafter\def\csname R@p85.geom.prog\endcsname{0.06}
\expandafter\def\csname R@p85.geom.replans\endcsname{10.4}
\expandafter\def\csname R@p85.geom.succ\endcsname{3}
\expandafter\def\csname R@p85.geom.trig\endcsname{21}
\expandafter\def\csname R@p85.geom.worse\endcsname{29}
\expandafter\def\csname R@p85.random.calls\endcsname{24,624}
\expandafter\def\csname R@p85.random.callsk\endcsname{24.6}
\expandafter\def\csname R@p85.random.cov\endcsname{0.77}
\expandafter\def\csname R@p85.random.exh\endcsname{0}
\expandafter\def\csname R@p85.random.n\endcsname{64}
\expandafter\def\csname R@p85.random.prog\endcsname{-0.08}
\expandafter\def\csname R@p85.random.replans\endcsname{10.7}
\expandafter\def\csname R@p85.random.succ\endcsname{2}
\expandafter\def\csname R@p85.random.trig\endcsname{24}
\expandafter\def\csname R@p85.random.worse\endcsname{37}
\expandafter\def\csname R@px.ang\endcsname{1.66}
\expandafter\def\csname R@px.auroc\endcsname{0.988}
\expandafter\def\csname R@px.base\endcsname{0.247}
\expandafter\def\csname R@px.brier\endcsname{0.042}
\expandafter\def\csname R@px.params\endcsname{150,022}
\expandafter\def\csname R@px.randrate\endcsname{24}
\expandafter\def\csname R@px.real.contact\endcsname{24}
\expandafter\def\csname R@px.real.disagreement\endcsname{13}
\expandafter\def\csname R@px.real.error\endcsname{14}
\expandafter\def\csname R@px.real.geom\endcsname{14}
\expandafter\def\csname R@px.rmse\endcsname{2.90}
\expandafter\def\csname R@px.testeps\endcsname{600}
\expandafter\def\csname R@px.testtrans\endcsname{19,200}
\expandafter\def\csname R@px.thr.contact\endcsname{0.0943}
\expandafter\def\csname R@px.thr.disagreement\endcsname{0.0013}
\expandafter\def\csname R@px.thr.error\endcsname{0.0042}
\expandafter\def\csname R@px.vis.ang\endcsname{1.58}
\expandafter\def\csname R@px.vis.rmse\endcsname{2.73}
\expandafter\def\csname R@px.visparams\endcsname{1,735,622}
\expandafter\def\csname R@ratio.fixed1.fixed4\endcsname{2.8}
\expandafter\def\csname R@ratio.random.fixed2\endcsname{80}
\expandafter\def\csname R@reach.r1\endcsname{64}
\expandafter\def\csname R@reach.r2\endcsname{231}
\expandafter\def\csname R@reach.r3\endcsname{340}
\expandafter\def\csname R@s0.contact.calls\endcsname{20,844}
\expandafter\def\csname R@s0.contact.callsk\endcsname{20.8}
\expandafter\def\csname R@s0.contact.cov\endcsname{0.92}
\expandafter\def\csname R@s0.contact.exh\endcsname{0}
\expandafter\def\csname R@s0.contact.n\endcsname{64}
\expandafter\def\csname R@s0.contact.prog\endcsname{1.00}
\expandafter\def\csname R@s0.contact.replans\endcsname{9.0}
\expandafter\def\csname R@s0.contact.rps\endcsname{0.33}
\expandafter\def\csname R@s0.contact.steps\endcsname{27.7}
\expandafter\def\csname R@s0.contact.succ\endcsname{20}
\expandafter\def\csname R@s0.contact.trig\endcsname{21}
\expandafter\def\csname R@s0.contact.worse\endcsname{0}
\expandafter\def\csname R@s0.disagreement.calls\endcsname{15,804}
\expandafter\def\csname R@s0.disagreement.callsk\endcsname{15.8}
\expandafter\def\csname R@s0.disagreement.cov\endcsname{0.91}
\expandafter\def\csname R@s0.disagreement.exh\endcsname{0}
\expandafter\def\csname R@s0.disagreement.n\endcsname{64}
\expandafter\def\csname R@s0.disagreement.prog\endcsname{1.00}
\expandafter\def\csname R@s0.disagreement.replans\endcsname{6.9}
\expandafter\def\csname R@s0.disagreement.rps\endcsname{0.25}
\expandafter\def\csname R@s0.disagreement.steps\endcsname{27.1}
\expandafter\def\csname R@s0.disagreement.succ\endcsname{20}
\expandafter\def\csname R@s0.disagreement.trig\endcsname{13}
\expandafter\def\csname R@s0.disagreement.worse\endcsname{0}
\expandafter\def\csname R@s0.error.calls\endcsname{15,624}
\expandafter\def\csname R@s0.error.callsk\endcsname{15.6}
\expandafter\def\csname R@s0.error.cov\endcsname{0.91}
\expandafter\def\csname R@s0.error.exh\endcsname{0}
\expandafter\def\csname R@s0.error.n\endcsname{64}
\expandafter\def\csname R@s0.error.prog\endcsname{1.00}
\expandafter\def\csname R@s0.error.replans\endcsname{6.8}
\expandafter\def\csname R@s0.error.rps\endcsname{0.25}
\expandafter\def\csname R@s0.error.steps\endcsname{27.2}
\expandafter\def\csname R@s0.error.succ\endcsname{21}
\expandafter\def\csname R@s0.error.trig\endcsname{12}
\expandafter\def\csname R@s0.error.worse\endcsname{0}
\expandafter\def\csname R@s0.fixed1.calls\endcsname{46,764}
\expandafter\def\csname R@s0.fixed1.callsk\endcsname{46.8}
\expandafter\def\csname R@s0.fixed1.cov\endcsname{0.94}
\expandafter\def\csname R@s0.fixed1.exh\endcsname{0}
\expandafter\def\csname R@s0.fixed1.n\endcsname{64}
\expandafter\def\csname R@s0.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@s0.fixed1.replans\endcsname{20.3}
\expandafter\def\csname R@s0.fixed1.rps\endcsname{1.00}
\expandafter\def\csname R@s0.fixed1.steps\endcsname{20.3}
\expandafter\def\csname R@s0.fixed1.succ\endcsname{38}
\expandafter\def\csname R@s0.fixed1.trig\endcsname{0}
\expandafter\def\csname R@s0.fixed1.worse\endcsname{0}
\expandafter\def\csname R@s0.fixed2.calls\endcsname{27,576}
\expandafter\def\csname R@s0.fixed2.callsk\endcsname{27.6}
\expandafter\def\csname R@s0.fixed2.cov\endcsname{0.92}
\expandafter\def\csname R@s0.fixed2.exh\endcsname{0}
\expandafter\def\csname R@s0.fixed2.n\endcsname{64}
\expandafter\def\csname R@s0.fixed2.prog\endcsname{1.00}
\expandafter\def\csname R@s0.fixed2.replans\endcsname{12.0}
\expandafter\def\csname R@s0.fixed2.rps\endcsname{0.52}
\expandafter\def\csname R@s0.fixed2.steps\endcsname{23.2}
\expandafter\def\csname R@s0.fixed2.succ\endcsname{30}
\expandafter\def\csname R@s0.fixed2.trig\endcsname{0}
\expandafter\def\csname R@s0.fixed2.worse\endcsname{0}
\expandafter\def\csname R@s0.fixed3.calls\endcsname{20,700}
\expandafter\def\csname R@s0.fixed3.callsk\endcsname{20.7}
\expandafter\def\csname R@s0.fixed3.cov\endcsname{0.90}
\expandafter\def\csname R@s0.fixed3.exh\endcsname{0}
\expandafter\def\csname R@s0.fixed3.n\endcsname{64}
\expandafter\def\csname R@s0.fixed3.prog\endcsname{1.00}
\expandafter\def\csname R@s0.fixed3.replans\endcsname{9.0}
\expandafter\def\csname R@s0.fixed3.rps\endcsname{0.35}
\expandafter\def\csname R@s0.fixed3.steps\endcsname{26.0}
\expandafter\def\csname R@s0.fixed3.succ\endcsname{22}
\expandafter\def\csname R@s0.fixed3.trig\endcsname{0}
\expandafter\def\csname R@s0.fixed3.worse\endcsname{0}
\expandafter\def\csname R@s0.fixed4.calls\endcsname{16,488}
\expandafter\def\csname R@s0.fixed4.callsk\endcsname{16.5}
\expandafter\def\csname R@s0.fixed4.cov\endcsname{0.90}
\expandafter\def\csname R@s0.fixed4.exh\endcsname{0}
\expandafter\def\csname R@s0.fixed4.n\endcsname{64}
\expandafter\def\csname R@s0.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@s0.fixed4.replans\endcsname{7.2}
\expandafter\def\csname R@s0.fixed4.rps\endcsname{0.26}
\expandafter\def\csname R@s0.fixed4.steps\endcsname{27.4}
\expandafter\def\csname R@s0.fixed4.succ\endcsname{19}
\expandafter\def\csname R@s0.fixed4.trig\endcsname{0}
\expandafter\def\csname R@s0.fixed4.worse\endcsname{0}
\expandafter\def\csname R@s0.fixed6.calls\endcsname{12,024}
\expandafter\def\csname R@s0.fixed6.callsk\endcsname{12.0}
\expandafter\def\csname R@s0.fixed6.cov\endcsname{0.88}
\expandafter\def\csname R@s0.fixed6.exh\endcsname{0}
\expandafter\def\csname R@s0.fixed6.n\endcsname{64}
\expandafter\def\csname R@s0.fixed6.prog\endcsname{1.00}
\expandafter\def\csname R@s0.fixed6.replans\endcsname{5.2}
\expandafter\def\csname R@s0.fixed6.rps\endcsname{0.17}
\expandafter\def\csname R@s0.fixed6.steps\endcsname{30.0}
\expandafter\def\csname R@s0.fixed6.succ\endcsname{12}
\expandafter\def\csname R@s0.fixed6.trig\endcsname{0}
\expandafter\def\csname R@s0.fixed6.worse\endcsname{0}
\expandafter\def\csname R@s0.geom.calls\endcsname{15,840}
\expandafter\def\csname R@s0.geom.callsk\endcsname{15.8}
\expandafter\def\csname R@s0.geom.cov\endcsname{0.92}
\expandafter\def\csname R@s0.geom.exh\endcsname{0}
\expandafter\def\csname R@s0.geom.n\endcsname{64}
\expandafter\def\csname R@s0.geom.prog\endcsname{1.00}
\expandafter\def\csname R@s0.geom.replans\endcsname{6.9}
\expandafter\def\csname R@s0.geom.rps\endcsname{0.25}
\expandafter\def\csname R@s0.geom.steps\endcsname{27.2}
\expandafter\def\csname R@s0.geom.succ\endcsname{21}
\expandafter\def\csname R@s0.geom.trig\endcsname{12}
\expandafter\def\csname R@s0.geom.worse\endcsname{0}
\expandafter\def\csname R@s0.minprog\endcsname{0.998}
\expandafter\def\csname R@s0.random.calls\endcsname{22,032}
\expandafter\def\csname R@s0.random.callsk\endcsname{22.0}
\expandafter\def\csname R@s0.random.cov\endcsname{0.92}
\expandafter\def\csname R@s0.random.exh\endcsname{0}
\expandafter\def\csname R@s0.random.n\endcsname{64}
\expandafter\def\csname R@s0.random.prog\endcsname{1.00}
\expandafter\def\csname R@s0.random.replans\endcsname{9.6}
\expandafter\def\csname R@s0.random.rps\endcsname{0.40}
\expandafter\def\csname R@s0.random.steps\endcsname{24.0}
\expandafter\def\csname R@s0.random.succ\endcsname{30}
\expandafter\def\csname R@s0.random.trig\endcsname{35}
\expandafter\def\csname R@s0.random.worse\endcsname{0}
\expandafter\def\csname R@s0b.contact.calls\endcsname{18,612}
\expandafter\def\csname R@s0b.contact.callsk\endcsname{18.6}
\expandafter\def\csname R@s0b.contact.cov\endcsname{0.91}
\expandafter\def\csname R@s0b.contact.exh\endcsname{9}
\expandafter\def\csname R@s0b.contact.n\endcsname{64}
\expandafter\def\csname R@s0b.contact.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.contact.replans\endcsname{8.1}
\expandafter\def\csname R@s0b.contact.succ\endcsname{19}
\expandafter\def\csname R@s0b.contact.trig\endcsname{20}
\expandafter\def\csname R@s0b.contact.worse\endcsname{0}
\expandafter\def\csname R@s0b.disagreement.calls\endcsname{15,264}
\expandafter\def\csname R@s0b.disagreement.callsk\endcsname{15.3}
\expandafter\def\csname R@s0b.disagreement.cov\endcsname{0.91}
\expandafter\def\csname R@s0b.disagreement.exh\endcsname{4}
\expandafter\def\csname R@s0b.disagreement.n\endcsname{64}
\expandafter\def\csname R@s0b.disagreement.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.disagreement.replans\endcsname{6.6}
\expandafter\def\csname R@s0b.disagreement.succ\endcsname{20}
\expandafter\def\csname R@s0b.disagreement.trig\endcsname{13}
\expandafter\def\csname R@s0b.disagreement.worse\endcsname{0}
\expandafter\def\csname R@s0b.error.calls\endcsname{15,372}
\expandafter\def\csname R@s0b.error.callsk\endcsname{15.4}
\expandafter\def\csname R@s0b.error.cov\endcsname{0.91}
\expandafter\def\csname R@s0b.error.exh\endcsname{3}
\expandafter\def\csname R@s0b.error.n\endcsname{64}
\expandafter\def\csname R@s0b.error.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.error.replans\endcsname{6.7}
\expandafter\def\csname R@s0b.error.succ\endcsname{21}
\expandafter\def\csname R@s0b.error.trig\endcsname{13}
\expandafter\def\csname R@s0b.error.worse\endcsname{0}
\expandafter\def\csname R@s0b.fixed1.calls\endcsname{22,032}
\expandafter\def\csname R@s0b.fixed1.callsk\endcsname{22.0}
\expandafter\def\csname R@s0b.fixed1.cov\endcsname{0.93}
\expandafter\def\csname R@s0b.fixed1.exh\endcsname{33}
\expandafter\def\csname R@s0b.fixed1.n\endcsname{64}
\expandafter\def\csname R@s0b.fixed1.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.fixed1.replans\endcsname{9.6}
\expandafter\def\csname R@s0b.fixed1.succ\endcsname{31}
\expandafter\def\csname R@s0b.fixed1.trig\endcsname{0}
\expandafter\def\csname R@s0b.fixed1.worse\endcsname{0}
\expandafter\def\csname R@s0b.fixed2.calls\endcsname{20,016}
\expandafter\def\csname R@s0b.fixed2.callsk\endcsname{20.0}
\expandafter\def\csname R@s0b.fixed2.cov\endcsname{0.92}
\expandafter\def\csname R@s0b.fixed2.exh\endcsname{35}
\expandafter\def\csname R@s0b.fixed2.n\endcsname{64}
\expandafter\def\csname R@s0b.fixed2.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.fixed2.replans\endcsname{8.7}
\expandafter\def\csname R@s0b.fixed2.succ\endcsname{29}
\expandafter\def\csname R@s0b.fixed2.trig\endcsname{0}
\expandafter\def\csname R@s0b.fixed2.worse\endcsname{0}
\expandafter\def\csname R@s0b.fixed3.calls\endcsname{20,700}
\expandafter\def\csname R@s0b.fixed3.callsk\endcsname{20.7}
\expandafter\def\csname R@s0b.fixed3.cov\endcsname{0.90}
\expandafter\def\csname R@s0b.fixed3.exh\endcsname{0}
\expandafter\def\csname R@s0b.fixed3.n\endcsname{64}
\expandafter\def\csname R@s0b.fixed3.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.fixed3.replans\endcsname{9.0}
\expandafter\def\csname R@s0b.fixed3.succ\endcsname{22}
\expandafter\def\csname R@s0b.fixed3.trig\endcsname{0}
\expandafter\def\csname R@s0b.fixed3.worse\endcsname{0}
\expandafter\def\csname R@s0b.fixed4.calls\endcsname{16,488}
\expandafter\def\csname R@s0b.fixed4.callsk\endcsname{16.5}
\expandafter\def\csname R@s0b.fixed4.cov\endcsname{0.90}
\expandafter\def\csname R@s0b.fixed4.exh\endcsname{0}
\expandafter\def\csname R@s0b.fixed4.n\endcsname{64}
\expandafter\def\csname R@s0b.fixed4.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.fixed4.replans\endcsname{7.2}
\expandafter\def\csname R@s0b.fixed4.succ\endcsname{19}
\expandafter\def\csname R@s0b.fixed4.trig\endcsname{0}
\expandafter\def\csname R@s0b.fixed4.worse\endcsname{0}
\expandafter\def\csname R@s0b.fixed6.calls\endcsname{12,024}
\expandafter\def\csname R@s0b.fixed6.callsk\endcsname{12.0}
\expandafter\def\csname R@s0b.fixed6.cov\endcsname{0.88}
\expandafter\def\csname R@s0b.fixed6.exh\endcsname{0}
\expandafter\def\csname R@s0b.fixed6.n\endcsname{64}
\expandafter\def\csname R@s0b.fixed6.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.fixed6.replans\endcsname{5.2}
\expandafter\def\csname R@s0b.fixed6.succ\endcsname{12}
\expandafter\def\csname R@s0b.fixed6.trig\endcsname{0}
\expandafter\def\csname R@s0b.fixed6.worse\endcsname{0}
\expandafter\def\csname R@s0b.geom.calls\endcsname{15,840}
\expandafter\def\csname R@s0b.geom.callsk\endcsname{15.8}
\expandafter\def\csname R@s0b.geom.cov\endcsname{0.92}
\expandafter\def\csname R@s0b.geom.exh\endcsname{0}
\expandafter\def\csname R@s0b.geom.n\endcsname{64}
\expandafter\def\csname R@s0b.geom.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.geom.replans\endcsname{6.9}
\expandafter\def\csname R@s0b.geom.succ\endcsname{21}
\expandafter\def\csname R@s0b.geom.trig\endcsname{12}
\expandafter\def\csname R@s0b.geom.worse\endcsname{0}
\expandafter\def\csname R@s0b.random.calls\endcsname{19,584}
\expandafter\def\csname R@s0b.random.callsk\endcsname{19.6}
\expandafter\def\csname R@s0b.random.cov\endcsname{0.92}
\expandafter\def\csname R@s0b.random.exh\endcsname{24}
\expandafter\def\csname R@s0b.random.n\endcsname{64}
\expandafter\def\csname R@s0b.random.prog\endcsname{1.00}
\expandafter\def\csname R@s0b.random.replans\endcsname{8.5}
\expandafter\def\csname R@s0b.random.succ\endcsname{29}
\expandafter\def\csname R@s0b.random.trig\endcsname{35}
\expandafter\def\csname R@s0b.random.worse\endcsname{0}
\expandafter\def\csname R@s25.contact.calls\endcsname{30,420}
\expandafter\def\csname R@s25.contact.callsk\endcsname{30.4}
\expandafter\def\csname R@s25.contact.cov\endcsname{0.78}
\expandafter\def\csname R@s25.contact.exh\endcsname{0}
\expandafter\def\csname R@s25.contact.n\endcsname{64}
\expandafter\def\csname R@s25.contact.prog\endcsname{-0.61}
\expandafter\def\csname R@s25.contact.replans\endcsname{13.2}
\expandafter\def\csname R@s25.contact.succ\endcsname{3}
\expandafter\def\csname R@s25.contact.trig\endcsname{31}
\expandafter\def\csname R@s25.contact.worse\endcsname{40}
\expandafter\def\csname R@s25.disagreement.calls\endcsname{50,400}
\expandafter\def\csname R@s25.disagreement.callsk\endcsname{50.4}
\expandafter\def\csname R@s25.disagreement.cov\endcsname{0.77}
\expandafter\def\csname R@s25.disagreement.exh\endcsname{0}
\expandafter\def\csname R@s25.disagreement.n\endcsname{64}
\expandafter\def\csname R@s25.disagreement.prog\endcsname{-0.40}
\expandafter\def\csname R@s25.disagreement.replans\endcsname{21.9}
\expandafter\def\csname R@s25.disagreement.succ\endcsname{2}
\expandafter\def\csname R@s25.disagreement.trig\endcsname{62}
\expandafter\def\csname R@s25.disagreement.worse\endcsname{40}
\expandafter\def\csname R@s25.error.calls\endcsname{68,544}
\expandafter\def\csname R@s25.error.callsk\endcsname{68.5}
\expandafter\def\csname R@s25.error.cov\endcsname{0.77}
\expandafter\def\csname R@s25.error.exh\endcsname{0}
\expandafter\def\csname R@s25.error.n\endcsname{64}
\expandafter\def\csname R@s25.error.prog\endcsname{-0.44}
\expandafter\def\csname R@s25.error.replans\endcsname{29.8}
\expandafter\def\csname R@s25.error.succ\endcsname{3}
\expandafter\def\csname R@s25.error.trig\endcsname{88}
\expandafter\def\csname R@s25.error.worse\endcsname{38}
\expandafter\def\csname R@s25.fixed1.calls\endcsname{79,488}
\expandafter\def\csname R@s25.fixed1.callsk\endcsname{79.5}
\expandafter\def\csname R@s25.fixed1.cov\endcsname{0.76}
\expandafter\def\csname R@s25.fixed1.exh\endcsname{0}
\expandafter\def\csname R@s25.fixed1.n\endcsname{64}
\expandafter\def\csname R@s25.fixed1.prog\endcsname{-0.44}
\expandafter\def\csname R@s25.fixed1.replans\endcsname{34.5}
\expandafter\def\csname R@s25.fixed1.succ\endcsname{1}
\expandafter\def\csname R@s25.fixed1.trig\endcsname{0}
\expandafter\def\csname R@s25.fixed1.worse\endcsname{39}
\expandafter\def\csname R@s25.fixed2.calls\endcsname{38,880}
\expandafter\def\csname R@s25.fixed2.callsk\endcsname{38.9}
\expandafter\def\csname R@s25.fixed2.cov\endcsname{0.77}
\expandafter\def\csname R@s25.fixed2.exh\endcsname{0}
\expandafter\def\csname R@s25.fixed2.n\endcsname{64}
\expandafter\def\csname R@s25.fixed2.prog\endcsname{-0.14}
\expandafter\def\csname R@s25.fixed2.replans\endcsname{16.9}
\expandafter\def\csname R@s25.fixed2.succ\endcsname{5}
\expandafter\def\csname R@s25.fixed2.trig\endcsname{0}
\expandafter\def\csname R@s25.fixed2.worse\endcsname{36}
\expandafter\def\csname R@s25.fixed3.calls\endcsname{27,252}
\expandafter\def\csname R@s25.fixed3.callsk\endcsname{27.3}
\expandafter\def\csname R@s25.fixed3.cov\endcsname{0.77}
\expandafter\def\csname R@s25.fixed3.exh\endcsname{0}
\expandafter\def\csname R@s25.fixed3.n\endcsname{64}
\expandafter\def\csname R@s25.fixed3.prog\endcsname{-0.19}
\expandafter\def\csname R@s25.fixed3.replans\endcsname{11.8}
\expandafter\def\csname R@s25.fixed3.succ\endcsname{1}
\expandafter\def\csname R@s25.fixed3.trig\endcsname{0}
\expandafter\def\csname R@s25.fixed3.worse\endcsname{36}
\expandafter\def\csname R@s25.fixed4.calls\endcsname{20,196}
\expandafter\def\csname R@s25.fixed4.callsk\endcsname{20.2}
\expandafter\def\csname R@s25.fixed4.cov\endcsname{0.77}
\expandafter\def\csname R@s25.fixed4.exh\endcsname{0}
\expandafter\def\csname R@s25.fixed4.n\endcsname{64}
\expandafter\def\csname R@s25.fixed4.prog\endcsname{-0.47}
\expandafter\def\csname R@s25.fixed4.replans\endcsname{8.8}
\expandafter\def\csname R@s25.fixed4.succ\endcsname{2}
\expandafter\def\csname R@s25.fixed4.trig\endcsname{0}
\expandafter\def\csname R@s25.fixed4.worse\endcsname{37}
\expandafter\def\csname R@s25.fixed6.calls\endcsname{13,212}
\expandafter\def\csname R@s25.fixed6.callsk\endcsname{13.2}
\expandafter\def\csname R@s25.fixed6.cov\endcsname{0.79}
\expandafter\def\csname R@s25.fixed6.exh\endcsname{0}
\expandafter\def\csname R@s25.fixed6.n\endcsname{64}
\expandafter\def\csname R@s25.fixed6.prog\endcsname{-1.11}
\expandafter\def\csname R@s25.fixed6.replans\endcsname{5.7}
\expandafter\def\csname R@s25.fixed6.succ\endcsname{4}
\expandafter\def\csname R@s25.fixed6.trig\endcsname{0}
\expandafter\def\csname R@s25.fixed6.worse\endcsname{43}
\expandafter\def\csname R@s25.geom.calls\endcsname{21,600}
\expandafter\def\csname R@s25.geom.callsk\endcsname{21.6}
\expandafter\def\csname R@s25.geom.cov\endcsname{0.77}
\expandafter\def\csname R@s25.geom.exh\endcsname{0}
\expandafter\def\csname R@s25.geom.n\endcsname{64}
\expandafter\def\csname R@s25.geom.prog\endcsname{-0.39}
\expandafter\def\csname R@s25.geom.replans\endcsname{9.4}
\expandafter\def\csname R@s25.geom.succ\endcsname{2}
\expandafter\def\csname R@s25.geom.trig\endcsname{15}
\expandafter\def\csname R@s25.geom.worse\endcsname{40}
\expandafter\def\csname R@s25.random.calls\endcsname{31,032}
\expandafter\def\csname R@s25.random.callsk\endcsname{31.0}
\expandafter\def\csname R@s25.random.cov\endcsname{0.77}
\expandafter\def\csname R@s25.random.exh\endcsname{0}
\expandafter\def\csname R@s25.random.n\endcsname{64}
\expandafter\def\csname R@s25.random.prog\endcsname{-0.73}
\expandafter\def\csname R@s25.random.replans\endcsname{13.5}
\expandafter\def\csname R@s25.random.succ\endcsname{2}
\expandafter\def\csname R@s25.random.trig\endcsname{35}
\expandafter\def\csname R@s25.random.worse\endcsname{46}
\expandafter\def\csname R@s85.contact.calls\endcsname{28,692}
\expandafter\def\csname R@s85.contact.callsk\endcsname{28.7}
\expandafter\def\csname R@s85.contact.cov\endcsname{0.80}
\expandafter\def\csname R@s85.contact.exh\endcsname{0}
\expandafter\def\csname R@s85.contact.n\endcsname{64}
\expandafter\def\csname R@s85.contact.prog\endcsname{0.12}
\expandafter\def\csname R@s85.contact.replans\endcsname{12.5}
\expandafter\def\csname R@s85.contact.succ\endcsname{6}
\expandafter\def\csname R@s85.contact.trig\endcsname{30}
\expandafter\def\csname R@s85.contact.worse\endcsname{29}
\expandafter\def\csname R@s85.disagreement.calls\endcsname{56,340}
\expandafter\def\csname R@s85.disagreement.callsk\endcsname{56.3}
\expandafter\def\csname R@s85.disagreement.cov\endcsname{0.81}
\expandafter\def\csname R@s85.disagreement.exh\endcsname{0}
\expandafter\def\csname R@s85.disagreement.n\endcsname{64}
\expandafter\def\csname R@s85.disagreement.prog\endcsname{-0.08}
\expandafter\def\csname R@s85.disagreement.replans\endcsname{24.5}
\expandafter\def\csname R@s85.disagreement.succ\endcsname{4}
\expandafter\def\csname R@s85.disagreement.trig\endcsname{72}
\expandafter\def\csname R@s85.disagreement.worse\endcsname{35}
\expandafter\def\csname R@s85.error.calls\endcsname{73,476}
\expandafter\def\csname R@s85.error.callsk\endcsname{73.5}
\expandafter\def\csname R@s85.error.cov\endcsname{0.80}
\expandafter\def\csname R@s85.error.exh\endcsname{0}
\expandafter\def\csname R@s85.error.n\endcsname{64}
\expandafter\def\csname R@s85.error.prog\endcsname{-0.37}
\expandafter\def\csname R@s85.error.replans\endcsname{31.9}
\expandafter\def\csname R@s85.error.succ\endcsname{3}
\expandafter\def\csname R@s85.error.trig\endcsname{95}
\expandafter\def\csname R@s85.error.worse\endcsname{42}
\expandafter\def\csname R@s85.fixed1.calls\endcsname{76,428}
\expandafter\def\csname R@s85.fixed1.callsk\endcsname{76.4}
\expandafter\def\csname R@s85.fixed1.cov\endcsname{0.79}
\expandafter\def\csname R@s85.fixed1.exh\endcsname{0}
\expandafter\def\csname R@s85.fixed1.n\endcsname{64}
\expandafter\def\csname R@s85.fixed1.prog\endcsname{-0.37}
\expandafter\def\csname R@s85.fixed1.replans\endcsname{33.2}
\expandafter\def\csname R@s85.fixed1.succ\endcsname{4}
\expandafter\def\csname R@s85.fixed1.trig\endcsname{0}
\expandafter\def\csname R@s85.fixed1.worse\endcsname{46}
\expandafter\def\csname R@s85.fixed2.calls\endcsname{38,520}
\expandafter\def\csname R@s85.fixed2.callsk\endcsname{38.5}
\expandafter\def\csname R@s85.fixed2.cov\endcsname{0.80}
\expandafter\def\csname R@s85.fixed2.exh\endcsname{0}
\expandafter\def\csname R@s85.fixed2.n\endcsname{64}
\expandafter\def\csname R@s85.fixed2.prog\endcsname{-0.71}
\expandafter\def\csname R@s85.fixed2.replans\endcsname{16.7}
\expandafter\def\csname R@s85.fixed2.succ\endcsname{6}
\expandafter\def\csname R@s85.fixed2.trig\endcsname{0}
\expandafter\def\csname R@s85.fixed2.worse\endcsname{40}
\expandafter\def\csname R@s85.fixed3.calls\endcsname{25,200}
\expandafter\def\csname R@s85.fixed3.callsk\endcsname{25.2}
\expandafter\def\csname R@s85.fixed3.cov\endcsname{0.79}
\expandafter\def\csname R@s85.fixed3.exh\endcsname{0}
\expandafter\def\csname R@s85.fixed3.n\endcsname{64}
\expandafter\def\csname R@s85.fixed3.prog\endcsname{-0.14}
\expandafter\def\csname R@s85.fixed3.replans\endcsname{10.9}
\expandafter\def\csname R@s85.fixed3.succ\endcsname{7}
\expandafter\def\csname R@s85.fixed3.trig\endcsname{0}
\expandafter\def\csname R@s85.fixed3.worse\endcsname{37}
\expandafter\def\csname R@s85.fixed4.calls\endcsname{19,440}
\expandafter\def\csname R@s85.fixed4.callsk\endcsname{19.4}
\expandafter\def\csname R@s85.fixed4.cov\endcsname{0.80}
\expandafter\def\csname R@s85.fixed4.exh\endcsname{0}
\expandafter\def\csname R@s85.fixed4.n\endcsname{64}
\expandafter\def\csname R@s85.fixed4.prog\endcsname{-0.08}
\expandafter\def\csname R@s85.fixed4.replans\endcsname{8.4}
\expandafter\def\csname R@s85.fixed4.succ\endcsname{5}
\expandafter\def\csname R@s85.fixed4.trig\endcsname{0}
\expandafter\def\csname R@s85.fixed4.worse\endcsname{37}
\expandafter\def\csname R@s85.fixed6.calls\endcsname{12,852}
\expandafter\def\csname R@s85.fixed6.callsk\endcsname{12.9}
\expandafter\def\csname R@s85.fixed6.cov\endcsname{0.80}
\expandafter\def\csname R@s85.fixed6.exh\endcsname{0}
\expandafter\def\csname R@s85.fixed6.n\endcsname{64}
\expandafter\def\csname R@s85.fixed6.prog\endcsname{-0.17}
\expandafter\def\csname R@s85.fixed6.replans\endcsname{5.6}
\expandafter\def\csname R@s85.fixed6.succ\endcsname{6}
\expandafter\def\csname R@s85.fixed6.trig\endcsname{0}
\expandafter\def\csname R@s85.fixed6.worse\endcsname{38}
\expandafter\def\csname R@s85.geom.calls\endcsname{20,016}
\expandafter\def\csname R@s85.geom.callsk\endcsname{20.0}
\expandafter\def\csname R@s85.geom.cov\endcsname{0.80}
\expandafter\def\csname R@s85.geom.exh\endcsname{0}
\expandafter\def\csname R@s85.geom.n\endcsname{64}
\expandafter\def\csname R@s85.geom.prog\endcsname{-0.13}
\expandafter\def\csname R@s85.geom.replans\endcsname{8.7}
\expandafter\def\csname R@s85.geom.succ\endcsname{5}
\expandafter\def\csname R@s85.geom.trig\endcsname{14}
\expandafter\def\csname R@s85.geom.worse\endcsname{39}
\expandafter\def\csname R@s85.random.calls\endcsname{29,160}
\expandafter\def\csname R@s85.random.callsk\endcsname{29.2}
\expandafter\def\csname R@s85.random.cov\endcsname{0.77}
\expandafter\def\csname R@s85.random.exh\endcsname{0}
\expandafter\def\csname R@s85.random.n\endcsname{64}
\expandafter\def\csname R@s85.random.prog\endcsname{-0.09}
\expandafter\def\csname R@s85.random.replans\endcsname{12.7}
\expandafter\def\csname R@s85.random.succ\endcsname{6}
\expandafter\def\csname R@s85.random.trig\endcsname{35}
\expandafter\def\csname R@s85.random.worse\endcsname{38}
\expandafter\def\csname R@shift.max\endcsname{7}
\expandafter\def\csname R@st.ang\endcsname{0.45}
\expandafter\def\csname R@st.auroc\endcsname{0.995}
\expandafter\def\csname R@st.base\endcsname{0.247}
\expandafter\def\csname R@st.brier\endcsname{0.027}
\expandafter\def\csname R@st.params\endcsname{150,022}
\expandafter\def\csname R@st.randrate\endcsname{36}
\expandafter\def\csname R@st.real.contact\endcsname{36}
\expandafter\def\csname R@st.real.disagreement\endcsname{13}
\expandafter\def\csname R@st.real.error\endcsname{12}
\expandafter\def\csname R@st.real.geom\endcsname{13}
\expandafter\def\csname R@st.rmse\endcsname{1.73}
\expandafter\def\csname R@st.testeps\endcsname{600}
\expandafter\def\csname R@st.testtrans\endcsname{19,200}
\expandafter\def\csname R@st.thr.contact\endcsname{0.0504}
\expandafter\def\csname R@st.thr.disagreement\endcsname{0.0008}
\expandafter\def\csname R@st.thr.error\endcsname{0.0008}
\expandafter\def\csname R@st.visparams\endcsname{0}
\expandafter\def\csname R@x.ci.p0.contact.fixed4\endcsname{$-13$ to $+1$}
\expandafter\def\csname R@x.ci.p0.contact.random\endcsname{$-13$ to $+0$}
\expandafter\def\csname R@x.ci.p0.error.fixed4\endcsname{$-11$ to $+4$}
\expandafter\def\csname R@x.ci.p0.fixed1.fixed4\endcsname{$+0$ to $+18$}
\expandafter\def\csname R@x.ci.p0.geom.fixed4\endcsname{$-6$ to $+10$}
\expandafter\def\csname R@x.ci.p0b.contact.fixed4\endcsname{$-13$ to $+1$}
\expandafter\def\csname R@x.ci.p0b.contact.random\endcsname{$-12$ to $+1$}
\expandafter\def\csname R@x.ci.p0b.error.fixed4\endcsname{$-11$ to $+5$}
\expandafter\def\csname R@x.ci.p0b.fixed1.fixed4\endcsname{$+0$ to $+18$}
\expandafter\def\csname R@x.ci.p0b.geom.fixed4\endcsname{$-6$ to $+10$}
\expandafter\def\csname R@x.ci.s0.contact.fixed4\endcsname{$-8$ to $+10$}
\expandafter\def\csname R@x.ci.s0.contact.random\endcsname{$-18$ to $-2$}
\expandafter\def\csname R@x.ci.s0.error.fixed4\endcsname{$-7$ to $+11$}
\expandafter\def\csname R@x.ci.s0.fixed1.fixed4\endcsname{$+10$ to $+28$}
\expandafter\def\csname R@x.ci.s0.geom.fixed4\endcsname{$-7$ to $+11$}
\expandafter\def\csname R@x.ci.s0.random.fixed2\endcsname{$-9$ to $+9$}
\expandafter\def\csname R@x.ci.s0.random.fixed3\endcsname{$-1$ to $+18$}
\expandafter\def\csname R@x.ci.s0b.contact.fixed4\endcsname{$-9$ to $+9$}
\expandafter\def\csname R@x.ci.s0b.contact.random\endcsname{$-18$ to $-2$}
\expandafter\def\csname R@x.ci.s0b.error.fixed4\endcsname{$-7$ to $+11$}
\expandafter\def\csname R@x.ci.s0b.fixed1.fixed3\endcsname{$+0$ to $+18$}
\expandafter\def\csname R@x.ci.s0b.fixed1.fixed4\endcsname{$+4$ to $+20$}
\expandafter\def\csname R@x.ci.s0b.fixed2.fixed3\endcsname{$+2$ to $+13$}
\expandafter\def\csname R@x.ci.s0b.geom.fixed4\endcsname{$-7$ to $+11$}
\expandafter\def\csname R@x.ci.s0b.random.fixed3\endcsname{$-2$ to $+16$}
\expandafter\def\csname R@x.contact.fire.changed\endcsname{59}
\expandafter\def\csname R@x.contact.fire.n\endcsname{305}
\expandafter\def\csname R@x.contact.quiet.changed\endcsname{2}
\expandafter\def\csname R@x.contact.quiet.n\endcsname{1152}
\expandafter\def\csname R@x.contact.score.above05\endcsname{9}
\expandafter\def\csname R@x.contact.score.below001\endcsname{76}
\expandafter\def\csname R@x.contact.score.q50\endcsname{0.0000}
\expandafter\def\csname R@x.contact.score.q75\endcsname{0.006}
\expandafter\def\csname R@x.contact.score.q90\endcsname{0.44}
\expandafter\def\csname R@x.cov.p0.contact.fixed4\endcsname{$+0.004$}
\expandafter\def\csname R@x.cov.p0.contact.random\endcsname{$+0.016$}
\expandafter\def\csname R@x.cov.p0.error.fixed4\endcsname{$+0.009$}
\expandafter\def\csname R@x.cov.p0.fixed1.fixed4\endcsname{$+0.036$}
\expandafter\def\csname R@x.cov.p0.geom.fixed4\endcsname{$+0.016$}
\expandafter\def\csname R@x.cov.p0b.contact.fixed4\endcsname{$+0.006$}
\expandafter\def\csname R@x.cov.p0b.contact.random\endcsname{$+0.017$}
\expandafter\def\csname R@x.cov.p0b.error.fixed4\endcsname{$+0.009$}
\expandafter\def\csname R@x.cov.p0b.fixed1.fixed4\endcsname{$+0.034$}
\expandafter\def\csname R@x.cov.p0b.geom.fixed4\endcsname{$+0.016$}
\expandafter\def\csname R@x.cov.s0.contact.fixed4\endcsname{$+0.019$}
\expandafter\def\csname R@x.cov.s0.contact.random\endcsname{$-0.004$}
\expandafter\def\csname R@x.cov.s0.error.fixed4\endcsname{$+0.014$}
\expandafter\def\csname R@x.cov.s0.fixed1.fixed4\endcsname{$+0.040$}
\expandafter\def\csname R@x.cov.s0.geom.fixed4\endcsname{$+0.019$}
\expandafter\def\csname R@x.cov.s0.random.fixed2\endcsname{$+0.000$}
\expandafter\def\csname R@x.cov.s0.random.fixed3\endcsname{$+0.022$}
\expandafter\def\csname R@x.cov.s0b.contact.fixed4\endcsname{$+0.018$}
\expandafter\def\csname R@x.cov.s0b.contact.random\endcsname{$-0.001$}
\expandafter\def\csname R@x.cov.s0b.error.fixed4\endcsname{$+0.014$}
\expandafter\def\csname R@x.cov.s0b.fixed1.fixed3\endcsname{$+0.032$}
\expandafter\def\csname R@x.cov.s0b.fixed1.fixed4\endcsname{$+0.033$}
\expandafter\def\csname R@x.cov.s0b.fixed2.fixed3\endcsname{$+0.021$}
\expandafter\def\csname R@x.cov.s0b.geom.fixed4\endcsname{$+0.019$}
\expandafter\def\csname R@x.cov.s0b.random.fixed3\endcsname{$+0.018$}
\expandafter\def\csname R@x.covci.p0.contact.fixed4\endcsname{$-0.011$ to $+0.020$}
\expandafter\def\csname R@x.covci.p0.contact.random\endcsname{$-0.002$ to $+0.034$}
\expandafter\def\csname R@x.covci.p0.error.fixed4\endcsname{$-0.008$ to $+0.033$}
\expandafter\def\csname R@x.covci.p0.fixed1.fixed4\endcsname{$+0.013$ to $+0.062$}
\expandafter\def\csname R@x.covci.p0.geom.fixed4\endcsname{$-0.004$ to $+0.041$}
\expandafter\def\csname R@x.covci.p0b.contact.fixed4\endcsname{$-0.010$ to $+0.022$}
\expandafter\def\csname R@x.covci.p0b.contact.random\endcsname{$-0.001$ to $+0.036$}
\expandafter\def\csname R@x.covci.p0b.error.fixed4\endcsname{$-0.008$ to $+0.032$}
\expandafter\def\csname R@x.covci.p0b.fixed1.fixed4\endcsname{$+0.011$ to $+0.061$}
\expandafter\def\csname R@x.covci.p0b.geom.fixed4\endcsname{$-0.004$ to $+0.041$}
\expandafter\def\csname R@x.covci.s0.contact.fixed4\endcsname{$-0.002$ to $+0.043$}
\expandafter\def\csname R@x.covci.s0.contact.random\endcsname{$-0.017$ to $+0.009$}
\expandafter\def\csname R@x.covci.s0.error.fixed4\endcsname{$-0.007$ to $+0.040$}
\expandafter\def\csname R@x.covci.s0.fixed1.fixed4\endcsname{$+0.021$ to $+0.065$}
\expandafter\def\csname R@x.covci.s0.geom.fixed4\endcsname{$-0.001$ to $+0.043$}
\expandafter\def\csname R@x.covci.s0.random.fixed2\endcsname{$-0.016$ to $+0.019$}
\expandafter\def\csname R@x.covci.s0.random.fixed3\endcsname{$+0.003$ to $+0.044$}
\expandafter\def\csname R@x.covci.s0b.contact.fixed4\endcsname{$-0.002$ to $+0.042$}
\expandafter\def\csname R@x.covci.s0b.contact.random\endcsname{$-0.013$ to $+0.013$}
\expandafter\def\csname R@x.covci.s0b.error.fixed4\endcsname{$-0.007$ to $+0.040$}
\expandafter\def\csname R@x.covci.s0b.fixed1.fixed3\endcsname{$+0.012$ to $+0.056$}
\expandafter\def\csname R@x.covci.s0b.fixed1.fixed4\endcsname{$+0.014$ to $+0.055$}
\expandafter\def\csname R@x.covci.s0b.fixed2.fixed3\endcsname{$+0.003$ to $+0.044$}
\expandafter\def\csname R@x.covci.s0b.geom.fixed4\endcsname{$-0.002$ to $+0.042$}
\expandafter\def\csname R@x.covci.s0b.random.fixed3\endcsname{$+0.001$ to $+0.039$}
\expandafter\def\csname R@x.diff.p0.contact.fixed4\endcsname{$-6$}
\expandafter\def\csname R@x.diff.p0.contact.random\endcsname{$-6$}
\expandafter\def\csname R@x.diff.p0.error.fixed4\endcsname{$-3$}
\expandafter\def\csname R@x.diff.p0.fixed1.fixed4\endcsname{$+9$}
\expandafter\def\csname R@x.diff.p0.geom.fixed4\endcsname{$+2$}
\expandafter\def\csname R@x.diff.p0b.contact.fixed4\endcsname{$-6$}
\expandafter\def\csname R@x.diff.p0b.contact.random\endcsname{$-5$}
\expandafter\def\csname R@x.diff.p0b.error.fixed4\endcsname{$-3$}
\expandafter\def\csname R@x.diff.p0b.fixed1.fixed4\endcsname{$+9$}
\expandafter\def\csname R@x.diff.p0b.geom.fixed4\endcsname{$+2$}
\expandafter\def\csname R@x.diff.s0.contact.fixed4\endcsname{$+1$}
\expandafter\def\csname R@x.diff.s0.contact.random\endcsname{$-10$}
\expandafter\def\csname R@x.diff.s0.error.fixed4\endcsname{$+2$}
\expandafter\def\csname R@x.diff.s0.fixed1.fixed4\endcsname{$+19$}
\expandafter\def\csname R@x.diff.s0.geom.fixed4\endcsname{$+2$}
\expandafter\def\csname R@x.diff.s0.random.fixed2\endcsname{$+0$}
\expandafter\def\csname R@x.diff.s0.random.fixed3\endcsname{$+8$}
\expandafter\def\csname R@x.diff.s0b.contact.fixed4\endcsname{$+0$}
\expandafter\def\csname R@x.diff.s0b.contact.random\endcsname{$-10$}
\expandafter\def\csname R@x.diff.s0b.error.fixed4\endcsname{$+2$}
\expandafter\def\csname R@x.diff.s0b.fixed1.fixed3\endcsname{$+9$}
\expandafter\def\csname R@x.diff.s0b.fixed1.fixed4\endcsname{$+12$}
\expandafter\def\csname R@x.diff.s0b.fixed2.fixed3\endcsname{$+7$}
\expandafter\def\csname R@x.diff.s0b.geom.fixed4\endcsname{$+2$}
\expandafter\def\csname R@x.diff.s0b.random.fixed3\endcsname{$+7$}
\expandafter\def\csname R@x.one.far.ang\endcsname{0.18}
\expandafter\def\csname R@x.one.far.n\endcsname{10,577}
\expandafter\def\csname R@x.one.far.pos\endcsname{0.43}
\expandafter\def\csname R@x.one.near.ang\endcsname{0.79}
\expandafter\def\csname R@x.one.near.n\endcsname{8,623}
\expandafter\def\csname R@x.one.near.pos\endcsname{1.73}
\expandafter\def\csname R@x.pn01.p0.contact.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn01.p0.contact.random\endcsname{9}
\expandafter\def\csname R@x.pn01.p0.error.fixed4\endcsname{9}
\expandafter\def\csname R@x.pn01.p0.fixed1.fixed4\endcsname{7}
\expandafter\def\csname R@x.pn01.p0.geom.fixed4\endcsname{7}
\expandafter\def\csname R@x.pn01.p0b.contact.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn01.p0b.contact.random\endcsname{8}
\expandafter\def\csname R@x.pn01.p0b.error.fixed4\endcsname{9}
\expandafter\def\csname R@x.pn01.p0b.fixed1.fixed4\endcsname{6}
\expandafter\def\csname R@x.pn01.p0b.geom.fixed4\endcsname{7}
\expandafter\def\csname R@x.pn01.s0.contact.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn01.s0.contact.random\endcsname{15}
\expandafter\def\csname R@x.pn01.s0.error.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn01.s0.fixed1.fixed4\endcsname{3}
\expandafter\def\csname R@x.pn01.s0.geom.fixed4\endcsname{9}
\expandafter\def\csname R@x.pn01.s0.random.fixed2\endcsname{11}
\expandafter\def\csname R@x.pn01.s0.random.fixed3\endcsname{8}
\expandafter\def\csname R@x.pn01.s0b.contact.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn01.s0b.contact.random\endcsname{14}
\expandafter\def\csname R@x.pn01.s0b.error.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn01.s0b.fixed1.fixed3\endcsname{7}
\expandafter\def\csname R@x.pn01.s0b.fixed1.fixed4\endcsname{4}
\expandafter\def\csname R@x.pn01.s0b.fixed2.fixed3\endcsname{1}
\expandafter\def\csname R@x.pn01.s0b.geom.fixed4\endcsname{9}
\expandafter\def\csname R@x.pn01.s0b.random.fixed3\endcsname{8}
\expandafter\def\csname R@x.pn10.p0.contact.fixed4\endcsname{4}
\expandafter\def\csname R@x.pn10.p0.contact.random\endcsname{3}
\expandafter\def\csname R@x.pn10.p0.error.fixed4\endcsname{6}
\expandafter\def\csname R@x.pn10.p0.fixed1.fixed4\endcsname{16}
\expandafter\def\csname R@x.pn10.p0.geom.fixed4\endcsname{9}
\expandafter\def\csname R@x.pn10.p0b.contact.fixed4\endcsname{4}
\expandafter\def\csname R@x.pn10.p0b.contact.random\endcsname{3}
\expandafter\def\csname R@x.pn10.p0b.error.fixed4\endcsname{6}
\expandafter\def\csname R@x.pn10.p0b.fixed1.fixed4\endcsname{15}
\expandafter\def\csname R@x.pn10.p0b.geom.fixed4\endcsname{9}
\expandafter\def\csname R@x.pn10.s0.contact.fixed4\endcsname{11}
\expandafter\def\csname R@x.pn10.s0.contact.random\endcsname{5}
\expandafter\def\csname R@x.pn10.s0.error.fixed4\endcsname{12}
\expandafter\def\csname R@x.pn10.s0.fixed1.fixed4\endcsname{22}
\expandafter\def\csname R@x.pn10.s0.geom.fixed4\endcsname{11}
\expandafter\def\csname R@x.pn10.s0.random.fixed2\endcsname{11}
\expandafter\def\csname R@x.pn10.s0.random.fixed3\endcsname{16}
\expandafter\def\csname R@x.pn10.s0b.contact.fixed4\endcsname{10}
\expandafter\def\csname R@x.pn10.s0b.contact.random\endcsname{4}
\expandafter\def\csname R@x.pn10.s0b.error.fixed4\endcsname{12}
\expandafter\def\csname R@x.pn10.s0b.fixed1.fixed3\endcsname{16}
\expandafter\def\csname R@x.pn10.s0b.fixed1.fixed4\endcsname{16}
\expandafter\def\csname R@x.pn10.s0b.fixed2.fixed3\endcsname{8}
\expandafter\def\csname R@x.pn10.s0b.geom.fixed4\endcsname{11}
\expandafter\def\csname R@x.pn10.s0b.random.fixed3\endcsname{15}
\expandafter\def\csname R@x.pp.p0.contact.fixed4\endcsname{0.180}
\expandafter\def\csname R@x.pp.p0.contact.random\endcsname{0.146}
\expandafter\def\csname R@x.pp.p0.error.fixed4\endcsname{0.607}
\expandafter\def\csname R@x.pp.p0.fixed1.fixed4\endcsname{0.093}
\expandafter\def\csname R@x.pp.p0.geom.fixed4\endcsname{0.804}
\expandafter\def\csname R@x.pp.p0b.contact.fixed4\endcsname{0.180}
\expandafter\def\csname R@x.pp.p0b.contact.random\endcsname{0.227}
\expandafter\def\csname R@x.pp.p0b.error.fixed4\endcsname{0.607}
\expandafter\def\csname R@x.pp.p0b.fixed1.fixed4\endcsname{0.078}
\expandafter\def\csname R@x.pp.p0b.geom.fixed4\endcsname{0.804}
\expandafter\def\csname R@x.pp.s0.contact.fixed4\endcsname{1.000}
\expandafter\def\csname R@x.pp.s0.contact.random\endcsname{0.041}
\expandafter\def\csname R@x.pp.s0.error.fixed4\endcsname{0.832}
\expandafter\def\csname R@x.pp.s0.fixed1.fixed4\endcsname{0.0002}
\expandafter\def\csname R@x.pp.s0.geom.fixed4\endcsname{0.824}
\expandafter\def\csname R@x.pp.s0.random.fixed2\endcsname{1.000}
\expandafter\def\csname R@x.pp.s0.random.fixed3\endcsname{0.152}
\expandafter\def\csname R@x.pp.s0b.contact.fixed4\endcsname{1.000}
\expandafter\def\csname R@x.pp.s0b.contact.random\endcsname{0.031}
\expandafter\def\csname R@x.pp.s0b.error.fixed4\endcsname{0.832}
\expandafter\def\csname R@x.pp.s0b.fixed1.fixed3\endcsname{0.093}
\expandafter\def\csname R@x.pp.s0b.fixed1.fixed4\endcsname{0.012}
\expandafter\def\csname R@x.pp.s0b.fixed2.fixed3\endcsname{0.039}
\expandafter\def\csname R@x.pp.s0b.geom.fixed4\endcsname{0.824}
\expandafter\def\csname R@x.pp.s0b.random.fixed3\endcsname{0.210}
\expandafter\def\csname R@x.six.far.ang\endcsname{0.32}
\expandafter\def\csname R@x.six.far.n\endcsname{1,100}
\expandafter\def\csname R@x.six.far.pos\endcsname{0.65}
\expandafter\def\csname R@x.six.near.ang\endcsname{2.88}
\expandafter\def\csname R@x.six.near.n\endcsname{1,900}
\expandafter\def\csname R@x.six.near.pos\endcsname{5.64}
\makeatother


==> numbers2.tex <==
% Generated by revision/build_stage2_assets.py from revision/stage2.json. Do not edit by hand.
\makeatletter
\renewcommand{\S}[1]{\@ifundefined{S@#1}{\textbf{??#1??}}{\csname S@#1\endcsname}}
\@namedef{S@coast.0}{4.6}
\@namedef{S@coast.0.02}{38.0}
\@namedef{S@coast.0.05}{48.4}
\@namedef{S@coast.0.1}{60.5}
\@namedef{S@coast.0.25}{86.3}
\@namedef{S@coast.0.85}{130.1}
\@namedef{S@cum.contactq75.10}{14.8}
\@namedef{S@cum.contactq75.15}{16.9}
\@namedef{S@cum.contactq75.20}{17.8}
\@namedef{S@cum.contactq75.35}{19.7}
\@namedef{S@cum.contactq75.5}{1.8}
\@namedef{S@cum.errorq75.10}{13.7}
\@namedef{S@cum.errorq75.15}{15.6}
\@namedef{S@cum.errorq75.20}{16.3}
\@namedef{S@cum.errorq75.35}{18.0}
\@namedef{S@cum.errorq75.5}{1.3}
\@namedef{S@cum.fixed1.10}{27.4}
\@namedef{S@cum.fixed1.15}{30.3}
\@namedef{S@cum.fixed1.20}{32.2}
\@namedef{S@cum.fixed1.35}{33.7}
\@namedef{S@cum.fixed1.5}{6.1}
\@namedef{S@cum.fixed2.10}{22.5}
\@namedef{S@cum.fixed2.15}{25.8}
\@namedef{S@cum.fixed2.20}{27.1}
\@namedef{S@cum.fixed2.35}{29.4}
\@namedef{S@cum.fixed2.5}{2.6}
\@namedef{S@cum.fixed3.10}{16.8}
\@namedef{S@cum.fixed3.15}{19.0}
\@namedef{S@cum.fixed3.20}{19.8}
\@namedef{S@cum.fixed3.35}{21.4}
\@namedef{S@cum.fixed3.5}{2.4}
\@namedef{S@cum.fixed4.10}{13.3}
\@namedef{S@cum.fixed4.15}{14.5}
\@namedef{S@cum.fixed4.20}{15.7}
\@namedef{S@cum.fixed4.35}{16.8}
\@namedef{S@cum.fixed4.5}{2.9}
\@namedef{S@cum.fixed6.10}{8.7}
\@namedef{S@cum.fixed6.15}{10.0}
\@namedef{S@cum.fixed6.20}{11.0}
\@namedef{S@cum.fixed6.35}{12.9}
\@namedef{S@cum.fixed6.5}{1.0}
\@namedef{S@cum.random.contactq75.10}{16.7}
\@namedef{S@cum.random.contactq75.15}{19.4}
\@namedef{S@cum.random.contactq75.20}{20.6}
\@namedef{S@cum.random.contactq75.35}{22.0}
\@namedef{S@cum.random.contactq75.5}{3.2}
\@namedef{S@err.event.err}{1.58}
\@namedef{S@err.event.errmoving}{2.17}
\@namedef{S@err.event.move}{6.10}
\@namedef{S@err.event.movingshare}{62}
\@namedef{S@err.event.n}{2,704}
\@namedef{S@err.event.rel}{22}
\@namedef{S@err.event.share}{14}
\@namedef{S@err.moving.err}{1.90}
\@namedef{S@err.moving.n}{8,433}
\@namedef{S@err.moving.rel}{18}
\@namedef{S@err.none.err}{0.28}
\@namedef{S@err.none.errmoving}{2.87}
\@namedef{S@err.none.move}{0.02}
\@namedef{S@err.none.movingshare}{1}
\@namedef{S@err.none.n}{9,324}
\@namedef{S@err.none.rel}{133}
\@namedef{S@err.none.share}{49}
\@namedef{S@err.still.err}{0.32}
\@namedef{S@err.still.n}{10,767}
\@namedef{S@err.sustained.err}{1.76}
\@namedef{S@err.sustained.errmoving}{1.82}
\@namedef{S@err.sustained.move}{10.48}
\@namedef{S@err.sustained.movingshare}{93}
\@namedef{S@err.sustained.n}{7,173}
\@namedef{S@err.sustained.rel}{16}
\@namedef{S@err.sustained.share}{37}
\@namedef{S@fire.contact.event.rate}{88}
\@namedef{S@fire.contact.event.share}{58}
\@namedef{S@fire.contact.event.steps}{15}
\@namedef{S@fire.contact.n}{3,437}
\@namedef{S@fire.contact.none.rate}{10}
\@namedef{S@fire.contact.none.share}{29}
\@namedef{S@fire.contact.none.steps}{68}
\@namedef{S@fire.contact.sustained.rate}{17}
\@namedef{S@fire.contact.sustained.share}{13}
\@namedef{S@fire.contact.sustained.steps}{17}
\@namedef{S@fire.error.event.rate}{22}
\@namedef{S@fire.error.event.share}{33}
\@namedef{S@fire.error.event.steps}{15}
\@namedef{S@fire.error.n}{1,549}
\@namedef{S@fire.error.none.rate}{5}
\@namedef{S@fire.error.none.share}{34}
\@namedef{S@fire.error.none.steps}{67}
\@namedef{S@fire.error.sustained.rate}{19}
\@namedef{S@fire.error.sustained.share}{33}
\@namedef{S@fire.error.sustained.steps}{18}
\@namedef{S@fire.random.event.rate}{29}
\@namedef{S@fire.random.event.share}{17}
\@namedef{S@fire.random.event.steps}{16}
\@namedef{S@fire.random.n}{82,394}
\@namedef{S@fire.random.none.rate}{27}
\@namedef{S@fire.random.none.share}{65}
\@namedef{S@fire.random.none.steps}{65}
\@namedef{S@fire.random.sustained.rate}{25}
\@namedef{S@fire.random.sustained.share}{18}
\@namedef{S@fire.random.sustained.steps}{19}
\@namedef{S@or.fixed1.0}{60}
\@namedef{S@or.fixed1.0.02}{32}
\@namedef{S@or.fixed1.0.02.cov}{0.93}
\@namedef{S@or.fixed1.0.05}{16}
\@namedef{S@or.fixed1.0.05.cov}{0.92}
\@namedef{S@or.fixed1.0.1}{8}
\@namedef{S@or.fixed1.0.1.cov}{0.89}
\@namedef{S@or.fixed1.0.25}{3}
\@namedef{S@or.fixed1.0.25.cov}{0.81}
\@namedef{S@or.fixed1.0.85}{27}
\@namedef{S@or.fixed1.0.85.cov}{0.86}
\@namedef{S@or.fixed1.0.cov}{0.96}
\@namedef{S@or.fixed2.0}{51}
\@namedef{S@or.fixed2.0.cov}{0.95}
\@namedef{S@or.fixed3.0}{43}
\@namedef{S@or.fixed3.0.cov}{0.95}
\@namedef{S@or.fixed4.0}{42}
\@namedef{S@or.fixed4.0.cov}{0.95}
\@namedef{S@or.fixed6.0}{24}
\@namedef{S@or.fixed6.0.cov}{0.91}
\@namedef{S@or.n}{64}
\@namedef{S@or.pair.fixed1.fixed2.ci}{+2 to +16}
\@namedef{S@or.pair.fixed1.fixed2.d}{+9}
\@namedef{S@or.pair.fixed1.fixed2.p}{0.011}
\@namedef{S@or.pair.fixed1.fixed2.pp}{$p=0.011$}
\@namedef{S@or.pair.fixed1.fixed4.ci}{+11 to +26}
\@namedef{S@or.pair.fixed1.fixed4.d}{+18}
\@namedef{S@or.pair.fixed1.fixed4.p}{<0.001}
\@namedef{S@or.pair.fixed1.fixed4.pp}{$p<0.001$}
\@namedef{S@or.pair.fixed1.fixed6.ci}{+28 to +44}
\@namedef{S@or.pair.fixed1.fixed6.d}{+36}
\@namedef{S@or.pair.fixed1.fixed6.p}{<0.001}
\@namedef{S@or.pair.fixed1.fixed6.pp}{$p<0.001$}
\@namedef{S@px.F.ci}{+0.0 to +11.8}
\@namedef{S@px.F.d}{+6.0}
\@namedef{S@px.F.hh}{$p_{\mathrm{Holm}}=0.272$}
\@namedef{S@px.F.holm}{0.272}
\@namedef{S@px.F.p}{0.054}
\@namedef{S@px.F.pp}{$p=0.054$}
\@namedef{S@px.Fcov.ci}{+0.022 to +0.064}
\@namedef{S@px.Fcov.d}{+0.041}
\@namedef{S@px.Fcov.hh}{$p_{\mathrm{Holm}}<0.001$}
\@namedef{S@px.Fcov.holm}{<0.001}
\@namedef{S@px.Fcov.p}{<0.001}
\@namedef{S@px.Fcov.pp}{$p<0.001$}
\@namedef{S@px.Fs90.ci}{+3.8 to +15.6}
\@namedef{S@px.Fs90.d}{+9.6}
\@namedef{S@px.Fs90.p}{0.002}
\@namedef{S@px.Fs90.pp}{$p=0.002$}
\@namedef{S@px.Fs97.ci}{+0.8 to +9.4}
\@namedef{S@px.Fs97.d}{+4.6}
\@namedef{S@px.Fs97.p}{0.020}
\@namedef{S@px.Fs97.pp}{$p=0.020$}
\@namedef{S@px.T-contact.ci}{\ensuremath{-}3.9 to +2.8}
\@namedef{S@px.T-contact.d}{\ensuremath{-}0.5}
\@namedef{S@px.T-contact.hh}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.T-contact.holm}{1.000}
\@namedef{S@px.T-contact.p}{0.799}
\@namedef{S@px.T-contact.pp}{$p=0.799$}
\@namedef{S@px.T-contactcov.ci}{\ensuremath{-}0.007 to +0.014}
\@namedef{S@px.T-contactcov.d}{+0.003}
\@namedef{S@px.T-contactcov.hh}{$p_{\mathrm{Holm}}=0.545$}
\@namedef{S@px.T-contactcov.holm}{0.545}
\@namedef{S@px.T-contactcov.p}{0.545}
\@namedef{S@px.T-contactcov.pp}{$p=0.545$}
\@namedef{S@px.T-disagreement.ci}{\ensuremath{-}0.9 to +4.8}
\@namedef{S@px.T-disagreement.d}{+1.8}
\@namedef{S@px.T-disagreement.hh}{$p_{\mathrm{Holm}}=0.825$}
\@namedef{S@px.T-disagreement.holm}{0.825}
\@namedef{S@px.T-disagreement.p}{0.206}
\@namedef{S@px.T-disagreement.pp}{$p=0.206$}
\@namedef{S@px.T-disagreementcov.ci}{+0.001 to +0.026}
\@namedef{S@px.T-disagreementcov.d}{+0.013}
\@namedef{S@px.T-disagreementcov.hh}{$p_{\mathrm{Holm}}=0.111$}
\@namedef{S@px.T-disagreementcov.holm}{0.111}
\@namedef{S@px.T-disagreementcov.p}{0.037}
\@namedef{S@px.T-disagreementcov.pp}{$p=0.037$}
\@namedef{S@px.T-error.ci}{\ensuremath{-}2.5 to +2.8}
\@namedef{S@px.T-error.d}{+0.1}
\@namedef{S@px.T-error.hh}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.T-error.holm}{1.000}
\@namedef{S@px.T-error.p}{0.984}
\@namedef{S@px.T-error.pp}{$p=0.984$}
\@namedef{S@px.T-errorcov.ci}{\ensuremath{-}0.004 to +0.017}
\@namedef{S@px.T-errorcov.d}{+0.006}
\@namedef{S@px.T-errorcov.hh}{$p_{\mathrm{Holm}}=0.470$}
\@namedef{S@px.T-errorcov.holm}{0.470}
\@namedef{S@px.T-errorcov.p}{0.235}
\@namedef{S@px.T-errorcov.pp}{$p=0.235$}
\@namedef{S@px.T-geom.ci}{\ensuremath{-}2.6 to +4.7}
\@namedef{S@px.T-geom.d}{+1.1}
\@namedef{S@px.T-geom.hh}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.T-geom.holm}{1.000}
\@namedef{S@px.T-geom.p}{0.542}
\@namedef{S@px.T-geom.pp}{$p=0.542$}
\@namedef{S@px.T-geomcov.ci}{+0.008 to +0.037}
\@namedef{S@px.T-geomcov.d}{+0.021}
\@namedef{S@px.T-geomcov.hh}{$p_{\mathrm{Holm}}=0.003$}
\@namedef{S@px.T-geomcov.holm}{0.003}
\@namedef{S@px.T-geomcov.p}{<0.001}
\@namedef{S@px.T-geomcov.pp}{$p<0.001$}
\@namedef{S@px.cells}{320}
\@namedef{S@px.contactq25.cov}{0.904}
\@namedef{S@px.contactq25.max}{22}
\@namedef{S@px.contactq25.mean}{16.4}
\@namedef{S@px.contactq25.min}{7}
\@namedef{S@px.contactq25.pct}{26}
\@namedef{S@px.contactq25.rate}{0.81}
\@namedef{S@px.contactq25.rate35}{0.83}
\@namedef{S@px.contactq25.s90}{41.2}
\@namedef{S@px.contactq25.s97}{8.0}
\@namedef{S@px.contactq25.sd}{6.0}
\@namedef{S@px.contactq25.sig}{92}
\@namedef{S@px.contactq25.trig}{79}
\@namedef{S@px.contactq25.u35k}{66.8}
\@namedef{S@px.contactq25.ups}{1859}
\@namedef{S@px.contactq25.ustopk}{52.3}
\@namedef{S@px.contactq50.cov}{0.902}
\@namedef{S@px.contactq50.max}{22}
\@namedef{S@px.contactq50.mean}{14.8}
\@namedef{S@px.contactq50.min}{5}
\@namedef{S@px.contactq50.pct}{23}
\@namedef{S@px.contactq50.rate}{0.63}
\@namedef{S@px.contactq50.rate35}{0.63}
\@namedef{S@px.contactq50.s90}{40.6}
\@namedef{S@px.contactq50.s97}{6.6}
\@namedef{S@px.contactq50.sd}{6.2}
\@namedef{S@px.contactq50.sig}{86}
\@namedef{S@px.contactq50.trig}{59}
\@namedef{S@px.contactq50.u35k}{50.6}
\@namedef{S@px.contactq50.ups}{1441}
\@namedef{S@px.contactq50.ustopk}{41.6}
\@namedef{S@px.contactq75.cov}{0.880}
\@namedef{S@px.contactq75.max}{14}
\@namedef{S@px.contactq75.mean}{11.8}
\@namedef{S@px.contactq75.min}{9}
\@namedef{S@px.contactq75.pct}{18}
\@namedef{S@px.contactq75.rate}{0.35}
\@namedef{S@px.contactq75.rate35}{0.34}
\@namedef{S@px.contactq75.s90}{32.2}
\@namedef{S@px.contactq75.s97}{3.0}
\@namedef{S@px.contactq75.sd}{1.9}
\@namedef{S@px.contactq75.sig}{61}
\@namedef{S@px.contactq75.trig}{25}
\@namedef{S@px.contactq75.u35k}{27.6}
\@namedef{S@px.contactq75.ups}{816}
\@namedef{S@px.contactq75.ustopk}{24.9}
\@namedef{S@px.contactq90.cov}{0.871}
\@namedef{S@px.contactq90.max}{17}
\@namedef{S@px.contactq90.mean}{11.0}
\@namedef{S@px.contactq90.min}{7}
\@namedef{S@px.contactq90.pct}{17}
\@namedef{S@px.contactq90.rate}{0.23}
\@namedef{S@px.contactq90.rate35}{0.22}
\@namedef{S@px.contactq90.s90}{31.6}
\@namedef{S@px.contactq90.s97}{3.4}
\@namedef{S@px.contactq90.sd}{4.0}
\@namedef{S@px.contactq90.sig}{29}
\@namedef{S@px.contactq90.trig}{8}
\@namedef{S@px.contactq90.u35k}{17.9}
\@namedef{S@px.contactq90.ups}{527}
\@namedef{S@px.contactq90.ustopk}{16.1}
\@namedef{S@px.disagreementq25.cov}{0.902}
\@namedef{S@px.disagreementq25.max}{20}
\@namedef{S@px.disagreementq25.mean}{14.2}
\@namedef{S@px.disagreementq25.min}{8}
\@namedef{S@px.disagreementq25.pct}{22}
\@namedef{S@px.disagreementq25.rate}{0.47}
\@namedef{S@px.disagreementq25.rate35}{0.44}
\@namedef{S@px.disagreementq25.s90}{38.6}
\@namedef{S@px.disagreementq25.s97}{7.2}
\@namedef{S@px.disagreementq25.sd}{5.0}
\@namedef{S@px.disagreementq25.sig}{87}
\@namedef{S@px.disagreementq25.trig}{43}
\@namedef{S@px.disagreementq25.u35k}{35.5}
\@namedef{S@px.disagreementq25.ups}{1079}
\@namedef{S@px.disagreementq25.ustopk}{31.7}
\@namedef{S@px.disagreementq50.cov}{0.887}
\@namedef{S@px.disagreementq50.max}{18}
\@namedef{S@px.disagreementq50.mean}{13.6}
\@namedef{S@px.disagreementq50.min}{7}
\@namedef{S@px.disagreementq50.pct}{21}
\@namedef{S@px.disagreementq50.rate}{0.34}
\@namedef{S@px.disagreementq50.rate35}{0.32}
\@namedef{S@px.disagreementq50.s90}{35.4}
\@namedef{S@px.disagreementq50.s97}{5.6}
\@namedef{S@px.disagreementq50.sd}{4.2}
\@namedef{S@px.disagreementq50.sig}{68}
\@namedef{S@px.disagreementq50.trig}{26}
\@namedef{S@px.disagreementq50.u35k}{25.8}
\@namedef{S@px.disagreementq50.ups}{780}
\@namedef{S@px.disagreementq50.ustopk}{23.2}
\@namedef{S@px.disagreementq75.cov}{0.874}
\@namedef{S@px.disagreementq75.max}{16}
\@namedef{S@px.disagreementq75.mean}{11.6}
\@namedef{S@px.disagreementq75.min}{6}
\@namedef{S@px.disagreementq75.pct}{18}
\@namedef{S@px.disagreementq75.rate}{0.23}
\@namedef{S@px.disagreementq75.rate35}{0.22}
\@namedef{S@px.disagreementq75.s90}{33.2}
\@namedef{S@px.disagreementq75.s97}{3.2}
\@namedef{S@px.disagreementq75.sd}{4.3}
\@namedef{S@px.disagreementq75.sig}{38}
\@namedef{S@px.disagreementq75.trig}{10}
\@namedef{S@px.disagreementq75.u35k}{17.9}
\@namedef{S@px.disagreementq75.ups}{527}
\@namedef{S@px.disagreementq75.ustopk}{16.0}
\@namedef{S@px.disagreementq90.cov}{0.861}
\@namedef{S@px.disagreementq90.max}{14}
\@namedef{S@px.disagreementq90.mean}{10.2}
\@namedef{S@px.disagreementq90.min}{6}
\@namedef{S@px.disagreementq90.pct}{16}
\@namedef{S@px.disagreementq90.rate}{0.19}
\@namedef{S@px.disagreementq90.rate35}{0.19}
\@namedef{S@px.disagreementq90.s90}{29.8}
\@namedef{S@px.disagreementq90.s97}{2.4}
\@namedef{S@px.disagreementq90.sd}{3.9}
\@namedef{S@px.disagreementq90.sig}{16}
\@namedef{S@px.disagreementq90.trig}{4}
\@namedef{S@px.disagreementq90.u35k}{15.3}
\@namedef{S@px.disagreementq90.ups}{446}
\@namedef{S@px.disagreementq90.ustopk}{13.8}
\@namedef{S@px.eq.1152.1}{13.8}
\@namedef{S@px.eq.1152.2}{13.0}
\@namedef{S@px.eq.1152.4}{13.4}
\@namedef{S@px.eq.2304.1}{16.6}
\@namedef{S@px.eq.2304.2}{16.8}
\@namedef{S@px.eq.2304.4}{13.0}
\@namedef{S@px.eq.576.1}{8.0}
\@namedef{S@px.eq.576.2}{8.0}
\@namedef{S@px.eq.576.4}{10.6}
\@namedef{S@px.eq.r4}{14.2}
\@namedef{S@px.eq.r8}{19.0}
\@namedef{S@px.errorq25.cov}{0.903}
\@namedef{S@px.errorq25.max}{22}
\@namedef{S@px.errorq25.mean}{15.4}
\@namedef{S@px.errorq25.min}{13}
\@namedef{S@px.errorq25.pct}{24}
\@namedef{S@px.errorq25.rate}{0.59}
\@namedef{S@px.errorq25.rate35}{0.55}
\@namedef{S@px.errorq25.s90}{41.4}
\@namedef{S@px.errorq25.s97}{6.4}
\@namedef{S@px.errorq25.sd}{3.8}
\@namedef{S@px.errorq25.sig}{90}
\@namedef{S@px.errorq25.trig}{56}
\@namedef{S@px.errorq25.u35k}{44.5}
\@namedef{S@px.errorq25.ups}{1356}
\@namedef{S@px.errorq25.ustopk}{39.4}
\@namedef{S@px.errorq50.cov}{0.891}
\@namedef{S@px.errorq50.max}{19}
\@namedef{S@px.errorq50.mean}{13.8}
\@namedef{S@px.errorq50.min}{10}
\@namedef{S@px.errorq50.pct}{22}
\@namedef{S@px.errorq50.rate}{0.38}
\@namedef{S@px.errorq50.rate35}{0.36}
\@namedef{S@px.errorq50.s90}{38.0}
\@namedef{S@px.errorq50.s97}{4.6}
\@namedef{S@px.errorq50.sd}{3.6}
\@namedef{S@px.errorq50.sig}{75}
\@namedef{S@px.errorq50.trig}{32}
\@namedef{S@px.errorq50.u35k}{29.2}
\@namedef{S@px.errorq50.ups}{879}
\@namedef{S@px.errorq50.ustopk}{26.4}
\@namedef{S@px.errorq75.cov}{0.874}
\@namedef{S@px.errorq75.max}{15}
\@namedef{S@px.errorq75.mean}{10.8}
\@namedef{S@px.errorq75.min}{7}
\@namedef{S@px.errorq75.pct}{17}
\@namedef{S@px.errorq75.rate}{0.27}
\@namedef{S@px.errorq75.rate35}{0.26}
\@namedef{S@px.errorq75.s90}{31.2}
\@namedef{S@px.errorq75.s97}{3.8}
\@namedef{S@px.errorq75.sd}{3.6}
\@namedef{S@px.errorq75.sig}{51}
\@namedef{S@px.errorq75.trig}{16}
\@namedef{S@px.errorq75.u35k}{20.9}
\@namedef{S@px.errorq75.ups}{616}
\@namedef{S@px.errorq75.ustopk}{19.0}
\@namedef{S@px.errorq90.cov}{0.860}
\@namedef{S@px.errorq90.max}{13}
\@namedef{S@px.errorq90.mean}{9.2}
\@namedef{S@px.errorq90.min}{6}
\@namedef{S@px.errorq90.pct}{14}
\@namedef{S@px.errorq90.rate}{0.21}
\@namedef{S@px.errorq90.rate35}{0.20}
\@namedef{S@px.errorq90.s90}{29.2}
\@namedef{S@px.errorq90.s97}{2.4}
\@namedef{S@px.errorq90.sd}{3.3}
\@namedef{S@px.errorq90.sig}{23}
\@namedef{S@px.errorq90.trig}{6}
\@namedef{S@px.errorq90.u35k}{16.3}
\@namedef{S@px.errorq90.ups}{475}
\@namedef{S@px.errorq90.ustopk}{14.9}
\@namedef{S@px.f1gtf4}{4}
\@namedef{S@px.fixed1.cov}{0.904}
\@namedef{S@px.fixed1.max}{22}
\@namedef{S@px.fixed1.mean}{16.6}
\@namedef{S@px.fixed1.min}{7}
\@namedef{S@px.fixed1.pct}{26}
\@namedef{S@px.fixed1.rate}{1.00}
\@namedef{S@px.fixed1.rate35}{1.00}
\@namedef{S@px.fixed1.s23}{21}
\@namedef{S@px.fixed1.s90}{41.8}
\@namedef{S@px.fixed1.s97}{8.0}
\@namedef{S@px.fixed1.sd}{6.0}
\@namedef{S@px.fixed1.sig}{0}
\@namedef{S@px.fixed1.trig}{0}
\@namedef{S@px.fixed1.u35k}{80.6}
\@namedef{S@px.fixed1.ups}{2304}
\@namedef{S@px.fixed1.ustopk}{64.9}
\@namedef{S@px.fixed1K16i2.cov}{0.888}
\@namedef{S@px.fixed1K16i2.max}{16}
\@namedef{S@px.fixed1K16i2.mean}{13.8}
\@namedef{S@px.fixed1K16i2.min}{10}
\@namedef{S@px.fixed1K16i2.pct}{22}
\@namedef{S@px.fixed1K16i2.rate}{1.00}
\@namedef{S@px.fixed1K16i2.rate35}{1.00}
\@namedef{S@px.fixed1K16i2.s90}{36.6}
\@namedef{S@px.fixed1K16i2.s97}{5.6}
\@namedef{S@px.fixed1K16i2.sd}{2.3}
\@namedef{S@px.fixed1K16i2.sig}{0}
\@namedef{S@px.fixed1K16i2.trig}{0}
\@namedef{S@px.fixed1K16i2.u35k}{40.3}
\@namedef{S@px.fixed1K16i2.ups}{1152}
\@namedef{S@px.fixed1K16i2.ustopk}{34.1}
\@namedef{S@px.fixed1K8i2.cov}{0.829}
\@namedef{S@px.fixed1K8i2.max}{10}
\@namedef{S@px.fixed1K8i2.mean}{8.0}
\@namedef{S@px.fixed1K8i2.min}{6}
\@namedef{S@px.fixed1K8i2.pct}{12}
\@namedef{S@px.fixed1K8i2.rate}{1.00}
\@namedef{S@px.fixed1K8i2.rate35}{1.00}
\@namedef{S@px.fixed1K8i2.s90}{25.0}
\@namedef{S@px.fixed1K8i2.s97}{2.2}
\@namedef{S@px.fixed1K8i2.sd}{1.6}
\@namedef{S@px.fixed1K8i2.sig}{0}
\@namedef{S@px.fixed1K8i2.trig}{0}
\@namedef{S@px.fixed1K8i2.u35k}{20.2}
\@namedef{S@px.fixed1K8i2.ups}{576}
\@namedef{S@px.fixed1K8i2.ustopk}{18.4}
\@namedef{S@px.fixed2.cov}{0.887}
\@namedef{S@px.fixed2.max}{18}
\@namedef{S@px.fixed2.mean}{13.0}
\@namedef{S@px.fixed2.min}{6}
\@namedef{S@px.fixed2.pct}{20}
\@namedef{S@px.fixed2.rate}{0.52}
\@namedef{S@px.fixed2.rate35}{0.51}
\@namedef{S@px.fixed2.s23}{18}
\@namedef{S@px.fixed2.s90}{37.4}
\@namedef{S@px.fixed2.s97}{6.4}
\@namedef{S@px.fixed2.sd}{4.5}
\@namedef{S@px.fixed2.sig}{0}
\@namedef{S@px.fixed2.trig}{0}
\@namedef{S@px.fixed2.u35k}{41.5}
\@namedef{S@px.fixed2.ups}{1187}
\@namedef{S@px.fixed2.ustopk}{35.3}
\@namedef{S@px.fixed2K16i2.cov}{0.850}
\@namedef{S@px.fixed2K16i2.max}{13}
\@namedef{S@px.fixed2K16i2.mean}{8.0}
\@namedef{S@px.fixed2K16i2.min}{5}
\@namedef{S@px.fixed2K16i2.pct}{12}
\@namedef{S@px.fixed2K16i2.rate}{0.51}
\@namedef{S@px.fixed2K16i2.rate35}{0.51}
\@namedef{S@px.fixed2K16i2.s90}{29.0}
\@namedef{S@px.fixed2K16i2.s97}{2.8}
\@namedef{S@px.fixed2K16i2.sd}{3.0}
\@namedef{S@px.fixed2K16i2.sig}{0}
\@namedef{S@px.fixed2K16i2.trig}{0}
\@namedef{S@px.fixed2K16i2.u35k}{20.7}
\@namedef{S@px.fixed2K16i2.ups}{592}
\@namedef{S@px.fixed2K16i2.ustopk}{19.0}
\@namedef{S@px.fixed2K64i2.cov}{0.899}
\@namedef{S@px.fixed2K64i2.max}{21}
\@namedef{S@px.fixed2K64i2.mean}{16.8}
\@namedef{S@px.fixed2K64i2.min}{11}
\@namedef{S@px.fixed2K64i2.pct}{26}
\@namedef{S@px.fixed2K64i2.rate}{0.52}
\@namedef{S@px.fixed2K64i2.rate35}{0.51}
\@namedef{S@px.fixed2K64i2.s90}{41.6}
\@namedef{S@px.fixed2K64i2.s97}{6.4}
\@namedef{S@px.fixed2K64i2.sd}{3.9}
\@namedef{S@px.fixed2K64i2.sig}{0}
\@namedef{S@px.fixed2K64i2.trig}{0}
\@namedef{S@px.fixed2K64i2.u35k}{82.9}
\@namedef{S@px.fixed2K64i2.ups}{2374}
\@namedef{S@px.fixed2K64i2.ustopk}{67.1}
\@namedef{S@px.fixed3.cov}{0.879}
\@namedef{S@px.fixed3.max}{16}
\@namedef{S@px.fixed3.mean}{12.4}
\@namedef{S@px.fixed3.min}{7}
\@namedef{S@px.fixed3.pct}{19}
\@namedef{S@px.fixed3.rate}{0.34}
\@namedef{S@px.fixed3.rate35}{0.34}
\@namedef{S@px.fixed3.s23}{15}
\@namedef{S@px.fixed3.s90}{35.6}
\@namedef{S@px.fixed3.s97}{4.0}
\@namedef{S@px.fixed3.sd}{4.1}
\@namedef{S@px.fixed3.sig}{0}
\@namedef{S@px.fixed3.trig}{0}
\@namedef{S@px.fixed3.u35k}{27.6}
\@namedef{S@px.fixed3.ups}{793}
\@namedef{S@px.fixed3.ustopk}{24.0}
\@namedef{S@px.fixed4.cov}{0.863}
\@namedef{S@px.fixed4.max}{14}
\@namedef{S@px.fixed4.mean}{10.6}
\@namedef{S@px.fixed4.min}{9}
\@namedef{S@px.fixed4.pct}{17}
\@namedef{S@px.fixed4.rate}{0.26}
\@namedef{S@px.fixed4.rate35}{0.26}
\@namedef{S@px.fixed4.s23}{14}
\@namedef{S@px.fixed4.s90}{32.2}
\@namedef{S@px.fixed4.s97}{3.4}
\@namedef{S@px.fixed4.sd}{2.1}
\@namedef{S@px.fixed4.sig}{0}
\@namedef{S@px.fixed4.trig}{0}
\@namedef{S@px.fixed4.u35k}{20.7}
\@namedef{S@px.fixed4.ups}{597}
\@namedef{S@px.fixed4.ustopk}{18.4}
\@namedef{S@px.fixed4K128i2.cov}{0.892}
\@namedef{S@px.fixed4K128i2.max}{16}
\@namedef{S@px.fixed4K128i2.mean}{13.0}
\@namedef{S@px.fixed4K128i2.min}{9}
\@namedef{S@px.fixed4K128i2.pct}{20}
\@namedef{S@px.fixed4K128i2.rate}{0.26}
\@namedef{S@px.fixed4K128i2.rate35}{0.26}
\@namedef{S@px.fixed4K128i2.s90}{35.6}
\@namedef{S@px.fixed4K128i2.s97}{3.8}
\@namedef{S@px.fixed4K128i2.sd}{2.5}
\@namedef{S@px.fixed4K128i2.sig}{0}
\@namedef{S@px.fixed4K128i2.trig}{0}
\@namedef{S@px.fixed4K128i2.u35k}{82.9}
\@namedef{S@px.fixed4K128i2.ups}{2390}
\@namedef{S@px.fixed4K128i2.ustopk}{71.7}
\@namedef{S@px.fixed4K32i8.cov}{0.911}
\@namedef{S@px.fixed4K32i8.max}{30}
\@namedef{S@px.fixed4K32i8.mean}{19.0}
\@namedef{S@px.fixed4K32i8.min}{7}
\@namedef{S@px.fixed4K32i8.pct}{30}
\@namedef{S@px.fixed4K32i8.rate}{0.26}
\@namedef{S@px.fixed4K32i8.rate35}{0.26}
\@namedef{S@px.fixed4K32i8.s90}{43.0}
\@namedef{S@px.fixed4K32i8.s97}{6.2}
\@namedef{S@px.fixed4K32i8.sd}{8.2}
\@namedef{S@px.fixed4K32i8.sig}{0}
\@namedef{S@px.fixed4K32i8.trig}{0}
\@namedef{S@px.fixed4K32i8.u35k}{82.9}
\@namedef{S@px.fixed4K32i8.ups}{2398}
\@namedef{S@px.fixed4K32i8.ustopk}{65.8}
\@namedef{S@px.fixed4K64i2.cov}{0.881}
\@namedef{S@px.fixed4K64i2.max}{23}
\@namedef{S@px.fixed4K64i2.mean}{13.4}
\@namedef{S@px.fixed4K64i2.min}{7}
\@namedef{S@px.fixed4K64i2.pct}{21}
\@namedef{S@px.fixed4K64i2.rate}{0.26}
\@namedef{S@px.fixed4K64i2.rate35}{0.26}
\@namedef{S@px.fixed4K64i2.s90}{34.8}
\@namedef{S@px.fixed4K64i2.s97}{4.4}
\@namedef{S@px.fixed4K64i2.sd}{6.3}
\@namedef{S@px.fixed4K64i2.sig}{0}
\@namedef{S@px.fixed4K64i2.trig}{0}
\@namedef{S@px.fixed4K64i2.u35k}{41.5}
\@namedef{S@px.fixed4K64i2.ups}{1198}
\@namedef{S@px.fixed4K64i2.ustopk}{35.6}
\@namedef{S@px.fixed4K64i4.cov}{0.897}
\@namedef{S@px.fixed4K64i4.max}{20}
\@namedef{S@px.fixed4K64i4.mean}{14.2}
\@namedef{S@px.fixed4K64i4.min}{7}
\@namedef{S@px.fixed4K64i4.pct}{22}
\@namedef{S@px.fixed4K64i4.rate}{0.26}
\@namedef{S@px.fixed4K64i4.rate35}{0.26}
\@namedef{S@px.fixed4K64i4.s90}{40.4}
\@namedef{S@px.fixed4K64i4.s97}{5.0}
\@namedef{S@px.fixed4K64i4.sd}{5.3}
\@namedef{S@px.fixed4K64i4.sig}{0}
\@namedef{S@px.fixed4K64i4.trig}{0}
\@namedef{S@px.fixed4K64i4.u35k}{82.9}
\@namedef{S@px.fixed4K64i4.ups}{2392}
\@namedef{S@px.fixed4K64i4.ustopk}{70.0}
\@namedef{S@px.fixed6.cov}{0.853}
\@namedef{S@px.fixed6.max}{13}
\@namedef{S@px.fixed6.mean}{9.6}
\@namedef{S@px.fixed6.min}{6}
\@namedef{S@px.fixed6.pct}{15}
\@namedef{S@px.fixed6.rate}{0.17}
\@namedef{S@px.fixed6.rate35}{0.17}
\@namedef{S@px.fixed6.s23}{13}
\@namedef{S@px.fixed6.s90}{28.0}
\@namedef{S@px.fixed6.s97}{2.2}
\@namedef{S@px.fixed6.sd}{3.4}
\@namedef{S@px.fixed6.sig}{0}
\@namedef{S@px.fixed6.trig}{0}
\@namedef{S@px.fixed6.u35k}{13.8}
\@namedef{S@px.fixed6.ups}{400}
\@namedef{S@px.fixed6.ustopk}{12.5}
\@namedef{S@px.geom.cov}{0.888}
\@namedef{S@px.geom.max}{15}
\@namedef{S@px.geom.mean}{11.8}
\@namedef{S@px.geom.min}{9}
\@namedef{S@px.geom.pct}{18}
\@namedef{S@px.geom.rate}{0.27}
\@namedef{S@px.geom.rate35}{0.26}
\@namedef{S@px.geom.s90}{34.6}
\@namedef{S@px.geom.s97}{5.2}
\@namedef{S@px.geom.sd}{2.4}
\@namedef{S@px.geom.sig}{46}
\@namedef{S@px.geom.trig}{14}
\@namedef{S@px.geom.u35k}{20.9}
\@namedef{S@px.geom.ups}{612}
\@namedef{S@px.geom.ustopk}{18.5}
\@namedef{S@px.holm10.max}{0.007}
\@namedef{S@px.mono}{1}
\@namedef{S@px.pair.budget.p1.ci}{+1.2 to +15.8}
\@namedef{S@px.pair.budget.p1.d}{+8.6}
\@namedef{S@px.pair.budget.p1.p}{0.028}
\@namedef{S@px.pair.budget.p1.pp}{$p=0.028$}
\@namedef{S@px.pair.budget.p2.ci}{+2.0 to +15.6}
\@namedef{S@px.pair.budget.p2.d}{+8.8}
\@namedef{S@px.pair.budget.p2.p}{0.014}
\@namedef{S@px.pair.budget.p2.pp}{$p=0.014$}
\@namedef{S@px.pair.budget.p4.ci}{\ensuremath{-}3.2 to +8.0}
\@namedef{S@px.pair.budget.p4.d}{+2.4}
\@namedef{S@px.pair.budget.p4.p}{0.403}
\@namedef{S@px.pair.budget.p4.pp}{$p=0.403$}
\@namedef{S@px.pair.cand.k128.k64.ci}{\ensuremath{-}7.6 to +6.2}
\@namedef{S@px.pair.cand.k128.k64.d}{\ensuremath{-}0.4}
\@namedef{S@px.pair.cand.k128.k64.p}{0.943}
\@namedef{S@px.pair.cand.k128.k64.pp}{$p=0.943$}
\@namedef{S@px.pair.cand.k64.fixed4.ci}{\ensuremath{-}3.6 to +9.8}
\@namedef{S@px.pair.cand.k64.fixed4.d}{+2.8}
\@namedef{S@px.pair.cand.k64.fixed4.p}{0.414}
\@namedef{S@px.pair.cand.k64.fixed4.pp}{$p=0.414$}
\@namedef{S@px.pair.fixed1.fixed2.ci}{\ensuremath{-}1.4 to +8.8}
\@namedef{S@px.pair.fixed1.fixed2.d}{+3.6}
\@namedef{S@px.pair.fixed1.fixed2.p}{0.171}
\@namedef{S@px.pair.fixed1.fixed2.pp}{$p=0.171$}
\@namedef{S@px.pair.fixed2.fixed3.ci}{\ensuremath{-}4.2 to +5.4}
\@namedef{S@px.pair.fixed2.fixed3.d}{+0.6}
\@namedef{S@px.pair.fixed2.fixed3.p}{0.826}
\@namedef{S@px.pair.fixed2.fixed3.pp}{$p=0.826$}
\@namedef{S@px.pair.fixed3.fixed4.ci}{\ensuremath{-}2.8 to +6.8}
\@namedef{S@px.pair.fixed3.fixed4.d}{+1.8}
\@namedef{S@px.pair.fixed3.fixed4.p}{0.483}
\@namedef{S@px.pair.fixed3.fixed4.pp}{$p=0.483$}
\@namedef{S@px.pair.fixed4.fixed6.ci}{\ensuremath{-}3.2 to +5.2}
\@namedef{S@px.pair.fixed4.fixed6.d}{+1.0}
\@namedef{S@px.pair.fixed4.fixed6.p}{0.656}
\@namedef{S@px.pair.fixed4.fixed6.pp}{$p=0.656$}
\@namedef{S@px.pair.period.1152.ci}{\ensuremath{-}6.6 to +6.8}
\@namedef{S@px.pair.period.1152.d}{+0.4}
\@namedef{S@px.pair.period.1152.p}{0.915}
\@namedef{S@px.pair.period.1152.pp}{$p=0.915$}
\@namedef{S@px.pair.period.2304.ci}{\ensuremath{-}3.2 to +10.8}
\@namedef{S@px.pair.period.2304.d}{+3.6}
\@namedef{S@px.pair.period.2304.p}{0.330}
\@namedef{S@px.pair.period.2304.pp}{$p=0.330$}
\@namedef{S@px.pair.period.576.ci}{\ensuremath{-}7.6 to +2.8}
\@namedef{S@px.pair.period.576.d}{\ensuremath{-}2.6}
\@namedef{S@px.pair.period.576.p}{0.336}
\@namedef{S@px.pair.period.576.pp}{$p=0.336$}
\@namedef{S@px.pair.rounds.r4.fixed1.ci}{\ensuremath{-}8.4 to +3.4}
\@namedef{S@px.pair.rounds.r4.fixed1.d}{\ensuremath{-}2.4}
\@namedef{S@px.pair.rounds.r4.fixed1.p}{0.448}
\@namedef{S@px.pair.rounds.r4.fixed1.pp}{$p=0.448$}
\@namedef{S@px.pair.rounds.r4.k128.ci}{\ensuremath{-}4.8 to +7.4}
\@namedef{S@px.pair.rounds.r4.k128.d}{+1.2}
\@namedef{S@px.pair.rounds.r4.k128.p}{0.719}
\@namedef{S@px.pair.rounds.r4.k128.pp}{$p=0.719$}
\@namedef{S@px.pair.rounds.r8.fixed1.ci}{\ensuremath{-}3.8 to +9.0}
\@namedef{S@px.pair.rounds.r8.fixed1.d}{+2.4}
\@namedef{S@px.pair.rounds.r8.fixed1.p}{0.470}
\@namedef{S@px.pair.rounds.r8.fixed1.pp}{$p=0.470$}
\@namedef{S@px.pair.rounds.r8.fixed4.ci}{+1.2 to +15.6}
\@namedef{S@px.pair.rounds.r8.fixed4.d}{+8.4}
\@namedef{S@px.pair.rounds.r8.fixed4.p}{0.027}
\@namedef{S@px.pair.rounds.r8.fixed4.pp}{$p=0.027$}
\@namedef{S@px.pair.rounds.r8.k128.ci}{\ensuremath{-}0.8 to +13.2}
\@namedef{S@px.pair.rounds.r8.k128.d}{+6.0}
\@namedef{S@px.pair.rounds.r8.k128.p}{0.086}
\@namedef{S@px.pair.rounds.r8.k128.pp}{$p=0.086$}
\@namedef{S@px.paircov.budget.p1.ci}{+0.047 to +0.105}
\@namedef{S@px.paircov.budget.p1.d}{+0.075}
\@namedef{S@px.paircov.budget.p1.p}{<0.001}
\@namedef{S@px.paircov.budget.p1.pp}{$p<0.001$}
\@namedef{S@px.paircov.budget.p2.ci}{+0.024 to +0.074}
\@namedef{S@px.paircov.budget.p2.d}{+0.048}
\@namedef{S@px.paircov.budget.p2.p}{<0.001}
\@namedef{S@px.paircov.budget.p2.pp}{$p<0.001$}
\@namedef{S@px.paircov.budget.p4.ci}{+0.008 to +0.053}
\@namedef{S@px.paircov.budget.p4.d}{+0.029}
\@namedef{S@px.paircov.budget.p4.p}{0.005}
\@namedef{S@px.paircov.budget.p4.pp}{$p=0.005$}
\@namedef{S@px.paircov.cand.k128.k64.ci}{\ensuremath{-}0.005 to +0.031}
\@namedef{S@px.paircov.cand.k128.k64.d}{+0.011}
\@namedef{S@px.paircov.cand.k128.k64.p}{0.189}
\@namedef{S@px.paircov.cand.k128.k64.pp}{$p=0.189$}
\@namedef{S@px.paircov.cand.k64.fixed4.ci}{\ensuremath{-}0.008 to +0.045}
\@namedef{S@px.paircov.cand.k64.fixed4.d}{+0.017}
\@namedef{S@px.paircov.cand.k64.fixed4.p}{0.169}
\@namedef{S@px.paircov.cand.k64.fixed4.pp}{$p=0.169$}
\@namedef{S@px.paircov.fixed1.fixed2.ci}{+0.003 to +0.033}
\@namedef{S@px.paircov.fixed1.fixed2.d}{+0.017}
\@namedef{S@px.paircov.fixed1.fixed2.p}{0.012}
\@namedef{S@px.paircov.fixed1.fixed2.pp}{$p=0.012$}
\@namedef{S@px.paircov.fixed2.fixed3.ci}{\ensuremath{-}0.002 to +0.020}
\@namedef{S@px.paircov.fixed2.fixed3.d}{+0.009}
\@namedef{S@px.paircov.fixed2.fixed3.p}{0.112}
\@namedef{S@px.paircov.fixed2.fixed3.pp}{$p=0.112$}
\@namedef{S@px.paircov.fixed3.fixed4.ci}{+0.003 to +0.030}
\@namedef{S@px.paircov.fixed3.fixed4.d}{+0.015}
\@namedef{S@px.paircov.fixed3.fixed4.p}{0.021}
\@namedef{S@px.paircov.fixed3.fixed4.pp}{$p=0.021$}
\@namedef{S@px.paircov.fixed4.fixed6.ci}{\ensuremath{-}0.005 to +0.024}
\@namedef{S@px.paircov.fixed4.fixed6.d}{+0.010}
\@namedef{S@px.paircov.fixed4.fixed6.p}{0.176}
\@namedef{S@px.paircov.fixed4.fixed6.pp}{$p=0.176$}
\@namedef{S@px.paircov.period.1152.ci}{\ensuremath{-}0.013 to +0.031}
\@namedef{S@px.paircov.period.1152.d}{+0.008}
\@namedef{S@px.paircov.period.1152.p}{0.455}
\@namedef{S@px.paircov.period.1152.pp}{$p=0.455$}
\@namedef{S@px.paircov.period.2304.ci}{\ensuremath{-}0.000 to +0.026}
\@namedef{S@px.paircov.period.2304.d}{+0.012}
\@namedef{S@px.paircov.period.2304.p}{0.052}
\@namedef{S@px.paircov.period.2304.pp}{$p=0.052$}
\@namedef{S@px.paircov.period.576.ci}{\ensuremath{-}0.067 to +0.000}
\@namedef{S@px.paircov.period.576.d}{\ensuremath{-}0.034}
\@namedef{S@px.paircov.period.576.p}{0.051}
\@namedef{S@px.paircov.period.576.pp}{$p=0.051$}
\@namedef{S@px.paircov.rounds.r4.fixed1.ci}{\ensuremath{-}0.021 to +0.005}
\@namedef{S@px.paircov.rounds.r4.fixed1.d}{\ensuremath{-}0.008}
\@namedef{S@px.paircov.rounds.r4.fixed1.p}{0.234}
\@namedef{S@px.paircov.rounds.r4.fixed1.pp}{$p=0.234$}
\@namedef{S@px.paircov.rounds.r4.k128.ci}{\ensuremath{-}0.008 to +0.018}
\@namedef{S@px.paircov.rounds.r4.k128.d}{+0.005}
\@namedef{S@px.paircov.rounds.r4.k128.p}{0.465}
\@namedef{S@px.paircov.rounds.r4.k128.pp}{$p=0.465$}
\@namedef{S@px.paircov.rounds.r8.fixed1.ci}{\ensuremath{-}0.006 to +0.018}
\@namedef{S@px.paircov.rounds.r8.fixed1.d}{+0.007}
\@namedef{S@px.paircov.rounds.r8.fixed1.p}{0.246}
\@namedef{S@px.paircov.rounds.r8.fixed1.pp}{$p=0.246$}
\@namedef{S@px.paircov.rounds.r8.fixed4.ci}{+0.028 to +0.072}
\@namedef{S@px.paircov.rounds.r8.fixed4.d}{+0.048}
\@namedef{S@px.paircov.rounds.r8.fixed4.p}{<0.001}
\@namedef{S@px.paircov.rounds.r8.fixed4.pp}{$p<0.001$}
\@namedef{S@px.paircov.rounds.r8.k128.ci}{+0.007 to +0.031}
\@namedef{S@px.paircov.rounds.r8.k128.d}{+0.019}
\@namedef{S@px.paircov.rounds.r8.k128.p}{0.007}
\@namedef{S@px.paircov.rounds.r8.k128.pp}{$p=0.007$}
\@namedef{S@px.prim.halfwidth}{3.7}
\@namedef{S@px.prim.maxhi}{+4.8}
\@namedef{S@px.prim.minlo}{\ensuremath{-}3.9}
\@namedef{S@px.r35.maxexcess}{+0.018}
\@namedef{S@px.r35.maxexcess4}{0.0180}
\@namedef{S@px.r35.minexcess}{\ensuremath{-}0.031}
\@namedef{S@px.random.contactq25.cov}{0.901}
\@namedef{S@px.random.contactq25.max}{22}
\@namedef{S@px.random.contactq25.mean}{16.6}
\@namedef{S@px.random.contactq25.min}{9}
\@namedef{S@px.random.contactq25.pct}{26}
\@namedef{S@px.random.contactq25.rate}{0.81}
\@namedef{S@px.random.contactq25.rate35}{0.81}
\@namedef{S@px.random.contactq25.s90}{39.4}
\@namedef{S@px.random.contactq25.s97}{3.4}
\@namedef{S@px.random.contactq25.sd}{4.8}
\@namedef{S@px.random.contactq25.sig}{96}
\@namedef{S@px.random.contactq25.trig}{80}
\@namedef{S@px.random.contactq25.u35k}{65.3}
\@namedef{S@px.random.contactq25.ups}{1868}
\@namedef{S@px.random.contactq25.ustopk}{53.0}
\@namedef{S@px.random.contactq50.cov}{0.894}
\@namedef{S@px.random.contactq50.max}{20}
\@namedef{S@px.random.contactq50.mean}{14.9}
\@namedef{S@px.random.contactq50.min}{9}
\@namedef{S@px.random.contactq50.pct}{23}
\@namedef{S@px.random.contactq50.rate}{0.62}
\@namedef{S@px.random.contactq50.rate35}{0.62}
\@namedef{S@px.random.contactq50.s90}{37.4}
\@namedef{S@px.random.contactq50.s97}{2.0}
\@namedef{S@px.random.contactq50.sd}{4.1}
\@namedef{S@px.random.contactq50.sig}{94}
\@namedef{S@px.random.contactq50.trig}{61}
\@namedef{S@px.random.contactq50.u35k}{50.1}
\@namedef{S@px.random.contactq50.ups}{1436}
\@namedef{S@px.random.contactq50.ustopk}{41.6}
\@namedef{S@px.random.contactq75.cov}{0.877}
\@namedef{S@px.random.contactq75.max}{16}
\@namedef{S@px.random.contactq75.mean}{12.3}
\@namedef{S@px.random.contactq75.min}{8}
\@namedef{S@px.random.contactq75.pct}{19}
\@namedef{S@px.random.contactq75.rate}{0.35}
\@namedef{S@px.random.contactq75.rate35}{0.35}
\@namedef{S@px.random.contactq75.s90}{33.0}
\@namedef{S@px.random.contactq75.s97}{0.8}
\@namedef{S@px.random.contactq75.sd}{2.9}
\@namedef{S@px.random.contactq75.sig}{76}
\@namedef{S@px.random.contactq75.trig}{29}
\@namedef{S@px.random.contactq75.u35k}{28.1}
\@namedef{S@px.random.contactq75.ups}{807}
\@namedef{S@px.random.contactq75.ustopk}{24.4}
\@namedef{S@px.random.contactq90.cov}{0.861}
\@namedef{S@px.random.contactq90.max}{13}
\@namedef{S@px.random.contactq90.mean}{9.8}
\@namedef{S@px.random.contactq90.min}{6}
\@namedef{S@px.random.contactq90.pct}{15}
\@namedef{S@px.random.contactq90.rate}{0.22}
\@namedef{S@px.random.contactq90.rate35}{0.22}
\@namedef{S@px.random.contactq90.s90}{28.4}
\@namedef{S@px.random.contactq90.s97}{0.8}
\@namedef{S@px.random.contactq90.sd}{2.8}
\@namedef{S@px.random.contactq90.sig}{35}
\@namedef{S@px.random.contactq90.trig}{9}
\@namedef{S@px.random.contactq90.u35k}{18.0}
\@namedef{S@px.random.contactq90.ups}{518}
\@namedef{S@px.random.contactq90.ustopk}{16.2}
\@namedef{S@px.random.disagreementq25.cov}{0.885}
\@namedef{S@px.random.disagreementq25.max}{17}
\@namedef{S@px.random.disagreementq25.mean}{13.5}
\@namedef{S@px.random.disagreementq25.min}{8}
\@namedef{S@px.random.disagreementq25.pct}{21}
\@namedef{S@px.random.disagreementq25.rate}{0.46}
\@namedef{S@px.random.disagreementq25.rate35}{0.46}
\@namedef{S@px.random.disagreementq25.s90}{34.2}
\@namedef{S@px.random.disagreementq25.s97}{0.8}
\@namedef{S@px.random.disagreementq25.sd}{3.4}
\@namedef{S@px.random.disagreementq25.sig}{88}
\@namedef{S@px.random.disagreementq25.trig}{43}
\@namedef{S@px.random.disagreementq25.u35k}{36.9}
\@namedef{S@px.random.disagreementq25.ups}{1060}
\@namedef{S@px.random.disagreementq25.ustopk}{31.4}
\@namedef{S@px.random.disagreementq50.cov}{0.875}
\@namedef{S@px.random.disagreementq50.max}{15}
\@namedef{S@px.random.disagreementq50.mean}{11.9}
\@namedef{S@px.random.disagreementq50.min}{7}
\@namedef{S@px.random.disagreementq50.pct}{19}
\@namedef{S@px.random.disagreementq50.rate}{0.34}
\@namedef{S@px.random.disagreementq50.rate35}{0.33}
\@namedef{S@px.random.disagreementq50.s90}{32.6}
\@namedef{S@px.random.disagreementq50.s97}{0.8}
\@namedef{S@px.random.disagreementq50.sd}{3.1}
\@namedef{S@px.random.disagreementq50.sig}{73}
\@namedef{S@px.random.disagreementq50.trig}{27}
\@namedef{S@px.random.disagreementq50.u35k}{26.9}
\@namedef{S@px.random.disagreementq50.ups}{774}
\@namedef{S@px.random.disagreementq50.ustopk}{23.4}
\@namedef{S@px.random.disagreementq75.cov}{0.862}
\@namedef{S@px.random.disagreementq75.max}{14}
\@namedef{S@px.random.disagreementq75.mean}{9.8}
\@namedef{S@px.random.disagreementq75.min}{6}
\@namedef{S@px.random.disagreementq75.pct}{15}
\@namedef{S@px.random.disagreementq75.rate}{0.22}
\@namedef{S@px.random.disagreementq75.rate35}{0.22}
\@namedef{S@px.random.disagreementq75.s90}{28.2}
\@namedef{S@px.random.disagreementq75.s97}{0.8}
\@namedef{S@px.random.disagreementq75.sd}{3.1}
\@namedef{S@px.random.disagreementq75.sig}{35}
\@namedef{S@px.random.disagreementq75.trig}{9}
\@namedef{S@px.random.disagreementq75.u35k}{18.0}
\@namedef{S@px.random.disagreementq75.ups}{518}
\@namedef{S@px.random.disagreementq75.ustopk}{16.1}
\@namedef{S@px.random.disagreementq90.cov}{0.857}
\@namedef{S@px.random.disagreementq90.max}{13}
\@namedef{S@px.random.disagreementq90.mean}{9.8}
\@namedef{S@px.random.disagreementq90.min}{6}
\@namedef{S@px.random.disagreementq90.pct}{15}
\@namedef{S@px.random.disagreementq90.rate}{0.19}
\@namedef{S@px.random.disagreementq90.rate35}{0.19}
\@namedef{S@px.random.disagreementq90.s90}{28.4}
\@namedef{S@px.random.disagreementq90.s97}{2.0}
\@namedef{S@px.random.disagreementq90.sd}{3.3}
\@namedef{S@px.random.disagreementq90.sig}{13}
\@namedef{S@px.random.disagreementq90.trig}{3}
\@namedef{S@px.random.disagreementq90.u35k}{15.3}
\@namedef{S@px.random.disagreementq90.ups}{440}
\@namedef{S@px.random.disagreementq90.ustopk}{13.7}
\@namedef{S@px.random.errorq25.cov}{0.892}
\@namedef{S@px.random.errorq25.max}{20}
\@namedef{S@px.random.errorq25.mean}{14.6}
\@namedef{S@px.random.errorq25.min}{9}
\@namedef{S@px.random.errorq25.pct}{23}
\@namedef{S@px.random.errorq25.rate}{0.59}
\@namedef{S@px.random.errorq25.rate35}{0.58}
\@namedef{S@px.random.errorq25.s90}{36.8}
\@namedef{S@px.random.errorq25.s97}{2.0}
\@namedef{S@px.random.errorq25.sd}{4.1}
\@namedef{S@px.random.errorq25.sig}{93}
\@namedef{S@px.random.errorq25.trig}{57}
\@namedef{S@px.random.errorq25.u35k}{47.0}
\@namedef{S@px.random.errorq25.ups}{1349}
\@namedef{S@px.random.errorq25.ustopk}{39.3}
\@namedef{S@px.random.errorq50.cov}{0.880}
\@namedef{S@px.random.errorq50.max}{16}
\@namedef{S@px.random.errorq50.mean}{12.6}
\@namedef{S@px.random.errorq50.min}{8}
\@namedef{S@px.random.errorq50.pct}{20}
\@namedef{S@px.random.errorq50.rate}{0.38}
\@namedef{S@px.random.errorq50.rate35}{0.37}
\@namedef{S@px.random.errorq50.s90}{32.8}
\@namedef{S@px.random.errorq50.s97}{1.0}
\@namedef{S@px.random.errorq50.sd}{3.1}
\@namedef{S@px.random.errorq50.sig}{80}
\@namedef{S@px.random.errorq50.trig}{32}
\@namedef{S@px.random.errorq50.u35k}{30.2}
\@namedef{S@px.random.errorq50.ups}{866}
\@namedef{S@px.random.errorq50.ustopk}{26.0}
\@namedef{S@px.random.errorq75.cov}{0.867}
\@namedef{S@px.random.errorq75.max}{14}
\@namedef{S@px.random.errorq75.mean}{10.7}
\@namedef{S@px.random.errorq75.min}{7}
\@namedef{S@px.random.errorq75.pct}{17}
\@namedef{S@px.random.errorq75.rate}{0.26}
\@namedef{S@px.random.errorq75.rate35}{0.26}
\@namedef{S@px.random.errorq75.s90}{30.2}
\@namedef{S@px.random.errorq75.s97}{0.6}
\@namedef{S@px.random.errorq75.sd}{2.7}
\@namedef{S@px.random.errorq75.sig}{53}
\@namedef{S@px.random.errorq75.trig}{16}
\@namedef{S@px.random.errorq75.u35k}{21.0}
\@namedef{S@px.random.errorq75.ups}{605}
\@namedef{S@px.random.errorq75.ustopk}{18.6}
\@namedef{S@px.random.errorq90.cov}{0.858}
\@namedef{S@px.random.errorq90.max}{13}
\@namedef{S@px.random.errorq90.mean}{9.8}
\@namedef{S@px.random.errorq90.min}{6}
\@namedef{S@px.random.errorq90.pct}{15}
\@namedef{S@px.random.errorq90.rate}{0.20}
\@namedef{S@px.random.errorq90.rate35}{0.20}
\@namedef{S@px.random.errorq90.s90}{28.4}
\@namedef{S@px.random.errorq90.s97}{1.4}
\@namedef{S@px.random.errorq90.sd}{3.0}
\@namedef{S@px.random.errorq90.sig}{22}
\@namedef{S@px.random.errorq90.trig}{5}
\@namedef{S@px.random.errorq90.u35k}{16.3}
\@namedef{S@px.random.errorq90.ups}{468}
\@namedef{S@px.random.errorq90.ustopk}{14.6}
\@namedef{S@px.random.geom.cov}{0.867}
\@namedef{S@px.random.geom.max}{14}
\@namedef{S@px.random.geom.mean}{10.7}
\@namedef{S@px.random.geom.min}{7}
\@namedef{S@px.random.geom.pct}{17}
\@namedef{S@px.random.geom.rate}{0.26}
\@namedef{S@px.random.geom.rate35}{0.26}
\@namedef{S@px.random.geom.s90}{30.0}
\@namedef{S@px.random.geom.s97}{0.6}
\@namedef{S@px.random.geom.sd}{2.6}
\@namedef{S@px.random.geom.sig}{52}
\@namedef{S@px.random.geom.trig}{15}
\@namedef{S@px.random.geom.u35k}{20.8}
\@namedef{S@px.random.geom.ups}{599}
\@namedef{S@px.random.geom.ustopk}{18.4}
\@namedef{S@px.ratio.rate}{3.9}
\@namedef{S@px.ratio.u35}{3.9}
\@namedef{S@px.ratio.ustop}{3.5}
\@namedef{S@px.seedlist}{23, 29, 37, 43, 53}
\@namedef{S@px.seeds}{5}
\@namedef{S@px.sh.0.02.cov}{0.82}
\@namedef{S@px.sh.0.02.fixed1}{1.6}
\@namedef{S@px.sh.0.02.fixed1.max}{3}
\@namedef{S@px.sh.0.02.fixed1.min}{1}
\@namedef{S@px.sh.0.02.fixed4}{3.2}
\@namedef{S@px.sh.0.02.trig}{72}
\@namedef{S@px.sh.0.05.cov}{0.80}
\@namedef{S@px.sh.0.05.fixed1}{1.6}
\@namedef{S@px.sh.0.05.fixed1.max}{3}
\@namedef{S@px.sh.0.05.fixed1.min}{0}
\@namedef{S@px.sh.0.05.fixed4}{1.6}
\@namedef{S@px.sh.0.05.trig}{82}
\@namedef{S@px.sh.0.1.cov}{0.79}
\@namedef{S@px.sh.0.1.fixed1}{1.6}
\@namedef{S@px.sh.0.1.fixed1.max}{3}
\@namedef{S@px.sh.0.1.fixed1.min}{0}
\@namedef{S@px.sh.0.1.fixed4}{3.0}
\@namedef{S@px.sh.0.1.trig}{84}
\@namedef{S@px.sh.0.25.cov}{0.79}
\@namedef{S@px.sh.0.25.fixed1}{2.2}
\@namedef{S@px.sh.0.25.fixed1.max}{4}
\@namedef{S@px.sh.0.25.fixed1.min}{0}
\@namedef{S@px.sh.0.25.fixed4}{1.8}
\@namedef{S@px.sh.0.25.trig}{87}
\@namedef{S@px.sh.0.85.cov}{0.80}
\@namedef{S@px.sh.0.85.fixed1}{2.6}
\@namedef{S@px.sh.0.85.fixed1.max}{4}
\@namedef{S@px.sh.0.85.fixed1.min}{1}
\@namedef{S@px.sh.0.85.fixed4}{4.2}
\@namedef{S@px.sh.0.85.trig}{86}
\@namedef{S@px.sh.f1max}{2.6}
\@namedef{S@px.sh.f1min}{1.6}
\@namedef{S@px.sh.max}{4.2}
\@namedef{S@px.sh.trigmax}{87}
\@namedef{S@px.sh.trigmin}{72}
\@namedef{S@px.sw.contactq25.ci}{\ensuremath{-}2.8 to +2.5}
\@namedef{S@px.sw.contactq25.crate}{0.81}
\@namedef{S@px.sw.contactq25.d}{\ensuremath{-}0.2}
\@namedef{S@px.sw.contactq25.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.contactq25.holm13}{1.000}
\@namedef{S@px.sw.contactq25.p}{0.900}
\@namedef{S@px.sw.contactq25.pp}{$p=0.900$}
\@namedef{S@px.sw.contactq25.unmatched}{0}
\@namedef{S@px.sw.contactq50.ci}{\ensuremath{-}3.6 to +3.3}
\@namedef{S@px.sw.contactq50.crate}{0.62}
\@namedef{S@px.sw.contactq50.d}{\ensuremath{-}0.1}
\@namedef{S@px.sw.contactq50.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.contactq50.holm13}{1.000}
\@namedef{S@px.sw.contactq50.p}{0.963}
\@namedef{S@px.sw.contactq50.pp}{$p=0.963$}
\@namedef{S@px.sw.contactq50.unmatched}{0}
\@namedef{S@px.sw.contactq75.ci}{\ensuremath{-}3.9 to +2.8}
\@namedef{S@px.sw.contactq75.crate}{0.35}
\@namedef{S@px.sw.contactq75.d}{\ensuremath{-}0.5}
\@namedef{S@px.sw.contactq75.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.contactq75.holm13}{1.000}
\@namedef{S@px.sw.contactq75.p}{0.799}
\@namedef{S@px.sw.contactq75.pp}{$p=0.799$}
\@namedef{S@px.sw.contactq75.unmatched}{0}
\@namedef{S@px.sw.contactq90.ci}{\ensuremath{-}1.9 to +4.6}
\@namedef{S@px.sw.contactq90.crate}{0.22}
\@namedef{S@px.sw.contactq90.d}{+1.2}
\@namedef{S@px.sw.contactq90.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.contactq90.holm13}{1.000}
\@namedef{S@px.sw.contactq90.p}{0.446}
\@namedef{S@px.sw.contactq90.pp}{$p=0.446$}
\@namedef{S@px.sw.contactq90.unmatched}{0}
\@namedef{S@px.sw.disagreementq25.ci}{\ensuremath{-}2.6 to +4.2}
\@namedef{S@px.sw.disagreementq25.crate}{0.46}
\@namedef{S@px.sw.disagreementq25.d}{+0.7}
\@namedef{S@px.sw.disagreementq25.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.disagreementq25.holm13}{1.000}
\@namedef{S@px.sw.disagreementq25.p}{0.681}
\@namedef{S@px.sw.disagreementq25.pp}{$p=0.681$}
\@namedef{S@px.sw.disagreementq25.unmatched}{0}
\@namedef{S@px.sw.disagreementq50.ci}{\ensuremath{-}1.4 to +5.1}
\@namedef{S@px.sw.disagreementq50.crate}{0.34}
\@namedef{S@px.sw.disagreementq50.d}{+1.7}
\@namedef{S@px.sw.disagreementq50.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.disagreementq50.holm13}{1.000}
\@namedef{S@px.sw.disagreementq50.p}{0.288}
\@namedef{S@px.sw.disagreementq50.pp}{$p=0.288$}
\@namedef{S@px.sw.disagreementq50.unmatched}{0}
\@namedef{S@px.sw.disagreementq75.ci}{\ensuremath{-}0.9 to +4.8}
\@namedef{S@px.sw.disagreementq75.crate}{0.22}
\@namedef{S@px.sw.disagreementq75.d}{+1.8}
\@namedef{S@px.sw.disagreementq75.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.disagreementq75.holm13}{1.000}
\@namedef{S@px.sw.disagreementq75.p}{0.206}
\@namedef{S@px.sw.disagreementq75.pp}{$p=0.206$}
\@namedef{S@px.sw.disagreementq75.unmatched}{0}
\@namedef{S@px.sw.disagreementq90.ci}{\ensuremath{-}1.3 to +2.4}
\@namedef{S@px.sw.disagreementq90.crate}{0.19}
\@namedef{S@px.sw.disagreementq90.d}{+0.3}
\@namedef{S@px.sw.disagreementq90.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.disagreementq90.holm13}{1.000}
\@namedef{S@px.sw.disagreementq90.p}{0.754}
\@namedef{S@px.sw.disagreementq90.pp}{$p=0.754$}
\@namedef{S@px.sw.disagreementq90.unmatched}{0}
\@namedef{S@px.sw.dmax}{+1.8}
\@namedef{S@px.sw.dmin}{\ensuremath{-}0.6}
\@namedef{S@px.sw.errorq25.ci}{\ensuremath{-}3.2 to +4.9}
\@namedef{S@px.sw.errorq25.crate}{0.59}
\@namedef{S@px.sw.errorq25.d}{+0.8}
\@namedef{S@px.sw.errorq25.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.errorq25.holm13}{1.000}
\@namedef{S@px.sw.errorq25.p}{0.695}
\@namedef{S@px.sw.errorq25.pp}{$p=0.695$}
\@namedef{S@px.sw.errorq25.unmatched}{0}
\@namedef{S@px.sw.errorq50.ci}{\ensuremath{-}2.2 to +4.8}
\@namedef{S@px.sw.errorq50.crate}{0.38}
\@namedef{S@px.sw.errorq50.d}{+1.2}
\@namedef{S@px.sw.errorq50.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.errorq50.holm13}{1.000}
\@namedef{S@px.sw.errorq50.p}{0.446}
\@namedef{S@px.sw.errorq50.pp}{$p=0.446$}
\@namedef{S@px.sw.errorq50.unmatched}{0}
\@namedef{S@px.sw.errorq75.ci}{\ensuremath{-}2.5 to +2.8}
\@namedef{S@px.sw.errorq75.crate}{0.26}
\@namedef{S@px.sw.errorq75.d}{+0.1}
\@namedef{S@px.sw.errorq75.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.errorq75.holm13}{1.000}
\@namedef{S@px.sw.errorq75.p}{0.984}
\@namedef{S@px.sw.errorq75.pp}{$p=0.984$}
\@namedef{S@px.sw.errorq75.unmatched}{0}
\@namedef{S@px.sw.errorq90.ci}{\ensuremath{-}2.0 to +0.9}
\@namedef{S@px.sw.errorq90.crate}{0.20}
\@namedef{S@px.sw.errorq90.d}{\ensuremath{-}0.6}
\@namedef{S@px.sw.errorq90.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.errorq90.holm13}{1.000}
\@namedef{S@px.sw.errorq90.p}{0.384}
\@namedef{S@px.sw.errorq90.pp}{$p=0.384$}
\@namedef{S@px.sw.errorq90.unmatched}{0}
\@namedef{S@px.sw.geom.ci}{\ensuremath{-}2.6 to +4.7}
\@namedef{S@px.sw.geom.crate}{0.26}
\@namedef{S@px.sw.geom.d}{+1.1}
\@namedef{S@px.sw.geom.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@px.sw.geom.holm13}{1.000}
\@namedef{S@px.sw.geom.p}{0.542}
\@namedef{S@px.sw.geom.pp}{$p=0.542$}
\@namedef{S@px.sw.geom.unmatched}{0}
\@namedef{S@px.sw.hi}{+5.1}
\@namedef{S@px.sw.lo}{\ensuremath{-}3.9}
\@namedef{S@px.sw.ndpos}{9}
\@namedef{S@px.sw.nholm}{0}
\@namedef{S@px.sw.nneg}{0}
\@namedef{S@px.sw.npos}{0}
\@namedef{S@px.sw.nsig}{0}
\@namedef{S@px.swc.contactq25.ci}{\ensuremath{-}0.8 to +3.3}
\@namedef{S@px.swc.contactq25.d}{+1.2}
\@namedef{S@px.swc.contactq25.p}{0.251}
\@namedef{S@px.swc.contactq25.pp}{$p=0.251$}
\@namedef{S@px.swc.contactq50.ci}{\ensuremath{-}2.7 to +5.0}
\@namedef{S@px.swc.contactq50.d}{+1.2}
\@namedef{S@px.swc.contactq50.p}{0.558}
\@namedef{S@px.swc.contactq50.pp}{$p=0.558$}
\@namedef{S@px.swc.contactq75.ci}{\ensuremath{-}5.1 to +4.1}
\@namedef{S@px.swc.contactq75.d}{\ensuremath{-}0.3}
\@namedef{S@px.swc.contactq75.p}{0.931}
\@namedef{S@px.swc.contactq75.pp}{$p=0.931$}
\@namedef{S@px.swc.contactq90.ci}{\ensuremath{-}3.5 to +4.7}
\@namedef{S@px.swc.contactq90.d}{+0.6}
\@namedef{S@px.swc.contactq90.p}{0.750}
\@namedef{S@px.swc.contactq90.pp}{$p=0.750$}
\@namedef{S@px.swc.disagreementq25.ci}{\ensuremath{-}3.0 to +5.9}
\@namedef{S@px.swc.disagreementq25.d}{+1.5}
\@namedef{S@px.swc.disagreementq25.p}{0.524}
\@namedef{S@px.swc.disagreementq25.pp}{$p=0.524$}
\@namedef{S@px.swc.disagreementq50.ci}{\ensuremath{-}3.1 to +6.0}
\@namedef{S@px.swc.disagreementq50.d}{+1.3}
\@namedef{S@px.swc.disagreementq50.p}{0.517}
\@namedef{S@px.swc.disagreementq50.pp}{$p=0.517$}
\@namedef{S@px.swc.disagreementq75.ci}{\ensuremath{-}2.2 to +4.9}
\@namedef{S@px.swc.disagreementq75.d}{+1.3}
\@namedef{S@px.swc.disagreementq75.p}{0.465}
\@namedef{S@px.swc.disagreementq75.pp}{$p=0.465$}
\@namedef{S@px.swc.disagreementq90.ci}{\ensuremath{-}1.5 to +2.6}
\@namedef{S@px.swc.disagreementq90.d}{+0.3}
\@namedef{S@px.swc.disagreementq90.p}{0.784}
\@namedef{S@px.swc.disagreementq90.pp}{$p=0.784$}
\@namedef{S@px.swc.errorq25.ci}{\ensuremath{-}3.2 to +6.9}
\@namedef{S@px.swc.errorq25.d}{+2.0}
\@namedef{S@px.swc.errorq25.p}{0.407}
\@namedef{S@px.swc.errorq25.pp}{$p=0.407$}
\@namedef{S@px.swc.errorq50.ci}{\ensuremath{-}3.5 to +6.0}
\@namedef{S@px.swc.errorq50.d}{+1.3}
\@namedef{S@px.swc.errorq50.p}{0.545}
\@namedef{S@px.swc.errorq50.pp}{$p=0.545$}
\@namedef{S@px.swc.errorq75.ci}{\ensuremath{-}3.6 to +3.9}
\@namedef{S@px.swc.errorq75.d}{+0.1}
\@namedef{S@px.swc.errorq75.p}{0.962}
\@namedef{S@px.swc.errorq75.pp}{$p=0.962$}
\@namedef{S@px.swc.errorq90.ci}{\ensuremath{-}2.5 to +1.2}
\@namedef{S@px.swc.errorq90.d}{\ensuremath{-}0.7}
\@namedef{S@px.swc.errorq90.p}{0.444}
\@namedef{S@px.swc.errorq90.pp}{$p=0.444$}
\@namedef{S@px.swc.geom.ci}{\ensuremath{-}3.2 to +5.7}
\@namedef{S@px.swc.geom.d}{+1.2}
\@namedef{S@px.swc.geom.p}{0.582}
\@namedef{S@px.swc.geom.pp}{$p=0.582$}
\@namedef{S@px.swc.nsig}{0}
\@namedef{S@px.swcov.contactq25.ci}{\ensuremath{-}0.001 to +0.008}
\@namedef{S@px.swcov.contactq25.d}{+0.003}
\@namedef{S@px.swcov.contactq25.p}{0.122}
\@namedef{S@px.swcov.contactq25.pp}{$p=0.122$}
\@namedef{S@px.swcov.contactq50.ci}{+0.000 to +0.016}
\@namedef{S@px.swcov.contactq50.d}{+0.008}
\@namedef{S@px.swcov.contactq50.p}{0.044}
\@namedef{S@px.swcov.contactq50.pp}{$p=0.044$}
\@namedef{S@px.swcov.contactq75.ci}{\ensuremath{-}0.007 to +0.014}
\@namedef{S@px.swcov.contactq75.d}{+0.003}
\@namedef{S@px.swcov.contactq75.p}{0.545}
\@namedef{S@px.swcov.contactq75.pp}{$p=0.545$}
\@namedef{S@px.swcov.contactq90.ci}{\ensuremath{-}0.001 to +0.021}
\@namedef{S@px.swcov.contactq90.d}{+0.009}
\@namedef{S@px.swcov.contactq90.p}{0.084}
\@namedef{S@px.swcov.contactq90.pp}{$p=0.084$}
\@namedef{S@px.swcov.disagreementq25.ci}{+0.007 to +0.027}
\@namedef{S@px.swcov.disagreementq25.d}{+0.016}
\@namedef{S@px.swcov.disagreementq25.p}{0.001}
\@namedef{S@px.swcov.disagreementq25.pp}{$p=0.001$}
\@namedef{S@px.swcov.disagreementq50.ci}{+0.000 to +0.023}
\@namedef{S@px.swcov.disagreementq50.d}{+0.011}
\@namedef{S@px.swcov.disagreementq50.p}{0.046}
\@namedef{S@px.swcov.disagreementq50.pp}{$p=0.046$}
\@namedef{S@px.swcov.disagreementq75.ci}{+0.001 to +0.026}
\@namedef{S@px.swcov.disagreementq75.d}{+0.013}
\@namedef{S@px.swcov.disagreementq75.p}{0.037}
\@namedef{S@px.swcov.disagreementq75.pp}{$p=0.037$}
\@namedef{S@px.swcov.disagreementq90.ci}{\ensuremath{-}0.005 to +0.019}
\@namedef{S@px.swcov.disagreementq90.d}{+0.004}
\@namedef{S@px.swcov.disagreementq90.p}{0.518}
\@namedef{S@px.swcov.disagreementq90.pp}{$p=0.518$}
\@namedef{S@px.swcov.errorq25.ci}{+0.003 to +0.019}
\@namedef{S@px.swcov.errorq25.d}{+0.011}
\@namedef{S@px.swcov.errorq25.p}{0.010}
\@namedef{S@px.swcov.errorq25.pp}{$p=0.010$}
\@namedef{S@px.swcov.errorq50.ci}{+0.001 to +0.022}
\@namedef{S@px.swcov.errorq50.d}{+0.011}
\@namedef{S@px.swcov.errorq50.p}{0.025}
\@namedef{S@px.swcov.errorq50.pp}{$p=0.025$}
\@namedef{S@px.swcov.errorq75.ci}{\ensuremath{-}0.004 to +0.017}
\@namedef{S@px.swcov.errorq75.d}{+0.006}
\@namedef{S@px.swcov.errorq75.p}{0.235}
\@namedef{S@px.swcov.errorq75.pp}{$p=0.235$}
\@namedef{S@px.swcov.errorq90.ci}{\ensuremath{-}0.007 to +0.011}
\@namedef{S@px.swcov.errorq90.d}{+0.002}
\@namedef{S@px.swcov.errorq90.p}{0.731}
\@namedef{S@px.swcov.errorq90.pp}{$p=0.731$}
\@namedef{S@px.swcov.geom.ci}{+0.008 to +0.037}
\@namedef{S@px.swcov.geom.d}{+0.021}
\@namedef{S@px.swcov.geom.p}{<0.001}
\@namedef{S@px.swcov.geom.pp}{$p<0.001$}
\@namedef{S@px.swcov.ndpos}{13}
\@namedef{S@px.swcov.nholm}{2}
\@namedef{S@px.swcov.nneg}{0}
\@namedef{S@px.swcov.npos}{7}
\@namedef{S@px.swk.contactq25.ci}{\ensuremath{-}0.7 to +3.3}
\@namedef{S@px.swk.contactq25.d}{+1.3}
\@namedef{S@px.swk.contactq25.p}{0.184}
\@namedef{S@px.swk.contactq25.pp}{$p=0.184$}
\@namedef{S@px.swk.contactq50.ci}{\ensuremath{-}1.5 to +3.8}
\@namedef{S@px.swk.contactq50.d}{+1.3}
\@namedef{S@px.swk.contactq50.p}{0.313}
\@namedef{S@px.swk.contactq50.pp}{$p=0.313$}
\@namedef{S@px.swk.contactq75.ci}{\ensuremath{-}2.9 to +3.1}
\@namedef{S@px.swk.contactq75.d}{+0.2}
\@namedef{S@px.swk.contactq75.p}{0.862}
\@namedef{S@px.swk.contactq75.pp}{$p=0.862$}
\@namedef{S@px.swk.contactq90.ci}{\ensuremath{-}2.8 to +1.3}
\@namedef{S@px.swk.contactq90.d}{\ensuremath{-}0.6}
\@namedef{S@px.swk.contactq90.p}{0.602}
\@namedef{S@px.swk.contactq90.pp}{$p=0.602$}
\@namedef{S@px.swk.disagreementq25.ci}{\ensuremath{-}1.9 to +3.3}
\@namedef{S@px.swk.disagreementq25.d}{+0.8}
\@namedef{S@px.swk.disagreementq25.p}{0.519}
\@namedef{S@px.swk.disagreementq25.pp}{$p=0.519$}
\@namedef{S@px.swk.disagreementq50.ci}{\ensuremath{-}3.5 to +2.5}
\@namedef{S@px.swk.disagreementq50.d}{\ensuremath{-}0.4}
\@namedef{S@px.swk.disagreementq50.p}{0.806}
\@namedef{S@px.swk.disagreementq50.pp}{$p=0.806$}
\@namedef{S@px.swk.disagreementq75.ci}{\ensuremath{-}2.6 to +1.4}
\@namedef{S@px.swk.disagreementq75.d}{\ensuremath{-}0.5}
\@namedef{S@px.swk.disagreementq75.p}{0.643}
\@namedef{S@px.swk.disagreementq75.pp}{$p=0.643$}
\@namedef{S@px.swk.disagreementq90.ci}{\ensuremath{-}1.0 to +0.8}
\@namedef{S@px.swk.disagreementq90.d}{\ensuremath{-}0.0}
\@namedef{S@px.swk.disagreementq90.p}{0.965}
\@namedef{S@px.swk.disagreementq90.pp}{$p=0.965$}
\@namedef{S@px.swk.dmax}{+1.3}
\@namedef{S@px.swk.dmin}{\ensuremath{-}0.6}
\@namedef{S@px.swk.errorq25.ci}{\ensuremath{-}1.7 to +4.0}
\@namedef{S@px.swk.errorq25.d}{+1.3}
\@namedef{S@px.swk.errorq25.p}{0.357}
\@namedef{S@px.swk.errorq25.pp}{$p=0.357$}
\@namedef{S@px.swk.errorq50.ci}{\ensuremath{-}3.2 to +3.0}
\@namedef{S@px.swk.errorq50.d}{+0.1}
\@namedef{S@px.swk.errorq50.p}{0.910}
\@namedef{S@px.swk.errorq50.pp}{$p=0.910$}
\@namedef{S@px.swk.errorq75.ci}{\ensuremath{-}2.6 to +2.9}
\@namedef{S@px.swk.errorq75.d}{+0.2}
\@namedef{S@px.swk.errorq75.p}{0.897}
\@namedef{S@px.swk.errorq75.pp}{$p=0.897$}
\@namedef{S@px.swk.errorq90.ci}{\ensuremath{-}1.4 to +1.2}
\@namedef{S@px.swk.errorq90.d}{\ensuremath{-}0.1}
\@namedef{S@px.swk.errorq90.p}{0.967}
\@namedef{S@px.swk.errorq90.pp}{$p=0.967$}
\@namedef{S@px.swk.geom.ci}{\ensuremath{-}2.8 to +3.1}
\@namedef{S@px.swk.geom.d}{+0.2}
\@namedef{S@px.swk.geom.p}{0.891}
\@namedef{S@px.swk.geom.pp}{$p=0.891$}
\@namedef{S@px.swk.nsig}{0}
\@namedef{S@px.tasks}{64}
\@namedef{S@px.thr.contact.q25}{below 0.001}
\@namedef{S@px.thr.contact.q50}{below 0.001}
\@namedef{S@px.thr.contact.q75}{0.08}
\@namedef{S@px.thr.contact.q90}{0.60}
\@namedef{S@px.thr.disagreement.q25}{0.37}
\@namedef{S@px.thr.disagreement.q50}{0.54}
\@namedef{S@px.thr.disagreement.q75}{0.78}
\@namedef{S@px.thr.disagreement.q90}{1.15}
\@namedef{S@px.thr.error.q25}{1.35}
\@namedef{S@px.thr.error.q50}{2.07}
\@namedef{S@px.thr.error.q75}{3.15}
\@namedef{S@px.thr.error.q90}{4.75}
\@namedef{S@px.unmatched.arms}{0}
\@namedef{S@px.unmatched.total}{0}
\@namedef{S@s14.contact.cal}{28}
\@namedef{S@s14.contact.cal23}{36}
\@namedef{S@s14.contact.higher}{8}
\@namedef{S@s14.contact.test}{23}
\@namedef{S@s14.contact.test23}{20}
\@namedef{S@s14.error.cal}{13}
\@namedef{S@s14.error.cal23}{12}
\@namedef{S@s14.error.higher}{9}
\@namedef{S@s14.error.test}{10}
\@namedef{S@s14.error.test23}{9}
\@namedef{S@s14.n}{10}
\@namedef{S@st.F.ci}{+11.6 to +22.2}
\@namedef{S@st.F.d}{+16.9}
\@namedef{S@st.F.hh}{$p_{\mathrm{Holm}}<0.001$}
\@namedef{S@st.F.holm}{<0.001}
\@namedef{S@st.F.p}{<0.001}
\@namedef{S@st.F.pp}{$p<0.001$}
\@namedef{S@st.Fcov.ci}{+0.023 to +0.044}
\@namedef{S@st.Fcov.d}{+0.033}
\@namedef{S@st.Fcov.hh}{$p_{\mathrm{Holm}}<0.001$}
\@namedef{S@st.Fcov.holm}{<0.001}
\@namedef{S@st.Fcov.p}{<0.001}
\@namedef{S@st.Fcov.pp}{$p<0.001$}
\@namedef{S@st.Fs90.ci}{+4.9 to +14.3}
\@namedef{S@st.Fs90.d}{+9.5}
\@namedef{S@st.Fs90.p}{<0.001}
\@namedef{S@st.Fs90.pp}{$p<0.001$}
\@namedef{S@st.Fs97.ci}{+8.7 to +18.3}
\@namedef{S@st.Fs97.d}{+13.4}
\@namedef{S@st.Fs97.p}{<0.001}
\@namedef{S@st.Fs97.pp}{$p<0.001$}
\@namedef{S@st.T-contact.ci}{\ensuremath{-}5.7 to +2.3}
\@namedef{S@st.T-contact.d}{\ensuremath{-}1.6}
\@namedef{S@st.T-contact.hh}{$p_{\mathrm{Holm}}=0.746$}
\@namedef{S@st.T-contact.holm}{0.746}
\@namedef{S@st.T-contact.p}{0.416}
\@namedef{S@st.T-contact.pp}{$p=0.416$}
\@namedef{S@st.T-contactcov.ci}{\ensuremath{-}0.004 to +0.013}
\@namedef{S@st.T-contactcov.d}{+0.004}
\@namedef{S@st.T-contactcov.hh}{$p_{\mathrm{Holm}}=0.371$}
\@namedef{S@st.T-contactcov.holm}{0.371}
\@namedef{S@st.T-contactcov.p}{0.371}
\@namedef{S@st.T-contactcov.pp}{$p=0.371$}
\@namedef{S@st.T-disagreement.ci}{\ensuremath{-}1.3 to +4.5}
\@namedef{S@st.T-disagreement.d}{+1.6}
\@namedef{S@st.T-disagreement.hh}{$p_{\mathrm{Holm}}=0.746$}
\@namedef{S@st.T-disagreement.holm}{0.746}
\@namedef{S@st.T-disagreement.p}{0.282}
\@namedef{S@st.T-disagreement.pp}{$p=0.282$}
\@namedef{S@st.T-disagreementcov.ci}{+0.005 to +0.021}
\@namedef{S@st.T-disagreementcov.d}{+0.013}
\@namedef{S@st.T-disagreementcov.hh}{$p_{\mathrm{Holm}}<0.001$}
\@namedef{S@st.T-disagreementcov.holm}{<0.001}
\@namedef{S@st.T-disagreementcov.p}{<0.001}
\@namedef{S@st.T-disagreementcov.pp}{$p<0.001$}
\@namedef{S@st.T-error.ci}{\ensuremath{-}1.1 to +5.5}
\@namedef{S@st.T-error.d}{+2.0}
\@namedef{S@st.T-error.hh}{$p_{\mathrm{Holm}}=0.746$}
\@namedef{S@st.T-error.holm}{0.746}
\@namedef{S@st.T-error.p}{0.223}
\@namedef{S@st.T-error.pp}{$p=0.223$}
\@namedef{S@st.T-errorcov.ci}{+0.005 to +0.019}
\@namedef{S@st.T-errorcov.d}{+0.012}
\@namedef{S@st.T-errorcov.hh}{$p_{\mathrm{Holm}}<0.001$}
\@namedef{S@st.T-errorcov.holm}{<0.001}
\@namedef{S@st.T-errorcov.p}{<0.001}
\@namedef{S@st.T-errorcov.pp}{$p<0.001$}
\@namedef{S@st.T-geom.ci}{\ensuremath{-}1.3 to +6.8}
\@namedef{S@st.T-geom.d}{+2.7}
\@namedef{S@st.T-geom.hh}{$p_{\mathrm{Holm}}=0.746$}
\@namedef{S@st.T-geom.holm}{0.746}
\@namedef{S@st.T-geom.p}{0.187}
\@namedef{S@st.T-geom.pp}{$p=0.187$}
\@namedef{S@st.T-geomcov.ci}{+0.008 to +0.023}
\@namedef{S@st.T-geomcov.d}{+0.015}
\@namedef{S@st.T-geomcov.hh}{$p_{\mathrm{Holm}}<0.001$}
\@namedef{S@st.T-geomcov.holm}{<0.001}
\@namedef{S@st.T-geomcov.p}{<0.001}
\@namedef{S@st.T-geomcov.pp}{$p<0.001$}
\@namedef{S@st.cells}{640}
\@namedef{S@st.contactq25.cov}{0.936}
\@namedef{S@st.contactq25.max}{37}
\@namedef{S@st.contactq25.mean}{33.4}
\@namedef{S@st.contactq25.min}{26}
\@namedef{S@st.contactq25.pct}{52}
\@namedef{S@st.contactq25.rate}{0.82}
\@namedef{S@st.contactq25.rate35}{0.74}
\@namedef{S@st.contactq25.s90}{50.7}
\@namedef{S@st.contactq25.s97}{21.3}
\@namedef{S@st.contactq25.sd}{3.4}
\@namedef{S@st.contactq25.sig}{91}
\@namedef{S@st.contactq25.trig}{80}
\@namedef{S@st.contactq25.u35k}{59.5}
\@namedef{S@st.contactq25.ups}{1885}
\@namedef{S@st.contactq25.ustopk}{40.1}
\@namedef{S@st.contactq50.cov}{0.935}
\@namedef{S@st.contactq50.max}{37}
\@namedef{S@st.contactq50.mean}{33.0}
\@namedef{S@st.contactq50.min}{29}
\@namedef{S@st.contactq50.pct}{52}
\@namedef{S@st.contactq50.rate}{0.63}
\@namedef{S@st.contactq50.rate35}{0.52}
\@namedef{S@st.contactq50.s90}{50.5}
\@namedef{S@st.contactq50.s97}{20.6}
\@namedef{S@st.contactq50.sd}{3.0}
\@namedef{S@st.contactq50.sig}{84}
\@namedef{S@st.contactq50.trig}{58}
\@namedef{S@st.contactq50.u35k}{42.3}
\@namedef{S@st.contactq50.ups}{1445}
\@namedef{S@st.contactq50.ustopk}{31.3}
\@namedef{S@st.contactq75.cov}{0.913}
\@namedef{S@st.contactq75.max}{23}
\@namedef{S@st.contactq75.mean}{19.7}
\@namedef{S@st.contactq75.min}{16}
\@namedef{S@st.contactq75.pct}{31}
\@namedef{S@st.contactq75.rate}{0.34}
\@namedef{S@st.contactq75.rate35}{0.32}
\@namedef{S@st.contactq75.s90}{42.7}
\@namedef{S@st.contactq75.s97}{9.2}
\@namedef{S@st.contactq75.sd}{2.4}
\@namedef{S@st.contactq75.sig}{58}
\@namedef{S@st.contactq75.trig}{23}
\@namedef{S@st.contactq75.u35k}{25.4}
\@namedef{S@st.contactq75.ups}{781}
\@namedef{S@st.contactq75.ustopk}{21.3}
\@namedef{S@st.contactq90.cov}{0.900}
\@namedef{S@st.contactq90.max}{20}
\@namedef{S@st.contactq90.mean}{16.6}
\@namedef{S@st.contactq90.min}{12}
\@namedef{S@st.contactq90.pct}{26}
\@namedef{S@st.contactq90.rate}{0.23}
\@namedef{S@st.contactq90.rate35}{0.22}
\@namedef{S@st.contactq90.s90}{39.0}
\@namedef{S@st.contactq90.s97}{7.5}
\@namedef{S@st.contactq90.sd}{2.4}
\@namedef{S@st.contactq90.sig}{29}
\@namedef{S@st.contactq90.trig}{8}
\@namedef{S@st.contactq90.u35k}{17.9}
\@namedef{S@st.contactq90.ups}{532}
\@namedef{S@st.contactq90.ustopk}{15.3}
\@namedef{S@st.disagreementq25.cov}{0.931}
\@namedef{S@st.disagreementq25.max}{35}
\@namedef{S@st.disagreementq25.mean}{29.5}
\@namedef{S@st.disagreementq25.min}{25}
\@namedef{S@st.disagreementq25.pct}{46}
\@namedef{S@st.disagreementq25.rate}{0.48}
\@namedef{S@st.disagreementq25.rate35}{0.43}
\@namedef{S@st.disagreementq25.s90}{50.0}
\@namedef{S@st.disagreementq25.s97}{17.7}
\@namedef{S@st.disagreementq25.sd}{3.2}
\@namedef{S@st.disagreementq25.sig}{84}
\@namedef{S@st.disagreementq25.trig}{44}
\@namedef{S@st.disagreementq25.u35k}{34.7}
\@namedef{S@st.disagreementq25.ups}{1108}
\@namedef{S@st.disagreementq25.ustopk}{25.6}
\@namedef{S@st.disagreementq50.cov}{0.921}
\@namedef{S@st.disagreementq50.max}{30}
\@namedef{S@st.disagreementq50.mean}{23.6}
\@namedef{S@st.disagreementq50.min}{20}
\@namedef{S@st.disagreementq50.pct}{37}
\@namedef{S@st.disagreementq50.rate}{0.33}
\@namedef{S@st.disagreementq50.rate35}{0.31}
\@namedef{S@st.disagreementq50.s90}{46.6}
\@namedef{S@st.disagreementq50.s97}{13.2}
\@namedef{S@st.disagreementq50.sd}{3.7}
\@namedef{S@st.disagreementq50.sig}{67}
\@namedef{S@st.disagreementq50.trig}{25}
\@namedef{S@st.disagreementq50.u35k}{24.7}
\@namedef{S@st.disagreementq50.ups}{772}
\@namedef{S@st.disagreementq50.ustopk}{19.7}
\@namedef{S@st.disagreementq75.cov}{0.908}
\@namedef{S@st.disagreementq75.max}{23}
\@namedef{S@st.disagreementq75.mean}{17.7}
\@namedef{S@st.disagreementq75.min}{11}
\@namedef{S@st.disagreementq75.pct}{28}
\@namedef{S@st.disagreementq75.rate}{0.23}
\@namedef{S@st.disagreementq75.rate35}{0.22}
\@namedef{S@st.disagreementq75.s90}{42.0}
\@namedef{S@st.disagreementq75.s97}{7.9}
\@namedef{S@st.disagreementq75.sd}{3.1}
\@namedef{S@st.disagreementq75.sig}{37}
\@namedef{S@st.disagreementq75.trig}{10}
\@namedef{S@st.disagreementq75.u35k}{18.0}
\@namedef{S@st.disagreementq75.ups}{541}
\@namedef{S@st.disagreementq75.ustopk}{15.3}
\@namedef{S@st.disagreementq90.cov}{0.895}
\@namedef{S@st.disagreementq90.max}{20}
\@namedef{S@st.disagreementq90.mean}{14.8}
\@namedef{S@st.disagreementq90.min}{11}
\@namedef{S@st.disagreementq90.pct}{23}
\@namedef{S@st.disagreementq90.rate}{0.19}
\@namedef{S@st.disagreementq90.rate35}{0.19}
\@namedef{S@st.disagreementq90.s90}{37.3}
\@namedef{S@st.disagreementq90.s97}{5.6}
\@namedef{S@st.disagreementq90.sd}{2.6}
\@namedef{S@st.disagreementq90.sig}{15}
\@namedef{S@st.disagreementq90.trig}{4}
\@namedef{S@st.disagreementq90.u35k}{15.2}
\@namedef{S@st.disagreementq90.ups}{449}
\@namedef{S@st.disagreementq90.ustopk}{13.4}
\@namedef{S@st.eq.1152.1}{25.5}
\@namedef{S@st.eq.1152.2}{29.4}
\@namedef{S@st.eq.1152.4}{23.6}
\@namedef{S@st.eq.2304.1}{33.7}
\@namedef{S@st.eq.2304.2}{26.9}
\@namedef{S@st.eq.2304.4}{23.5}
\@namedef{S@st.eq.576.1}{12.5}
\@namedef{S@st.eq.576.2}{16.2}
\@namedef{S@st.eq.576.4}{16.8}
\@namedef{S@st.eq.r4}{31.4}
\@namedef{S@st.eq.r8}{34.2}
\@namedef{S@st.errorq25.cov}{0.933}
\@namedef{S@st.errorq25.max}{35}
\@namedef{S@st.errorq25.mean}{31.5}
\@namedef{S@st.errorq25.min}{26}
\@namedef{S@st.errorq25.pct}{49}
\@namedef{S@st.errorq25.rate}{0.56}
\@namedef{S@st.errorq25.rate35}{0.48}
\@namedef{S@st.errorq25.s90}{49.8}
\@namedef{S@st.errorq25.s97}{18.4}
\@namedef{S@st.errorq25.sd}{2.7}
\@namedef{S@st.errorq25.sig}{89}
\@namedef{S@st.errorq25.trig}{53}
\@namedef{S@st.errorq25.u35k}{38.9}
\@namedef{S@st.errorq25.ups}{1298}
\@namedef{S@st.errorq25.ustopk}{28.7}
\@namedef{S@st.errorq50.cov}{0.927}
\@namedef{S@st.errorq50.max}{33}
\@namedef{S@st.errorq50.mean}{27.1}
\@namedef{S@st.errorq50.min}{24}
\@namedef{S@st.errorq50.pct}{42}
\@namedef{S@st.errorq50.rate}{0.36}
\@namedef{S@st.errorq50.rate35}{0.32}
\@namedef{S@st.errorq50.s90}{49.1}
\@namedef{S@st.errorq50.s97}{15.6}
\@namedef{S@st.errorq50.sd}{2.6}
\@namedef{S@st.errorq50.sig}{73}
\@namedef{S@st.errorq50.trig}{29}
\@namedef{S@st.errorq50.u35k}{25.6}
\@namedef{S@st.errorq50.ups}{837}
\@namedef{S@st.errorq50.ustopk}{20.1}
\@namedef{S@st.errorq75.cov}{0.907}
\@namedef{S@st.errorq75.max}{23}
\@namedef{S@st.errorq75.mean}{18.0}
\@namedef{S@st.errorq75.min}{15}
\@namedef{S@st.errorq75.pct}{28}
\@namedef{S@st.errorq75.rate}{0.23}
\@namedef{S@st.errorq75.rate35}{0.22}
\@namedef{S@st.errorq75.s90}{41.1}
\@namedef{S@st.errorq75.s97}{8.4}
\@namedef{S@st.errorq75.sd}{3.3}
\@namedef{S@st.errorq75.sig}{37}
\@namedef{S@st.errorq75.trig}{10}
\@namedef{S@st.errorq75.u35k}{17.8}
\@namedef{S@st.errorq75.ups}{537}
\@namedef{S@st.errorq75.ustopk}{15.0}
\@namedef{S@st.errorq90.cov}{0.891}
\@namedef{S@st.errorq90.max}{17}
\@namedef{S@st.errorq90.mean}{13.7}
\@namedef{S@st.errorq90.min}{11}
\@namedef{S@st.errorq90.pct}{21}
\@namedef{S@st.errorq90.rate}{0.19}
\@namedef{S@st.errorq90.rate35}{0.19}
\@namedef{S@st.errorq90.s90}{35.7}
\@namedef{S@st.errorq90.s97}{5.5}
\@namedef{S@st.errorq90.sd}{2.0}
\@namedef{S@st.errorq90.sig}{13}
\@namedef{S@st.errorq90.trig}{3}
\@namedef{S@st.errorq90.u35k}{15.0}
\@namedef{S@st.errorq90.ups}{441}
\@namedef{S@st.errorq90.ustopk}{13.2}
\@namedef{S@st.f1gtf4}{10}
\@namedef{S@st.fixed1.cov}{0.936}
\@namedef{S@st.fixed1.max}{38}
\@namedef{S@st.fixed1.mean}{33.7}
\@namedef{S@st.fixed1.min}{28}
\@namedef{S@st.fixed1.pct}{53}
\@namedef{S@st.fixed1.rate}{1.00}
\@namedef{S@st.fixed1.rate35}{1.00}
\@namedef{S@st.fixed1.s23}{28}
\@namedef{S@st.fixed1.s90}{50.9}
\@namedef{S@st.fixed1.s97}{21.3}
\@namedef{S@st.fixed1.sd}{2.9}
\@namedef{S@st.fixed1.sig}{0}
\@namedef{S@st.fixed1.trig}{0}
\@namedef{S@st.fixed1.u35k}{80.6}
\@namedef{S@st.fixed1.ups}{2304}
\@namedef{S@st.fixed1.ustopk}{48.7}
\@namedef{S@st.fixed1K16i2.cov}{0.923}
\@namedef{S@st.fixed1K16i2.max}{29}
\@namedef{S@st.fixed1K16i2.mean}{25.5}
\@namedef{S@st.fixed1K16i2.min}{21}
\@namedef{S@st.fixed1K16i2.pct}{40}
\@namedef{S@st.fixed1K16i2.rate}{1.00}
\@namedef{S@st.fixed1K16i2.rate35}{1.00}
\@namedef{S@st.fixed1K16i2.s90}{49.2}
\@namedef{S@st.fixed1K16i2.s97}{12.6}
\@namedef{S@st.fixed1K16i2.sd}{2.4}
\@namedef{S@st.fixed1K16i2.sig}{0}
\@namedef{S@st.fixed1K16i2.trig}{0}
\@namedef{S@st.fixed1K16i2.u35k}{40.3}
\@namedef{S@st.fixed1K16i2.ups}{1152}
\@namedef{S@st.fixed1K16i2.ustopk}{29.4}
\@namedef{S@st.fixed1K8i2.cov}{0.854}
\@namedef{S@st.fixed1K8i2.max}{15}
\@namedef{S@st.fixed1K8i2.mean}{12.5}
\@namedef{S@st.fixed1K8i2.min}{7}
\@namedef{S@st.fixed1K8i2.pct}{20}
\@namedef{S@st.fixed1K8i2.rate}{1.00}
\@namedef{S@st.fixed1K8i2.rate35}{1.00}
\@namedef{S@st.fixed1K8i2.s90}{33.7}
\@namedef{S@st.fixed1K8i2.s97}{5.4}
\@namedef{S@st.fixed1K8i2.sd}{2.4}
\@namedef{S@st.fixed1K8i2.sig}{0}
\@namedef{S@st.fixed1K8i2.trig}{0}
\@namedef{S@st.fixed1K8i2.u35k}{20.2}
\@namedef{S@st.fixed1K8i2.ups}{576}
\@namedef{S@st.fixed1K8i2.ustopk}{17.6}
\@namedef{S@st.fixed2.cov}{0.928}
\@namedef{S@st.fixed2.max}{36}
\@namedef{S@st.fixed2.mean}{29.4}
\@namedef{S@st.fixed2.min}{23}
\@namedef{S@st.fixed2.pct}{46}
\@namedef{S@st.fixed2.rate}{0.52}
\@namedef{S@st.fixed2.rate35}{0.51}
\@namedef{S@st.fixed2.s23}{27}
\@namedef{S@st.fixed2.s90}{47.9}
\@namedef{S@st.fixed2.s97}{15.8}
\@namedef{S@st.fixed2.sd}{4.5}
\@namedef{S@st.fixed2.sig}{0}
\@namedef{S@st.fixed2.trig}{0}
\@namedef{S@st.fixed2.u35k}{41.5}
\@namedef{S@st.fixed2.ups}{1190}
\@namedef{S@st.fixed2.ustopk}{27.9}
\@namedef{S@st.fixed2K16i2.cov}{0.893}
\@namedef{S@st.fixed2K16i2.max}{21}
\@namedef{S@st.fixed2K16i2.mean}{16.2}
\@namedef{S@st.fixed2K16i2.min}{8}
\@namedef{S@st.fixed2K16i2.pct}{25}
\@namedef{S@st.fixed2K16i2.rate}{0.52}
\@namedef{S@st.fixed2K16i2.rate35}{0.51}
\@namedef{S@st.fixed2K16i2.s90}{39.8}
\@namedef{S@st.fixed2K16i2.s97}{7.4}
\@namedef{S@st.fixed2K16i2.sd}{3.9}
\@namedef{S@st.fixed2K16i2.sig}{0}
\@namedef{S@st.fixed2K16i2.trig}{0}
\@namedef{S@st.fixed2K16i2.u35k}{20.7}
\@namedef{S@st.fixed2K16i2.ups}{593}
\@namedef{S@st.fixed2K16i2.ustopk}{17.2}
\@namedef{S@st.fixed2K64i2.cov}{0.925}
\@namedef{S@st.fixed2K64i2.max}{31}
\@namedef{S@st.fixed2K64i2.mean}{26.9}
\@namedef{S@st.fixed2K64i2.min}{22}
\@namedef{S@st.fixed2K64i2.pct}{42}
\@namedef{S@st.fixed2K64i2.rate}{0.52}
\@namedef{S@st.fixed2K64i2.rate35}{0.51}
\@namedef{S@st.fixed2K64i2.s90}{47.9}
\@namedef{S@st.fixed2K64i2.s97}{13.4}
\@namedef{S@st.fixed2K64i2.sd}{2.9}
\@namedef{S@st.fixed2K64i2.sig}{0}
\@namedef{S@st.fixed2K64i2.trig}{0}
\@namedef{S@st.fixed2K64i2.u35k}{82.9}
\@namedef{S@st.fixed2K64i2.ups}{2380}
\@namedef{S@st.fixed2K64i2.ustopk}{56.7}
\@namedef{S@st.fixed3.cov}{0.909}
\@namedef{S@st.fixed3.max}{27}
\@namedef{S@st.fixed3.mean}{21.4}
\@namedef{S@st.fixed3.min}{17}
\@namedef{S@st.fixed3.pct}{33}
\@namedef{S@st.fixed3.rate}{0.35}
\@namedef{S@st.fixed3.rate35}{0.34}
\@namedef{S@st.fixed3.s23}{21}
\@namedef{S@st.fixed3.s90}{43.3}
\@namedef{S@st.fixed3.s97}{11.2}
\@namedef{S@st.fixed3.sd}{3.2}
\@namedef{S@st.fixed3.sig}{0}
\@namedef{S@st.fixed3.trig}{0}
\@namedef{S@st.fixed3.u35k}{27.6}
\@namedef{S@st.fixed3.ups}{799}
\@namedef{S@st.fixed3.ustopk}{21.1}
\@namedef{S@st.fixed4.cov}{0.903}
\@namedef{S@st.fixed4.max}{19}
\@namedef{S@st.fixed4.mean}{16.8}
\@namedef{S@st.fixed4.min}{15}
\@namedef{S@st.fixed4.pct}{26}
\@namedef{S@st.fixed4.rate}{0.26}
\@namedef{S@st.fixed4.rate35}{0.26}
\@namedef{S@st.fixed4.s23}{15}
\@namedef{S@st.fixed4.s90}{41.4}
\@namedef{S@st.fixed4.s97}{7.9}
\@namedef{S@st.fixed4.sd}{1.3}
\@namedef{S@st.fixed4.sig}{0}
\@namedef{S@st.fixed4.trig}{0}
\@namedef{S@st.fixed4.u35k}{20.7}
\@namedef{S@st.fixed4.ups}{602}
\@namedef{S@st.fixed4.ustopk}{17.0}
\@namedef{S@st.fixed4K128i2.cov}{0.919}
\@namedef{S@st.fixed4K128i2.max}{30}
\@namedef{S@st.fixed4K128i2.mean}{23.5}
\@namedef{S@st.fixed4K128i2.min}{17}
\@namedef{S@st.fixed4K128i2.pct}{37}
\@namedef{S@st.fixed4K128i2.rate}{0.26}
\@namedef{S@st.fixed4K128i2.rate35}{0.26}
\@namedef{S@st.fixed4K128i2.s90}{46.6}
\@namedef{S@st.fixed4K128i2.s97}{10.2}
\@namedef{S@st.fixed4K128i2.sd}{3.7}
\@namedef{S@st.fixed4K128i2.sig}{0}
\@namedef{S@st.fixed4K128i2.trig}{0}
\@namedef{S@st.fixed4K128i2.u35k}{82.9}
\@namedef{S@st.fixed4K128i2.ups}{2422}
\@namedef{S@st.fixed4K128i2.ustopk}{62.8}
\@namedef{S@st.fixed4K32i8.cov}{0.941}
\@namedef{S@st.fixed4K32i8.max}{39}
\@namedef{S@st.fixed4K32i8.mean}{34.2}
\@namedef{S@st.fixed4K32i8.min}{26}
\@namedef{S@st.fixed4K32i8.pct}{53}
\@namedef{S@st.fixed4K32i8.rate}{0.27}
\@namedef{S@st.fixed4K32i8.rate35}{0.26}
\@namedef{S@st.fixed4K32i8.s90}{54.1}
\@namedef{S@st.fixed4K32i8.s97}{18.5}
\@namedef{S@st.fixed4K32i8.sd}{4.1}
\@namedef{S@st.fixed4K32i8.sig}{0}
\@namedef{S@st.fixed4K32i8.trig}{0}
\@namedef{S@st.fixed4K32i8.u35k}{82.9}
\@namedef{S@st.fixed4K32i8.ups}{2443}
\@namedef{S@st.fixed4K32i8.ustopk}{50.0}
\@namedef{S@st.fixed4K64i2.cov}{0.911}
\@namedef{S@st.fixed4K64i2.max}{27}
\@namedef{S@st.fixed4K64i2.mean}{23.6}
\@namedef{S@st.fixed4K64i2.min}{21}
\@namedef{S@st.fixed4K64i2.pct}{37}
\@namedef{S@st.fixed4K64i2.rate}{0.26}
\@namedef{S@st.fixed4K64i2.rate35}{0.26}
\@namedef{S@st.fixed4K64i2.s90}{45.4}
\@namedef{S@st.fixed4K64i2.s97}{10.8}
\@namedef{S@st.fixed4K64i2.sd}{2.0}
\@namedef{S@st.fixed4K64i2.sig}{0}
\@namedef{S@st.fixed4K64i2.trig}{0}
\@namedef{S@st.fixed4K64i2.u35k}{41.5}
\@namedef{S@st.fixed4K64i2.ups}{1208}
\@namedef{S@st.fixed4K64i2.ustopk}{31.1}
\@namedef{S@st.fixed4K64i4.cov}{0.934}
\@namedef{S@st.fixed4K64i4.max}{36}
\@namedef{S@st.fixed4K64i4.mean}{31.4}
\@namedef{S@st.fixed4K64i4.min}{25}
\@namedef{S@st.fixed4K64i4.pct}{49}
\@namedef{S@st.fixed4K64i4.rate}{0.26}
\@namedef{S@st.fixed4K64i4.rate35}{0.26}
\@namedef{S@st.fixed4K64i4.s90}{51.2}
\@namedef{S@st.fixed4K64i4.s97}{15.8}
\@namedef{S@st.fixed4K64i4.sd}{3.4}
\@namedef{S@st.fixed4K64i4.sig}{0}
\@namedef{S@st.fixed4K64i4.trig}{0}
\@namedef{S@st.fixed4K64i4.u35k}{82.9}
\@namedef{S@st.fixed4K64i4.ups}{2442}
\@namedef{S@st.fixed4K64i4.ustopk}{54.1}
\@namedef{S@st.fixed6.cov}{0.886}
\@namedef{S@st.fixed6.max}{15}
\@namedef{S@st.fixed6.mean}{12.9}
\@namedef{S@st.fixed6.min}{10}
\@namedef{S@st.fixed6.pct}{20}
\@namedef{S@st.fixed6.rate}{0.17}
\@namedef{S@st.fixed6.rate35}{0.17}
\@namedef{S@st.fixed6.s23}{12}
\@namedef{S@st.fixed6.s90}{34.0}
\@namedef{S@st.fixed6.s97}{4.6}
\@namedef{S@st.fixed6.sd}{1.6}
\@namedef{S@st.fixed6.sig}{0}
\@namedef{S@st.fixed6.trig}{0}
\@namedef{S@st.fixed6.u35k}{13.8}
\@namedef{S@st.fixed6.ups}{402}
\@namedef{S@st.fixed6.ustopk}{12.2}
\@namedef{S@st.geom.cov}{0.913}
\@namedef{S@st.geom.max}{23}
\@namedef{S@st.geom.mean}{20.1}
\@namedef{S@st.geom.min}{18}
\@namedef{S@st.geom.pct}{31}
\@namedef{S@st.geom.rate}{0.26}
\@namedef{S@st.geom.rate35}{0.24}
\@namedef{S@st.geom.s90}{44.9}
\@namedef{S@st.geom.s97}{10.3}
\@namedef{S@st.geom.sd}{1.9}
\@namedef{S@st.geom.sig}{40}
\@namedef{S@st.geom.trig}{12}
\@namedef{S@st.geom.u35k}{19.5}
\@namedef{S@st.geom.ups}{588}
\@namedef{S@st.geom.ustopk}{15.8}
\@namedef{S@st.holm10.max}{0.002}
\@namedef{S@st.mono}{7}
\@namedef{S@st.pair.budget.p1.ci}{+13.7 to +28.6}
\@namedef{S@st.pair.budget.p1.d}{+21.2}
\@namedef{S@st.pair.budget.p1.p}{<0.001}
\@namedef{S@st.pair.budget.p1.pp}{$p<0.001$}
\@namedef{S@st.pair.budget.p2.ci}{+3.0 to +18.6}
\@namedef{S@st.pair.budget.p2.d}{+10.7}
\@namedef{S@st.pair.budget.p2.p}{0.007}
\@namedef{S@st.pair.budget.p2.pp}{$p=0.007$}
\@namedef{S@st.pair.budget.p4.ci}{\ensuremath{-}0.3 to +14.0}
\@namedef{S@st.pair.budget.p4.d}{+6.7}
\@namedef{S@st.pair.budget.p4.p}{0.061}
\@namedef{S@st.pair.budget.p4.pp}{$p=0.061$}
\@namedef{S@st.pair.cand.k128.k64.ci}{\ensuremath{-}7.4 to +6.9}
\@namedef{S@st.pair.cand.k128.k64.d}{\ensuremath{-}0.1}
\@namedef{S@st.pair.cand.k128.k64.p}{1.000}
\@namedef{S@st.pair.cand.k128.k64.pp}{$p=1.000$}
\@namedef{S@st.pair.cand.k64.fixed4.ci}{\ensuremath{-}1.0 to +14.7}
\@namedef{S@st.pair.cand.k64.fixed4.d}{+6.8}
\@namedef{S@st.pair.cand.k64.fixed4.p}{0.092}
\@namedef{S@st.pair.cand.k64.fixed4.pp}{$p=0.092$}
\@namedef{S@st.pair.fixed1.fixed2.ci}{\ensuremath{-}0.4 to +8.8}
\@namedef{S@st.pair.fixed1.fixed2.d}{+4.3}
\@namedef{S@st.pair.fixed1.fixed2.p}{0.072}
\@namedef{S@st.pair.fixed1.fixed2.pp}{$p=0.072$}
\@namedef{S@st.pair.fixed2.fixed3.ci}{+2.8 to +13.4}
\@namedef{S@st.pair.fixed2.fixed3.d}{+8.0}
\@namedef{S@st.pair.fixed2.fixed3.p}{0.001}
\@namedef{S@st.pair.fixed2.fixed3.pp}{$p=0.001$}
\@namedef{S@st.pair.fixed3.fixed4.ci}{+0.3 to +9.2}
\@namedef{S@st.pair.fixed3.fixed4.d}{+4.6}
\@namedef{S@st.pair.fixed3.fixed4.p}{0.040}
\@namedef{S@st.pair.fixed3.fixed4.pp}{$p=0.040$}
\@namedef{S@st.pair.fixed4.fixed6.ci}{\ensuremath{-}0.5 to +8.6}
\@namedef{S@st.pair.fixed4.fixed6.d}{+3.9}
\@namedef{S@st.pair.fixed4.fixed6.p}{0.088}
\@namedef{S@st.pair.fixed4.fixed6.pp}{$p=0.088$}
\@namedef{S@st.pair.period.1152.ci}{\ensuremath{-}5.5 to +9.1}
\@namedef{S@st.pair.period.1152.d}{+1.9}
\@namedef{S@st.pair.period.1152.p}{0.623}
\@namedef{S@st.pair.period.1152.pp}{$p=0.623$}
\@namedef{S@st.pair.period.2304.ci}{+2.6 to +17.5}
\@namedef{S@st.pair.period.2304.d}{+10.2}
\@namedef{S@st.pair.period.2304.p}{0.008}
\@namedef{S@st.pair.period.2304.pp}{$p=0.008$}
\@namedef{S@st.pair.period.576.ci}{\ensuremath{-}11.2 to +2.5}
\@namedef{S@st.pair.period.576.d}{\ensuremath{-}4.3}
\@namedef{S@st.pair.period.576.p}{0.223}
\@namedef{S@st.pair.period.576.pp}{$p=0.223$}
\@namedef{S@st.pair.rounds.r4.fixed1.ci}{\ensuremath{-}8.7 to +4.3}
\@namedef{S@st.pair.rounds.r4.fixed1.d}{\ensuremath{-}2.3}
\@namedef{S@st.pair.rounds.r4.fixed1.p}{0.495}
\@namedef{S@st.pair.rounds.r4.fixed1.pp}{$p=0.495$}
\@namedef{S@st.pair.rounds.r4.k128.ci}{+1.5 to +14.3}
\@namedef{S@st.pair.rounds.r4.k128.d}{+7.9}
\@namedef{S@st.pair.rounds.r4.k128.p}{0.016}
\@namedef{S@st.pair.rounds.r4.k128.pp}{$p=0.016$}
\@namedef{S@st.pair.rounds.r8.fixed1.ci}{\ensuremath{-}5.5 to +6.7}
\@namedef{S@st.pair.rounds.r8.fixed1.d}{+0.5}
\@namedef{S@st.pair.rounds.r8.fixed1.p}{0.889}
\@namedef{S@st.pair.rounds.r8.fixed1.pp}{$p=0.889$}
\@namedef{S@st.pair.rounds.r8.fixed4.ci}{+11.2 to +23.7}
\@namedef{S@st.pair.rounds.r8.fixed4.d}{+17.4}
\@namedef{S@st.pair.rounds.r8.fixed4.p}{<0.001}
\@namedef{S@st.pair.rounds.r8.fixed4.pp}{$p<0.001$}
\@namedef{S@st.pair.rounds.r8.k128.ci}{+3.7 to +17.6}
\@namedef{S@st.pair.rounds.r8.k128.d}{+10.7}
\@namedef{S@st.pair.rounds.r8.k128.p}{0.002}
\@namedef{S@st.pair.rounds.r8.k128.pp}{$p=0.002$}
\@namedef{S@st.paircov.budget.p1.ci}{+0.055 to +0.113}
\@namedef{S@st.paircov.budget.p1.d}{+0.082}
\@namedef{S@st.paircov.budget.p1.p}{<0.001}
\@namedef{S@st.paircov.budget.p1.pp}{$p<0.001$}
\@namedef{S@st.paircov.budget.p2.ci}{+0.012 to +0.055}
\@namedef{S@st.paircov.budget.p2.d}{+0.032}
\@namedef{S@st.paircov.budget.p2.p}{<0.001}
\@namedef{S@st.paircov.budget.p2.pp}{$p<0.001$}
\@namedef{S@st.paircov.budget.p4.ci}{+0.000 to +0.032}
\@namedef{S@st.paircov.budget.p4.d}{+0.015}
\@namedef{S@st.paircov.budget.p4.p}{0.045}
\@namedef{S@st.paircov.budget.p4.pp}{$p=0.045$}
\@namedef{S@st.paircov.cand.k128.k64.ci}{\ensuremath{-}0.008 to +0.025}
\@namedef{S@st.paircov.cand.k128.k64.d}{+0.008}
\@namedef{S@st.paircov.cand.k128.k64.p}{0.346}
\@namedef{S@st.paircov.cand.k128.k64.pp}{$p=0.346$}
\@namedef{S@st.paircov.cand.k64.fixed4.ci}{\ensuremath{-}0.011 to +0.027}
\@namedef{S@st.paircov.cand.k64.fixed4.d}{+0.008}
\@namedef{S@st.paircov.cand.k64.fixed4.p}{0.414}
\@namedef{S@st.paircov.cand.k64.fixed4.pp}{$p=0.414$}
\@namedef{S@st.paircov.fixed1.fixed2.ci}{+0.002 to +0.014}
\@namedef{S@st.paircov.fixed1.fixed2.d}{+0.008}
\@namedef{S@st.paircov.fixed1.fixed2.p}{0.016}
\@namedef{S@st.paircov.fixed1.fixed2.pp}{$p=0.016$}
\@namedef{S@st.paircov.fixed2.fixed3.ci}{+0.010 to +0.029}
\@namedef{S@st.paircov.fixed2.fixed3.d}{+0.019}
\@namedef{S@st.paircov.fixed2.fixed3.p}{<0.001}
\@namedef{S@st.paircov.fixed2.fixed3.pp}{$p<0.001$}
\@namedef{S@st.paircov.fixed3.fixed4.ci}{\ensuremath{-}0.003 to +0.016}
\@namedef{S@st.paircov.fixed3.fixed4.d}{+0.006}
\@namedef{S@st.paircov.fixed3.fixed4.p}{0.191}
\@namedef{S@st.paircov.fixed3.fixed4.pp}{$p=0.191$}
\@namedef{S@st.paircov.fixed4.fixed6.ci}{+0.005 to +0.028}
\@namedef{S@st.paircov.fixed4.fixed6.d}{+0.017}
\@namedef{S@st.paircov.fixed4.fixed6.p}{0.007}
\@namedef{S@st.paircov.fixed4.fixed6.pp}{$p=0.007$}
\@namedef{S@st.paircov.period.1152.ci}{\ensuremath{-}0.004 to +0.029}
\@namedef{S@st.paircov.period.1152.d}{+0.013}
\@namedef{S@st.paircov.period.1152.p}{0.136}
\@namedef{S@st.paircov.period.1152.pp}{$p=0.136$}
\@namedef{S@st.paircov.period.2304.ci}{+0.005 to +0.029}
\@namedef{S@st.paircov.period.2304.d}{+0.017}
\@namedef{S@st.paircov.period.2304.p}{0.005}
\@namedef{S@st.paircov.period.2304.pp}{$p=0.005$}
\@namedef{S@st.paircov.period.576.ci}{\ensuremath{-}0.080 to \ensuremath{-}0.021}
\@namedef{S@st.paircov.period.576.d}{\ensuremath{-}0.049}
\@namedef{S@st.paircov.period.576.p}{<0.001}
\@namedef{S@st.paircov.period.576.pp}{$p<0.001$}
\@namedef{S@st.paircov.rounds.r4.fixed1.ci}{\ensuremath{-}0.011 to +0.008}
\@namedef{S@st.paircov.rounds.r4.fixed1.d}{\ensuremath{-}0.001}
\@namedef{S@st.paircov.rounds.r4.fixed1.p}{0.756}
\@namedef{S@st.paircov.rounds.r4.fixed1.pp}{$p=0.756$}
\@namedef{S@st.paircov.rounds.r4.k128.ci}{+0.006 to +0.027}
\@namedef{S@st.paircov.rounds.r4.k128.d}{+0.016}
\@namedef{S@st.paircov.rounds.r4.k128.p}{0.004}
\@namedef{S@st.paircov.rounds.r4.k128.pp}{$p=0.004$}
\@namedef{S@st.paircov.rounds.r8.fixed1.ci}{\ensuremath{-}0.003 to +0.014}
\@namedef{S@st.paircov.rounds.r8.fixed1.d}{+0.005}
\@namedef{S@st.paircov.rounds.r8.fixed1.p}{0.209}
\@namedef{S@st.paircov.rounds.r8.fixed1.pp}{$p=0.209$}
\@namedef{S@st.paircov.rounds.r8.fixed4.ci}{+0.025 to +0.054}
\@namedef{S@st.paircov.rounds.r8.fixed4.d}{+0.038}
\@namedef{S@st.paircov.rounds.r8.fixed4.p}{<0.001}
\@namedef{S@st.paircov.rounds.r8.fixed4.pp}{$p<0.001$}
\@namedef{S@st.paircov.rounds.r8.k128.ci}{+0.012 to +0.034}
\@namedef{S@st.paircov.rounds.r8.k128.d}{+0.023}
\@namedef{S@st.paircov.rounds.r8.k128.p}{<0.001}
\@namedef{S@st.paircov.rounds.r8.k128.pp}{$p<0.001$}
\@namedef{S@st.prim.halfwidth}{4.1}
\@namedef{S@st.prim.maxhi}{+6.8}
\@namedef{S@st.prim.minlo}{\ensuremath{-}5.7}
\@namedef{S@st.r35.maxexcess}{+0.000}
\@namedef{S@st.r35.maxexcess4}{0.0003}
\@namedef{S@st.r35.minexcess}{\ensuremath{-}0.098}
\@namedef{S@st.random.contactq25.cov}{0.934}
\@namedef{S@st.random.contactq25.max}{36}
\@namedef{S@st.random.contactq25.mean}{32.3}
\@namedef{S@st.random.contactq25.min}{29}
\@namedef{S@st.random.contactq25.pct}{50}
\@namedef{S@st.random.contactq25.rate}{0.82}
\@namedef{S@st.random.contactq25.rate35}{0.82}
\@namedef{S@st.random.contactq25.s90}{49.9}
\@namedef{S@st.random.contactq25.s97}{16.9}
\@namedef{S@st.random.contactq25.sd}{2.2}
\@namedef{S@st.random.contactq25.sig}{94}
\@namedef{S@st.random.contactq25.trig}{81}
\@namedef{S@st.random.contactq25.u35k}{66.1}
\@namedef{S@st.random.contactq25.ups}{1895}
\@namedef{S@st.random.contactq25.ustopk}{41.4}
\@namedef{S@st.random.contactq50.cov}{0.927}
\@namedef{S@st.random.contactq50.max}{33}
\@namedef{S@st.random.contactq50.mean}{29.1}
\@namedef{S@st.random.contactq50.min}{27}
\@namedef{S@st.random.contactq50.pct}{45}
\@namedef{S@st.random.contactq50.rate}{0.62}
\@namedef{S@st.random.contactq50.rate35}{0.62}
\@namedef{S@st.random.contactq50.s90}{47.5}
\@namedef{S@st.random.contactq50.s97}{12.3}
\@namedef{S@st.random.contactq50.sd}{2.3}
\@namedef{S@st.random.contactq50.sig}{92}
\@namedef{S@st.random.contactq50.trig}{60}
\@namedef{S@st.random.contactq50.u35k}{50.1}
\@namedef{S@st.random.contactq50.ups}{1436}
\@namedef{S@st.random.contactq50.ustopk}{33.3}
\@namedef{S@st.random.contactq75.cov}{0.909}
\@namedef{S@st.random.contactq75.max}{26}
\@namedef{S@st.random.contactq75.mean}{21.4}
\@namedef{S@st.random.contactq75.min}{19}
\@namedef{S@st.random.contactq75.pct}{33}
\@namedef{S@st.random.contactq75.rate}{0.34}
\@namedef{S@st.random.contactq75.rate35}{0.33}
\@namedef{S@st.random.contactq75.s90}{43.6}
\@namedef{S@st.random.contactq75.s97}{5.6}
\@namedef{S@st.random.contactq75.sd}{2.1}
\@namedef{S@st.random.contactq75.sig}{72}
\@namedef{S@st.random.contactq75.trig}{27}
\@namedef{S@st.random.contactq75.u35k}{26.9}
\@namedef{S@st.random.contactq75.ups}{775}
\@namedef{S@st.random.contactq75.ustopk}{20.7}
\@namedef{S@st.random.contactq90.cov}{0.895}
\@namedef{S@st.random.contactq90.max}{17}
\@namedef{S@st.random.contactq90.mean}{15.6}
\@namedef{S@st.random.contactq90.min}{13}
\@namedef{S@st.random.contactq90.pct}{24}
\@namedef{S@st.random.contactq90.rate}{0.23}
\@namedef{S@st.random.contactq90.rate35}{0.22}
\@namedef{S@st.random.contactq90.s90}{38.0}
\@namedef{S@st.random.contactq90.s97}{4.0}
\@namedef{S@st.random.contactq90.sd}{1.3}
\@namedef{S@st.random.contactq90.sig}{35}
\@namedef{S@st.random.contactq90.trig}{9}
\@namedef{S@st.random.contactq90.u35k}{18.1}
\@namedef{S@st.random.contactq90.ups}{522}
\@namedef{S@st.random.contactq90.ustopk}{15.2}
\@namedef{S@st.random.disagreementq25.cov}{0.921}
\@namedef{S@st.random.disagreementq25.max}{30}
\@namedef{S@st.random.disagreementq25.mean}{26.0}
\@namedef{S@st.random.disagreementq25.min}{23}
\@namedef{S@st.random.disagreementq25.pct}{41}
\@namedef{S@st.random.disagreementq25.rate}{0.48}
\@namedef{S@st.random.disagreementq25.rate35}{0.47}
\@namedef{S@st.random.disagreementq25.s90}{45.3}
\@namedef{S@st.random.disagreementq25.s97}{8.0}
\@namedef{S@st.random.disagreementq25.sd}{2.0}
\@namedef{S@st.random.disagreementq25.sig}{87}
\@namedef{S@st.random.disagreementq25.trig}{44}
\@namedef{S@st.random.disagreementq25.u35k}{38.0}
\@namedef{S@st.random.disagreementq25.ups}{1095}
\@namedef{S@st.random.disagreementq25.ustopk}{27.0}
\@namedef{S@st.random.disagreementq50.cov}{0.909}
\@namedef{S@st.random.disagreementq50.max}{25}
\@namedef{S@st.random.disagreementq50.mean}{21.3}
\@namedef{S@st.random.disagreementq50.min}{19}
\@namedef{S@st.random.disagreementq50.pct}{33}
\@namedef{S@st.random.disagreementq50.rate}{0.33}
\@namedef{S@st.random.disagreementq50.rate35}{0.33}
\@namedef{S@st.random.disagreementq50.s90}{43.7}
\@namedef{S@st.random.disagreementq50.s97}{5.3}
\@namedef{S@st.random.disagreementq50.sd}{1.6}
\@namedef{S@st.random.disagreementq50.sig}{71}
\@namedef{S@st.random.disagreementq50.trig}{26}
\@namedef{S@st.random.disagreementq50.u35k}{26.6}
\@namedef{S@st.random.disagreementq50.ups}{769}
\@namedef{S@st.random.disagreementq50.ustopk}{20.5}
\@namedef{S@st.random.disagreementq75.cov}{0.895}
\@namedef{S@st.random.disagreementq75.max}{19}
\@namedef{S@st.random.disagreementq75.mean}{16.1}
\@namedef{S@st.random.disagreementq75.min}{12}
\@namedef{S@st.random.disagreementq75.pct}{25}
\@namedef{S@st.random.disagreementq75.rate}{0.23}
\@namedef{S@st.random.disagreementq75.rate35}{0.23}
\@namedef{S@st.random.disagreementq75.s90}{38.5}
\@namedef{S@st.random.disagreementq75.s97}{3.4}
\@namedef{S@st.random.disagreementq75.sd}{1.9}
\@namedef{S@st.random.disagreementq75.sig}{38}
\@namedef{S@st.random.disagreementq75.trig}{10}
\@namedef{S@st.random.disagreementq75.u35k}{18.4}
\@namedef{S@st.random.disagreementq75.ups}{532}
\@namedef{S@st.random.disagreementq75.ustopk}{15.4}
\@namedef{S@st.random.disagreementq90.cov}{0.889}
\@namedef{S@st.random.disagreementq90.max}{16}
\@namedef{S@st.random.disagreementq90.mean}{14.1}
\@namedef{S@st.random.disagreementq90.min}{11}
\@namedef{S@st.random.disagreementq90.pct}{22}
\@namedef{S@st.random.disagreementq90.rate}{0.19}
\@namedef{S@st.random.disagreementq90.rate35}{0.19}
\@namedef{S@st.random.disagreementq90.s90}{36.2}
\@namedef{S@st.random.disagreementq90.s97}{4.4}
\@namedef{S@st.random.disagreementq90.sd}{1.8}
\@namedef{S@st.random.disagreementq90.sig}{13}
\@namedef{S@st.random.disagreementq90.trig}{3}
\@namedef{S@st.random.disagreementq90.u35k}{15.3}
\@namedef{S@st.random.disagreementq90.ups}{444}
\@namedef{S@st.random.disagreementq90.ustopk}{13.2}
\@namedef{S@st.random.errorq25.cov}{0.925}
\@namedef{S@st.random.errorq25.max}{31}
\@namedef{S@st.random.errorq25.mean}{27.8}
\@namedef{S@st.random.errorq25.min}{25}
\@namedef{S@st.random.errorq25.pct}{43}
\@namedef{S@st.random.errorq25.rate}{0.56}
\@namedef{S@st.random.errorq25.rate35}{0.56}
\@namedef{S@st.random.errorq25.s90}{46.3}
\@namedef{S@st.random.errorq25.s97}{10.5}
\@namedef{S@st.random.errorq25.sd}{1.8}
\@namedef{S@st.random.errorq25.sig}{91}
\@namedef{S@st.random.errorq25.trig}{53}
\@namedef{S@st.random.errorq25.u35k}{44.8}
\@namedef{S@st.random.errorq25.ups}{1287}
\@namedef{S@st.random.errorq25.ustopk}{30.6}
\@namedef{S@st.random.errorq50.cov}{0.912}
\@namedef{S@st.random.errorq50.max}{26}
\@namedef{S@st.random.errorq50.mean}{22.2}
\@namedef{S@st.random.errorq50.min}{20}
\@namedef{S@st.random.errorq50.pct}{35}
\@namedef{S@st.random.errorq50.rate}{0.36}
\@namedef{S@st.random.errorq50.rate35}{0.36}
\@namedef{S@st.random.errorq50.s90}{43.7}
\@namedef{S@st.random.errorq50.s97}{5.8}
\@namedef{S@st.random.errorq50.sd}{1.9}
\@namedef{S@st.random.errorq50.sig}{76}
\@namedef{S@st.random.errorq50.trig}{30}
\@namedef{S@st.random.errorq50.u35k}{28.8}
\@namedef{S@st.random.errorq50.ups}{832}
\@namedef{S@st.random.errorq50.ustopk}{21.9}
\@namedef{S@st.random.errorq75.cov}{0.895}
\@namedef{S@st.random.errorq75.max}{20}
\@namedef{S@st.random.errorq75.mean}{16.0}
\@namedef{S@st.random.errorq75.min}{13}
\@namedef{S@st.random.errorq75.pct}{25}
\@namedef{S@st.random.errorq75.rate}{0.23}
\@namedef{S@st.random.errorq75.rate35}{0.23}
\@namedef{S@st.random.errorq75.s90}{38.4}
\@namedef{S@st.random.errorq75.s97}{3.5}
\@namedef{S@st.random.errorq75.sd}{1.8}
\@namedef{S@st.random.errorq75.sig}{36}
\@namedef{S@st.random.errorq75.trig}{10}
\@namedef{S@st.random.errorq75.u35k}{18.2}
\@namedef{S@st.random.errorq75.ups}{527}
\@namedef{S@st.random.errorq75.ustopk}{15.3}
\@namedef{S@st.random.errorq90.cov}{0.889}
\@namedef{S@st.random.errorq90.max}{16}
\@namedef{S@st.random.errorq90.mean}{13.9}
\@namedef{S@st.random.errorq90.min}{11}
\@namedef{S@st.random.errorq90.pct}{22}
\@namedef{S@st.random.errorq90.rate}{0.19}
\@namedef{S@st.random.errorq90.rate35}{0.19}
\@namedef{S@st.random.errorq90.s90}{35.8}
\@namedef{S@st.random.errorq90.s97}{4.5}
\@namedef{S@st.random.errorq90.sd}{1.5}
\@namedef{S@st.random.errorq90.sig}{10}
\@namedef{S@st.random.errorq90.trig}{2}
\@namedef{S@st.random.errorq90.u35k}{15.0}
\@namedef{S@st.random.errorq90.ups}{435}
\@namedef{S@st.random.errorq90.ustopk}{13.0}
\@namedef{S@st.random.geom.cov}{0.898}
\@namedef{S@st.random.geom.max}{20}
\@namedef{S@st.random.geom.mean}{17.4}
\@namedef{S@st.random.geom.min}{14}
\@namedef{S@st.random.geom.pct}{27}
\@namedef{S@st.random.geom.rate}{0.25}
\@namedef{S@st.random.geom.rate35}{0.25}
\@namedef{S@st.random.geom.s90}{39.4}
\@namedef{S@st.random.geom.s97}{3.8}
\@namedef{S@st.random.geom.sd}{1.8}
\@namedef{S@st.random.geom.sig}{47}
\@namedef{S@st.random.geom.trig}{14}
\@namedef{S@st.random.geom.u35k}{19.9}
\@namedef{S@st.random.geom.ups}{577}
\@namedef{S@st.random.geom.ustopk}{16.4}
\@namedef{S@st.ratio.rate}{3.8}
\@namedef{S@st.ratio.u35}{3.9}
\@namedef{S@st.ratio.ustop}{2.9}
\@namedef{S@st.seedlist}{23, 29, 37, 43, 53, 59, 61, 67, 73, 79}
\@namedef{S@st.seeds}{10}
\@namedef{S@st.sh.0.02.cov}{0.82}
\@namedef{S@st.sh.0.02.fixed1}{1.9}
\@namedef{S@st.sh.0.02.fixed1.max}{4}
\@namedef{S@st.sh.0.02.fixed1.min}{0}
\@namedef{S@st.sh.0.02.fixed4}{0.9}
\@namedef{S@st.sh.0.02.trig}{65}
\@namedef{S@st.sh.0.05.cov}{0.80}
\@namedef{S@st.sh.0.05.fixed1}{1.7}
\@namedef{S@st.sh.0.05.fixed1.max}{4}
\@namedef{S@st.sh.0.05.fixed1.min}{0}
\@namedef{S@st.sh.0.05.fixed4}{1.2}
\@namedef{S@st.sh.0.05.trig}{73}
\@namedef{S@st.sh.0.1.cov}{0.81}
\@namedef{S@st.sh.0.1.fixed1}{2.3}
\@namedef{S@st.sh.0.1.fixed1.max}{4}
\@namedef{S@st.sh.0.1.fixed1.min}{1}
\@namedef{S@st.sh.0.1.fixed4}{2.5}
\@namedef{S@st.sh.0.1.trig}{80}
\@namedef{S@st.sh.0.25.cov}{0.79}
\@namedef{S@st.sh.0.25.fixed1}{2.2}
\@namedef{S@st.sh.0.25.fixed1.max}{4}
\@namedef{S@st.sh.0.25.fixed1.min}{1}
\@namedef{S@st.sh.0.25.fixed4}{0.9}
\@namedef{S@st.sh.0.25.trig}{87}
\@namedef{S@st.sh.0.85.cov}{0.80}
\@namedef{S@st.sh.0.85.fixed1}{2.7}
\@namedef{S@st.sh.0.85.fixed1.max}{4}
\@namedef{S@st.sh.0.85.fixed1.min}{2}
\@namedef{S@st.sh.0.85.fixed4}{4.2}
\@namedef{S@st.sh.0.85.trig}{92}
\@namedef{S@st.sh.f1max}{2.7}
\@namedef{S@st.sh.f1min}{1.7}
\@namedef{S@st.sh.max}{4.2}
\@namedef{S@st.sh.trigmax}{92}
\@namedef{S@st.sh.trigmin}{65}
\@namedef{S@st.sw.contactq25.ci}{\ensuremath{-}1.0 to +3.1}
\@namedef{S@st.sw.contactq25.crate}{0.82}
\@namedef{S@st.sw.contactq25.d}{+1.1}
\@namedef{S@st.sw.contactq25.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.contactq25.holm13}{1.000}
\@namedef{S@st.sw.contactq25.p}{0.292}
\@namedef{S@st.sw.contactq25.pp}{$p=0.292$}
\@namedef{S@st.sw.contactq25.unmatched}{0}
\@namedef{S@st.sw.contactq50.ci}{+1.5 to +6.5}
\@namedef{S@st.sw.contactq50.crate}{0.62}
\@namedef{S@st.sw.contactq50.d}{+3.9}
\@namedef{S@st.sw.contactq50.hh13}{$p_{\mathrm{Holm}}=0.026$}
\@namedef{S@st.sw.contactq50.holm13}{0.026}
\@namedef{S@st.sw.contactq50.p}{0.002}
\@namedef{S@st.sw.contactq50.pp}{$p=0.002$}
\@namedef{S@st.sw.contactq50.unmatched}{0}
\@namedef{S@st.sw.contactq75.ci}{\ensuremath{-}5.7 to +2.3}
\@namedef{S@st.sw.contactq75.crate}{0.34}
\@namedef{S@st.sw.contactq75.d}{\ensuremath{-}1.6}
\@namedef{S@st.sw.contactq75.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.contactq75.holm13}{1.000}
\@namedef{S@st.sw.contactq75.p}{0.416}
\@namedef{S@st.sw.contactq75.pp}{$p=0.416$}
\@namedef{S@st.sw.contactq75.unmatched}{0}
\@namedef{S@st.sw.contactq90.ci}{\ensuremath{-}2.0 to +4.2}
\@namedef{S@st.sw.contactq90.crate}{0.23}
\@namedef{S@st.sw.contactq90.d}{+1.0}
\@namedef{S@st.sw.contactq90.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.contactq90.holm13}{1.000}
\@namedef{S@st.sw.contactq90.p}{0.537}
\@namedef{S@st.sw.contactq90.pp}{$p=0.537$}
\@namedef{S@st.sw.contactq90.unmatched}{0}
\@namedef{S@st.sw.disagreementq25.ci}{+0.5 to +6.6}
\@namedef{S@st.sw.disagreementq25.crate}{0.48}
\@namedef{S@st.sw.disagreementq25.d}{+3.5}
\@namedef{S@st.sw.disagreementq25.hh13}{$p_{\mathrm{Holm}}=0.226$}
\@namedef{S@st.sw.disagreementq25.holm13}{0.226}
\@namedef{S@st.sw.disagreementq25.p}{0.023}
\@namedef{S@st.sw.disagreementq25.pp}{$p=0.023$}
\@namedef{S@st.sw.disagreementq25.unmatched}{0}
\@namedef{S@st.sw.disagreementq50.ci}{\ensuremath{-}1.2 to +6.1}
\@namedef{S@st.sw.disagreementq50.crate}{0.33}
\@namedef{S@st.sw.disagreementq50.d}{+2.3}
\@namedef{S@st.sw.disagreementq50.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.disagreementq50.holm13}{1.000}
\@namedef{S@st.sw.disagreementq50.p}{0.202}
\@namedef{S@st.sw.disagreementq50.pp}{$p=0.202$}
\@namedef{S@st.sw.disagreementq50.unmatched}{0}
\@namedef{S@st.sw.disagreementq75.ci}{\ensuremath{-}1.3 to +4.5}
\@namedef{S@st.sw.disagreementq75.crate}{0.23}
\@namedef{S@st.sw.disagreementq75.d}{+1.6}
\@namedef{S@st.sw.disagreementq75.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.disagreementq75.holm13}{1.000}
\@namedef{S@st.sw.disagreementq75.p}{0.282}
\@namedef{S@st.sw.disagreementq75.pp}{$p=0.282$}
\@namedef{S@st.sw.disagreementq75.unmatched}{0}
\@namedef{S@st.sw.disagreementq90.ci}{\ensuremath{-}1.3 to +2.8}
\@namedef{S@st.sw.disagreementq90.crate}{0.19}
\@namedef{S@st.sw.disagreementq90.d}{+0.7}
\@namedef{S@st.sw.disagreementq90.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.disagreementq90.holm13}{1.000}
\@namedef{S@st.sw.disagreementq90.p}{0.523}
\@namedef{S@st.sw.disagreementq90.pp}{$p=0.523$}
\@namedef{S@st.sw.disagreementq90.unmatched}{0}
\@namedef{S@st.sw.dmax}{+4.9}
\@namedef{S@st.sw.dmin}{\ensuremath{-}1.6}
\@namedef{S@st.sw.errorq25.ci}{+0.9 to +6.4}
\@namedef{S@st.sw.errorq25.crate}{0.56}
\@namedef{S@st.sw.errorq25.d}{+3.7}
\@namedef{S@st.sw.errorq25.hh13}{$p_{\mathrm{Holm}}=0.092$}
\@namedef{S@st.sw.errorq25.holm13}{0.092}
\@namedef{S@st.sw.errorq25.p}{0.008}
\@namedef{S@st.sw.errorq25.pp}{$p=0.008$}
\@namedef{S@st.sw.errorq25.unmatched}{0}
\@namedef{S@st.sw.errorq50.ci}{+1.8 to +8.1}
\@namedef{S@st.sw.errorq50.crate}{0.36}
\@namedef{S@st.sw.errorq50.d}{+4.9}
\@namedef{S@st.sw.errorq50.hh13}{$p_{\mathrm{Holm}}=0.026$}
\@namedef{S@st.sw.errorq50.holm13}{0.026}
\@namedef{S@st.sw.errorq50.p}{0.002}
\@namedef{S@st.sw.errorq50.pp}{$p=0.002$}
\@namedef{S@st.sw.errorq50.unmatched}{0}
\@namedef{S@st.sw.errorq75.ci}{\ensuremath{-}1.1 to +5.5}
\@namedef{S@st.sw.errorq75.crate}{0.23}
\@namedef{S@st.sw.errorq75.d}{+2.0}
\@namedef{S@st.sw.errorq75.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.errorq75.holm13}{1.000}
\@namedef{S@st.sw.errorq75.p}{0.223}
\@namedef{S@st.sw.errorq75.pp}{$p=0.223$}
\@namedef{S@st.sw.errorq75.unmatched}{0}
\@namedef{S@st.sw.errorq90.ci}{\ensuremath{-}1.9 to +1.6}
\@namedef{S@st.sw.errorq90.crate}{0.19}
\@namedef{S@st.sw.errorq90.d}{\ensuremath{-}0.2}
\@namedef{S@st.sw.errorq90.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.errorq90.holm13}{1.000}
\@namedef{S@st.sw.errorq90.p}{0.860}
\@namedef{S@st.sw.errorq90.pp}{$p=0.860$}
\@namedef{S@st.sw.errorq90.unmatched}{0}
\@namedef{S@st.sw.geom.ci}{\ensuremath{-}1.3 to +6.8}
\@namedef{S@st.sw.geom.crate}{0.25}
\@namedef{S@st.sw.geom.d}{+2.7}
\@namedef{S@st.sw.geom.hh13}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@st.sw.geom.holm13}{1.000}
\@namedef{S@st.sw.geom.p}{0.187}
\@namedef{S@st.sw.geom.pp}{$p=0.187$}
\@namedef{S@st.sw.geom.unmatched}{0}
\@namedef{S@st.sw.hi}{+8.1}
\@namedef{S@st.sw.lo}{\ensuremath{-}5.7}
\@namedef{S@st.sw.ndpos}{11}
\@namedef{S@st.sw.nholm}{2}
\@namedef{S@st.sw.nneg}{0}
\@namedef{S@st.sw.npos}{4}
\@namedef{S@st.sw.nsig}{4}
\@namedef{S@st.swc.contactq25.ci}{\ensuremath{-}0.7 to +4.1}
\@namedef{S@st.swc.contactq25.d}{+1.6}
\@namedef{S@st.swc.contactq25.p}{0.182}
\@namedef{S@st.swc.contactq25.pp}{$p=0.182$}
\@namedef{S@st.swc.contactq50.ci}{\ensuremath{-}1.0 to +6.2}
\@namedef{S@st.swc.contactq50.d}{+2.6}
\@namedef{S@st.swc.contactq50.p}{0.155}
\@namedef{S@st.swc.contactq50.pp}{$p=0.155$}
\@namedef{S@st.swc.contactq75.ci}{\ensuremath{-}6.3 to +3.8}
\@namedef{S@st.swc.contactq75.d}{\ensuremath{-}1.3}
\@namedef{S@st.swc.contactq75.p}{0.610}
\@namedef{S@st.swc.contactq75.pp}{$p=0.610$}
\@namedef{S@st.swc.contactq90.ci}{\ensuremath{-}2.3 to +4.9}
\@namedef{S@st.swc.contactq90.d}{+1.2}
\@namedef{S@st.swc.contactq90.p}{0.509}
\@namedef{S@st.swc.contactq90.pp}{$p=0.509$}
\@namedef{S@st.swc.disagreementq25.ci}{\ensuremath{-}2.5 to +5.9}
\@namedef{S@st.swc.disagreementq25.d}{+1.7}
\@namedef{S@st.swc.disagreementq25.p}{0.405}
\@namedef{S@st.swc.disagreementq25.pp}{$p=0.405$}
\@namedef{S@st.swc.disagreementq50.ci}{\ensuremath{-}1.5 to +7.3}
\@namedef{S@st.swc.disagreementq50.d}{+2.7}
\@namedef{S@st.swc.disagreementq50.p}{0.208}
\@namedef{S@st.swc.disagreementq50.pp}{$p=0.208$}
\@namedef{S@st.swc.disagreementq75.ci}{\ensuremath{-}1.2 to +5.4}
\@namedef{S@st.swc.disagreementq75.d}{+2.1}
\@namedef{S@st.swc.disagreementq75.p}{0.194}
\@namedef{S@st.swc.disagreementq75.pp}{$p=0.194$}
\@namedef{S@st.swc.disagreementq90.ci}{\ensuremath{-}1.0 to +3.3}
\@namedef{S@st.swc.disagreementq90.d}{+1.0}
\@namedef{S@st.swc.disagreementq90.p}{0.337}
\@namedef{S@st.swc.disagreementq90.pp}{$p=0.337$}
\@namedef{S@st.swc.errorq25.ci}{\ensuremath{-}2.5 to +5.9}
\@namedef{S@st.swc.errorq25.d}{+1.6}
\@namedef{S@st.swc.errorq25.p}{0.428}
\@namedef{S@st.swc.errorq25.pp}{$p=0.428$}
\@namedef{S@st.swc.errorq50.ci}{+0.7 to +9.4}
\@namedef{S@st.swc.errorq50.d}{+5.0}
\@namedef{S@st.swc.errorq50.p}{0.025}
\@namedef{S@st.swc.errorq50.pp}{$p=0.025$}
\@namedef{S@st.swc.errorq75.ci}{\ensuremath{-}1.1 to +6.3}
\@namedef{S@st.swc.errorq75.d}{+2.5}
\@namedef{S@st.swc.errorq75.p}{0.175}
\@namedef{S@st.swc.errorq75.pp}{$p=0.175$}
\@namedef{S@st.swc.errorq90.ci}{\ensuremath{-}1.6 to +1.7}
\@namedef{S@st.swc.errorq90.d}{+0.0}
\@namedef{S@st.swc.errorq90.p}{0.940}
\@namedef{S@st.swc.errorq90.pp}{$p=0.940$}
\@namedef{S@st.swc.geom.ci}{\ensuremath{-}1.3 to +8.3}
\@namedef{S@st.swc.geom.d}{+3.5}
\@namedef{S@st.swc.geom.p}{0.153}
\@namedef{S@st.swc.geom.pp}{$p=0.153$}
\@namedef{S@st.swc.nsig}{1}
\@namedef{S@st.swcov.contactq25.ci}{\ensuremath{-}0.000 to +0.005}
\@namedef{S@st.swcov.contactq25.d}{+0.002}
\@namedef{S@st.swcov.contactq25.p}{0.104}
\@namedef{S@st.swcov.contactq25.pp}{$p=0.104$}
\@namedef{S@st.swcov.contactq50.ci}{+0.004 to +0.011}
\@namedef{S@st.swcov.contactq50.d}{+0.007}
\@namedef{S@st.swcov.contactq50.p}{<0.001}
\@namedef{S@st.swcov.contactq50.pp}{$p<0.001$}
\@namedef{S@st.swcov.contactq75.ci}{\ensuremath{-}0.004 to +0.013}
\@namedef{S@st.swcov.contactq75.d}{+0.004}
\@namedef{S@st.swcov.contactq75.p}{0.371}
\@namedef{S@st.swcov.contactq75.pp}{$p=0.371$}
\@namedef{S@st.swcov.contactq90.ci}{\ensuremath{-}0.000 to +0.013}
\@namedef{S@st.swcov.contactq90.d}{+0.006}
\@namedef{S@st.swcov.contactq90.p}{0.060}
\@namedef{S@st.swcov.contactq90.pp}{$p=0.060$}
\@namedef{S@st.swcov.disagreementq25.ci}{+0.006 to +0.015}
\@namedef{S@st.swcov.disagreementq25.d}{+0.010}
\@namedef{S@st.swcov.disagreementq25.p}{<0.001}
\@namedef{S@st.swcov.disagreementq25.pp}{$p<0.001$}
\@namedef{S@st.swcov.disagreementq50.ci}{+0.006 to +0.020}
\@namedef{S@st.swcov.disagreementq50.d}{+0.012}
\@namedef{S@st.swcov.disagreementq50.p}{0.001}
\@namedef{S@st.swcov.disagreementq50.pp}{$p=0.001$}
\@namedef{S@st.swcov.disagreementq75.ci}{+0.005 to +0.021}
\@namedef{S@st.swcov.disagreementq75.d}{+0.013}
\@namedef{S@st.swcov.disagreementq75.p}{<0.001}
\@namedef{S@st.swcov.disagreementq75.pp}{$p<0.001$}
\@namedef{S@st.swcov.disagreementq90.ci}{\ensuremath{-}0.001 to +0.012}
\@namedef{S@st.swcov.disagreementq90.d}{+0.005}
\@namedef{S@st.swcov.disagreementq90.p}{0.127}
\@namedef{S@st.swcov.disagreementq90.pp}{$p=0.127$}
\@namedef{S@st.swcov.errorq25.ci}{+0.004 to +0.013}
\@namedef{S@st.swcov.errorq25.d}{+0.008}
\@namedef{S@st.swcov.errorq25.p}{<0.001}
\@namedef{S@st.swcov.errorq25.pp}{$p<0.001$}
\@namedef{S@st.swcov.errorq50.ci}{+0.010 to +0.022}
\@namedef{S@st.swcov.errorq50.d}{+0.015}
\@namedef{S@st.swcov.errorq50.p}{<0.001}
\@namedef{S@st.swcov.errorq50.pp}{$p<0.001$}
\@namedef{S@st.swcov.errorq75.ci}{+0.005 to +0.019}
\@namedef{S@st.swcov.errorq75.d}{+0.012}
\@namedef{S@st.swcov.errorq75.p}{<0.001}
\@namedef{S@st.swcov.errorq75.pp}{$p<0.001$}
\@namedef{S@st.swcov.errorq90.ci}{\ensuremath{-}0.003 to +0.009}
\@namedef{S@st.swcov.errorq90.d}{+0.003}
\@namedef{S@st.swcov.errorq90.p}{0.338}
\@namedef{S@st.swcov.errorq90.pp}{$p=0.338$}
\@namedef{S@st.swcov.geom.ci}{+0.008 to +0.023}
\@namedef{S@st.swcov.geom.d}{+0.015}
\@namedef{S@st.swcov.geom.p}{<0.001}
\@namedef{S@st.swcov.geom.pp}{$p<0.001$}
\@namedef{S@st.swcov.ndpos}{13}
\@namedef{S@st.swcov.nholm}{8}
\@namedef{S@st.swcov.nneg}{0}
\@namedef{S@st.swcov.npos}{8}
\@namedef{S@st.swk.contactq25.ci}{\ensuremath{-}1.4 to +2.3}
\@namedef{S@st.swk.contactq25.d}{+0.4}
\@namedef{S@st.swk.contactq25.p}{0.656}
\@namedef{S@st.swk.contactq25.pp}{$p=0.656$}
\@namedef{S@st.swk.contactq50.ci}{\ensuremath{-}4.2 to +1.5}
\@namedef{S@st.swk.contactq50.d}{\ensuremath{-}1.3}
\@namedef{S@st.swk.contactq50.p}{0.363}
\@namedef{S@st.swk.contactq50.pp}{$p=0.363$}
\@namedef{S@st.swk.contactq75.ci}{\ensuremath{-}2.5 to +3.5}
\@namedef{S@st.swk.contactq75.d}{+0.5}
\@namedef{S@st.swk.contactq75.p}{0.760}
\@namedef{S@st.swk.contactq75.pp}{$p=0.760$}
\@namedef{S@st.swk.contactq90.ci}{\ensuremath{-}1.3 to +2.1}
\@namedef{S@st.swk.contactq90.d}{+0.4}
\@namedef{S@st.swk.contactq90.p}{0.652}
\@namedef{S@st.swk.contactq90.pp}{$p=0.652$}
\@namedef{S@st.swk.disagreementq25.ci}{\ensuremath{-}4.4 to +1.3}
\@namedef{S@st.swk.disagreementq25.d}{\ensuremath{-}1.6}
\@namedef{S@st.swk.disagreementq25.p}{0.285}
\@namedef{S@st.swk.disagreementq25.pp}{$p=0.285$}
\@namedef{S@st.swk.disagreementq50.ci}{\ensuremath{-}2.6 to +3.5}
\@namedef{S@st.swk.disagreementq50.d}{+0.5}
\@namedef{S@st.swk.disagreementq50.p}{0.771}
\@namedef{S@st.swk.disagreementq50.pp}{$p=0.771$}
\@namedef{S@st.swk.disagreementq75.ci}{\ensuremath{-}1.1 to +2.7}
\@namedef{S@st.swk.disagreementq75.d}{+0.7}
\@namedef{S@st.swk.disagreementq75.p}{0.450}
\@namedef{S@st.swk.disagreementq75.pp}{$p=0.450$}
\@namedef{S@st.swk.disagreementq90.ci}{\ensuremath{-}0.3 to +1.2}
\@namedef{S@st.swk.disagreementq90.d}{+0.4}
\@namedef{S@st.swk.disagreementq90.p}{0.245}
\@namedef{S@st.swk.disagreementq90.pp}{$p=0.245$}
\@namedef{S@st.swk.dmax}{+1.0}
\@namedef{S@st.swk.dmin}{\ensuremath{-}2.0}
\@namedef{S@st.swk.errorq25.ci}{\ensuremath{-}5.4 to +1.1}
\@namedef{S@st.swk.errorq25.d}{\ensuremath{-}2.0}
\@namedef{S@st.swk.errorq25.p}{0.214}
\@namedef{S@st.swk.errorq25.pp}{$p=0.214$}
\@namedef{S@st.swk.errorq50.ci}{\ensuremath{-}2.9 to +3.1}
\@namedef{S@st.swk.errorq50.d}{+0.2}
\@namedef{S@st.swk.errorq50.p}{0.927}
\@namedef{S@st.swk.errorq50.pp}{$p=0.927$}
\@namedef{S@st.swk.errorq75.ci}{\ensuremath{-}1.1 to +2.6}
\@namedef{S@st.swk.errorq75.d}{+0.7}
\@namedef{S@st.swk.errorq75.p}{0.458}
\@namedef{S@st.swk.errorq75.pp}{$p=0.458$}
\@namedef{S@st.swk.errorq90.ci}{\ensuremath{-}0.3 to +0.9}
\@namedef{S@st.swk.errorq90.d}{+0.3}
\@namedef{S@st.swk.errorq90.p}{0.317}
\@namedef{S@st.swk.errorq90.pp}{$p=0.317$}
\@namedef{S@st.swk.geom.ci}{\ensuremath{-}1.6 to +3.6}
\@namedef{S@st.swk.geom.d}{+1.0}
\@namedef{S@st.swk.geom.p}{0.447}
\@namedef{S@st.swk.geom.pp}{$p=0.447$}
\@namedef{S@st.swk.nsig}{0}
\@namedef{S@st.tasks}{64}
\@namedef{S@st.thr.contact.q25}{below 0.001}
\@namedef{S@st.thr.contact.q50}{below 0.001}
\@namedef{S@st.thr.contact.q75}{0.06}
\@namedef{S@st.thr.contact.q90}{0.71}
\@namedef{S@st.thr.disagreement.q25}{0.16}
\@namedef{S@st.thr.disagreement.q50}{0.25}
\@namedef{S@st.thr.disagreement.q75}{0.41}
\@namedef{S@st.thr.disagreement.q90}{0.70}
\@namedef{S@st.thr.error.q25}{0.12}
\@namedef{S@st.thr.error.q50}{0.23}
\@namedef{S@st.thr.error.q75}{0.45}
\@namedef{S@st.thr.error.q90}{0.88}
\@namedef{S@st.unmatched.arms}{0}
\@namedef{S@st.unmatched.total}{0}
\@namedef{S@time.pixels.obs}{1.2}
\@namedef{S@time.pixels.plan}{20}
\@namedef{S@time.plan.k128i2}{27}
\@namedef{S@time.plan.k32i2}{19}
\@namedef{S@time.plan.k32i8}{77}
\@namedef{S@time.plan.k64i4}{44}
\@namedef{S@time.state.obs}{0.0}
\@namedef{S@time.state.plan}{19}
\makeatother


==> numbers3.tex <==
% Generated by revision/build_stage3_assets.py from revision/stage3.json. Do not edit by hand.
\makeatletter
\@namedef{S@s3.floor.px.above.q25}{74}
\@namedef{S@s3.floor.px.above.q50}{50}
\@namedef{S@s3.floor.px.above.q75}{25}
\@namedef{S@s3.floor.px.above.q90}{10}
\@namedef{S@s3.floor.px.moving}{2.08}
\@namedef{S@s3.floor.px.mult.q25}{0.7}
\@namedef{S@s3.floor.px.mult.q25.max}{0.7}
\@namedef{S@s3.floor.px.mult.q25.min}{0.6}
\@namedef{S@s3.floor.px.mult.q50}{1.0}
\@namedef{S@s3.floor.px.mult.q50.max}{1.0}
\@namedef{S@s3.floor.px.mult.q50.min}{1.0}
\@namedef{S@s3.floor.px.mult.q75}{1.5}
\@namedef{S@s3.floor.px.mult.q75.max}{1.6}
\@namedef{S@s3.floor.px.mult.q75.min}{1.5}
\@namedef{S@s3.floor.px.mult.q90}{2.3}
\@namedef{S@s3.floor.px.mult.q90.max}{2.6}
\@namedef{S@s3.floor.px.mult.q90.min}{2.0}
\@namedef{S@s3.floor.px.n}{5}
\@namedef{S@s3.floor.px.p90}{4.79}
\@namedef{S@s3.floor.px.px}{2.06}
\@namedef{S@s3.floor.px.rest}{77}
\@namedef{S@s3.floor.px.thr.q25}{1.35}
\@namedef{S@s3.floor.px.thr.q50}{2.07}
\@namedef{S@s3.floor.px.thr.q75}{3.15}
\@namedef{S@s3.floor.px.thr.q90}{4.75}
\@namedef{S@s3.floor.st.above.q25}{70}
\@namedef{S@s3.floor.st.above.q50}{42}
\@namedef{S@s3.floor.st.above.q75}{19}
\@namedef{S@s3.floor.st.above.q90}{7}
\@namedef{S@s3.floor.st.moving}{0.42}
\@namedef{S@s3.floor.st.mult.q25}{0.6}
\@namedef{S@s3.floor.st.mult.q25.max}{0.6}
\@namedef{S@s3.floor.st.mult.q25.min}{0.6}
\@namedef{S@s3.floor.st.mult.q50}{1.2}
\@namedef{S@s3.floor.st.mult.q50.max}{1.2}
\@namedef{S@s3.floor.st.mult.q50.min}{1.2}
\@namedef{S@s3.floor.st.mult.q75}{2.4}
\@namedef{S@s3.floor.st.mult.q75.max}{2.6}
\@namedef{S@s3.floor.st.mult.q75.min}{2.2}
\@namedef{S@s3.floor.st.mult.q90}{4.7}
\@namedef{S@s3.floor.st.mult.q90.max}{5.5}
\@namedef{S@s3.floor.st.mult.q90.min}{4.0}
\@namedef{S@s3.floor.st.n}{10}
\@namedef{S@s3.floor.st.p90}{0.68}
\@namedef{S@s3.floor.st.px}{0.19}
\@namedef{S@s3.floor.st.rest}{76}
\@namedef{S@s3.floor.st.thr.q25}{0.12}
\@namedef{S@s3.floor.st.thr.q50}{0.23}
\@namedef{S@s3.floor.st.thr.q75}{0.45}
\@namedef{S@s3.floor.st.thr.q90}{0.88}
\@namedef{S@s3.mild.0.001.F.ci}{\ensuremath{-}0.5 to +5.6}
\@namedef{S@s3.mild.0.001.F.ci2}{\ensuremath{-}0.50 to +5.60}
\@namedef{S@s3.mild.0.001.F.d}{+2.4}
\@namedef{S@s3.mild.0.001.F.p}{0.107}
\@namedef{S@s3.mild.0.001.F.pp}{$p=0.107$}
\@namedef{S@s3.mild.0.001.coast}{22.3}
\@namedef{S@s3.mild.0.001.errorq75}{5.0}
\@namedef{S@s3.mild.0.001.errorq75.max}{9}
\@namedef{S@s3.mild.0.001.errorq75.min}{3}
\@namedef{S@s3.mild.0.001.fixed1}{5.0}
\@namedef{S@s3.mild.0.001.fixed1.max}{7}
\@namedef{S@s3.mild.0.001.fixed1.min}{2}
\@namedef{S@s3.mild.0.001.fixed4}{2.6}
\@namedef{S@s3.mild.0.001.fixed4.max}{4}
\@namedef{S@s3.mild.0.001.fixed4.min}{1}
\@namedef{S@s3.mild.0.001.oracle}{45}
\@namedef{S@s3.mild.0.001.trig}{45}
\@namedef{S@s3.mild.0.005.F.ci}{\ensuremath{-}4.6 to +2.3}
\@namedef{S@s3.mild.0.005.F.ci2}{\ensuremath{-}4.60 to +2.30}
\@namedef{S@s3.mild.0.005.F.d}{\ensuremath{-}1.1}
\@namedef{S@s3.mild.0.005.F.p}{0.537}
\@namedef{S@s3.mild.0.005.F.pp}{$p=0.537$}
\@namedef{S@s3.mild.0.005.coast}{28.7}
\@namedef{S@s3.mild.0.005.errorq75}{4.3}
\@namedef{S@s3.mild.0.005.errorq75.max}{7}
\@namedef{S@s3.mild.0.005.errorq75.min}{2}
\@namedef{S@s3.mild.0.005.fixed1}{4.0}
\@namedef{S@s3.mild.0.005.fixed1.max}{6}
\@namedef{S@s3.mild.0.005.fixed1.min}{2}
\@namedef{S@s3.mild.0.005.fixed4}{5.1}
\@namedef{S@s3.mild.0.005.fixed4.max}{8}
\@namedef{S@s3.mild.0.005.fixed4.min}{2}
\@namedef{S@s3.mild.0.005.oracle}{44}
\@namedef{S@s3.mild.0.005.trig}{56}
\@namedef{S@s3.mild.1e-05.F.ci}{\ensuremath{-}4.1 to +5.5}
\@namedef{S@s3.mild.1e-05.F.ci2}{\ensuremath{-}4.10 to +5.50}
\@namedef{S@s3.mild.1e-05.F.d}{+0.7}
\@namedef{S@s3.mild.1e-05.F.p}{0.782}
\@namedef{S@s3.mild.1e-05.F.pp}{$p=0.782$}
\@namedef{S@s3.mild.1e-05.coast}{13.7}
\@namedef{S@s3.mild.1e-05.errorq75}{11.3}
\@namedef{S@s3.mild.1e-05.errorq75.max}{15}
\@namedef{S@s3.mild.1e-05.errorq75.min}{6}
\@namedef{S@s3.mild.1e-05.fixed1}{11.3}
\@namedef{S@s3.mild.1e-05.fixed1.max}{14}
\@namedef{S@s3.mild.1e-05.fixed1.min}{9}
\@namedef{S@s3.mild.1e-05.fixed4}{10.6}
\@namedef{S@s3.mild.1e-05.fixed4.max}{13}
\@namedef{S@s3.mild.1e-05.fixed4.min}{9}
\@namedef{S@s3.mild.1e-05.oracle}{56}
\@namedef{S@s3.mild.1e-05.trig}{30}
\@namedef{S@s3.mild.1e-09.F.ci}{+2.6 to +14.2}
\@namedef{S@s3.mild.1e-09.F.ci2}{+2.60 to +14.20}
\@namedef{S@s3.mild.1e-09.F.d}{+8.2}
\@namedef{S@s3.mild.1e-09.F.p}{0.005}
\@namedef{S@s3.mild.1e-09.F.pp}{$p=0.005$}
\@namedef{S@s3.mild.1e-09.coast}{7.9}
\@namedef{S@s3.mild.1e-09.errorq75}{18.5}
\@namedef{S@s3.mild.1e-09.errorq75.max}{23}
\@namedef{S@s3.mild.1e-09.errorq75.min}{16}
\@namedef{S@s3.mild.1e-09.fixed1}{23.0}
\@namedef{S@s3.mild.1e-09.fixed1.max}{29}
\@namedef{S@s3.mild.1e-09.fixed1.min}{18}
\@namedef{S@s3.mild.1e-09.fixed4}{14.8}
\@namedef{S@s3.mild.1e-09.fixed4.max}{18}
\@namedef{S@s3.mild.1e-09.fixed4.min}{11}
\@namedef{S@s3.mild.1e-09.oracle}{55}
\@namedef{S@s3.mild.1e-09.trig}{21}
\@namedef{S@s3.mild.coast.max}{28.7}
\@namedef{S@s3.mild.coast.min}{7.9}
\@namedef{S@s3.mild.fixed1.max}{23.0}
\@namedef{S@s3.mild.fixed1.min}{4.0}
\@namedef{S@s3.mild.max}{23.0}
\@namedef{S@s3.mild.max3}{11.3}
\@namedef{S@s3.mild.n}{4}
\@namedef{S@s3.mild.oracle.max}{56}
\@namedef{S@s3.mild.oracle.min}{44}
\@namedef{S@s3.mild.oracle.nmost}{4}
\@namedef{S@s3.mild.trig.max}{56}
\@namedef{S@s3.mild.trig.min}{21}
\@namedef{S@s3.px.cells}{320}
\@namedef{S@s3.px.contactq25.ahead}{2}
\@namedef{S@s3.px.contactq25.aheadcov}{2}
\@namedef{S@s3.px.contactq25.aheadrandom}{3}
\@namedef{S@s3.px.contactq25.behind}{3}
\@namedef{S@s3.px.contactq25.random}{16.6}
\@namedef{S@s3.px.contactq25.random.cov}{0.901}
\@namedef{S@s3.px.contactq25.random.early}{0.83}
\@namedef{S@s3.px.contactq25.random.rate}{0.81}
\@namedef{S@s3.px.contactq25.random.rate35}{0.81}
\@namedef{S@s3.px.contactq25.random.u10}{0.82}
\@namedef{S@s3.px.contactq25.rule}{16.4}
\@namedef{S@s3.px.contactq25.rule.cov}{0.904}
\@namedef{S@s3.px.contactq25.rule.early}{0.97}
\@namedef{S@s3.px.contactq25.rule.rate}{0.81}
\@namedef{S@s3.px.contactq25.rule.rate35}{0.83}
\@namedef{S@s3.px.contactq25.rule.u10}{0.97}
\@namedef{S@s3.px.contactq25.shuffle}{16.4}
\@namedef{S@s3.px.contactq25.shuffle.cov}{0.904}
\@namedef{S@s3.px.contactq25.shuffle.early}{0.97}
\@namedef{S@s3.px.contactq25.shuffle.rate}{0.83}
\@namedef{S@s3.px.contactq25.shuffle.rate35}{0.83}
\@namedef{S@s3.px.contactq25.shuffle.u10}{0.97}
\@namedef{S@s3.px.contactq50.ahead}{2}
\@namedef{S@s3.px.contactq50.aheadcov}{3}
\@namedef{S@s3.px.contactq50.aheadrandom}{4}
\@namedef{S@s3.px.contactq50.behind}{3}
\@namedef{S@s3.px.contactq50.random}{14.9}
\@namedef{S@s3.px.contactq50.random.cov}{0.894}
\@namedef{S@s3.px.contactq50.random.early}{0.65}
\@namedef{S@s3.px.contactq50.random.rate}{0.62}
\@namedef{S@s3.px.contactq50.random.rate35}{0.62}
\@namedef{S@s3.px.contactq50.random.u10}{0.64}
\@namedef{S@s3.px.contactq50.rule}{14.8}
\@namedef{S@s3.px.contactq50.rule.cov}{0.902}
\@namedef{S@s3.px.contactq50.rule.early}{0.78}
\@namedef{S@s3.px.contactq50.rule.rate}{0.63}
\@namedef{S@s3.px.contactq50.rule.rate35}{0.63}
\@namedef{S@s3.px.contactq50.rule.u10}{0.78}
\@namedef{S@s3.px.contactq50.shuffle}{15.5}
\@namedef{S@s3.px.contactq50.shuffle.cov}{0.901}
\@namedef{S@s3.px.contactq50.shuffle.early}{0.78}
\@namedef{S@s3.px.contactq50.shuffle.rate}{0.64}
\@namedef{S@s3.px.contactq50.shuffle.rate35}{0.63}
\@namedef{S@s3.px.contactq50.shuffle.u10}{0.78}
\@namedef{S@s3.px.contactq75.ahead}{2}
\@namedef{S@s3.px.contactq75.aheadcov}{3}
\@namedef{S@s3.px.contactq75.aheadrandom}{3}
\@namedef{S@s3.px.contactq75.behind}{3}
\@namedef{S@s3.px.contactq75.random}{12.3}
\@namedef{S@s3.px.contactq75.random.cov}{0.877}
\@namedef{S@s3.px.contactq75.random.early}{0.39}
\@namedef{S@s3.px.contactq75.random.rate}{0.35}
\@namedef{S@s3.px.contactq75.random.rate35}{0.35}
\@namedef{S@s3.px.contactq75.random.u10}{0.38}
\@namedef{S@s3.px.contactq75.rule}{11.8}
\@namedef{S@s3.px.contactq75.rule.cov}{0.880}
\@namedef{S@s3.px.contactq75.rule.early}{0.46}
\@namedef{S@s3.px.contactq75.rule.rate}{0.35}
\@namedef{S@s3.px.contactq75.rule.rate35}{0.34}
\@namedef{S@s3.px.contactq75.rule.u10}{0.46}
\@namedef{S@s3.px.contactq75.shuffle}{12.3}
\@namedef{S@s3.px.contactq75.shuffle.cov}{0.877}
\@namedef{S@s3.px.contactq75.shuffle.early}{0.46}
\@namedef{S@s3.px.contactq75.shuffle.rate}{0.35}
\@namedef{S@s3.px.contactq75.shuffle.rate35}{0.34}
\@namedef{S@s3.px.contactq75.shuffle.u10}{0.46}
\@namedef{S@s3.px.contactq90.ahead}{3}
\@namedef{S@s3.px.contactq90.aheadcov}{3}
\@namedef{S@s3.px.contactq90.aheadrandom}{4}
\@namedef{S@s3.px.contactq90.behind}{2}
\@namedef{S@s3.px.contactq90.random}{9.8}
\@namedef{S@s3.px.contactq90.random.cov}{0.861}
\@namedef{S@s3.px.contactq90.random.early}{0.26}
\@namedef{S@s3.px.contactq90.random.rate}{0.22}
\@namedef{S@s3.px.contactq90.random.rate35}{0.22}
\@namedef{S@s3.px.contactq90.random.u10}{0.25}
\@namedef{S@s3.px.contactq90.rule}{11.0}
\@namedef{S@s3.px.contactq90.rule.cov}{0.871}
\@namedef{S@s3.px.contactq90.rule.early}{0.33}
\@namedef{S@s3.px.contactq90.rule.rate}{0.23}
\@namedef{S@s3.px.contactq90.rule.rate35}{0.22}
\@namedef{S@s3.px.contactq90.rule.u10}{0.32}
\@namedef{S@s3.px.contactq90.shuffle}{11.0}
\@namedef{S@s3.px.contactq90.shuffle.cov}{0.869}
\@namedef{S@s3.px.contactq90.shuffle.early}{0.33}
\@namedef{S@s3.px.contactq90.shuffle.rate}{0.23}
\@namedef{S@s3.px.contactq90.shuffle.rate35}{0.22}
\@namedef{S@s3.px.contactq90.shuffle.u10}{0.32}
\@namedef{S@s3.px.disagreementq25.ahead}{0}
\@namedef{S@s3.px.disagreementq25.aheadcov}{5}
\@namedef{S@s3.px.disagreementq25.aheadrandom}{3}
\@namedef{S@s3.px.disagreementq25.behind}{4}
\@namedef{S@s3.px.disagreementq25.random}{13.5}
\@namedef{S@s3.px.disagreementq25.random.cov}{0.885}
\@namedef{S@s3.px.disagreementq25.random.early}{0.49}
\@namedef{S@s3.px.disagreementq25.random.rate}{0.46}
\@namedef{S@s3.px.disagreementq25.random.rate35}{0.46}
\@namedef{S@s3.px.disagreementq25.random.u10}{0.49}
\@namedef{S@s3.px.disagreementq25.rule}{14.2}
\@namedef{S@s3.px.disagreementq25.rule.cov}{0.902}
\@namedef{S@s3.px.disagreementq25.rule.early}{0.57}
\@namedef{S@s3.px.disagreementq25.rule.rate}{0.47}
\@namedef{S@s3.px.disagreementq25.rule.rate35}{0.44}
\@namedef{S@s3.px.disagreementq25.rule.u10}{0.55}
\@namedef{S@s3.px.disagreementq25.shuffle}{15.2}
\@namedef{S@s3.px.disagreementq25.shuffle.cov}{0.895}
\@namedef{S@s3.px.disagreementq25.shuffle.early}{0.57}
\@namedef{S@s3.px.disagreementq25.shuffle.rate}{0.45}
\@namedef{S@s3.px.disagreementq25.shuffle.rate35}{0.44}
\@namedef{S@s3.px.disagreementq25.shuffle.u10}{0.55}
\@namedef{S@s3.px.disagreementq50.ahead}{3}
\@namedef{S@s3.px.disagreementq50.aheadcov}{5}
\@namedef{S@s3.px.disagreementq50.aheadrandom}{3}
\@namedef{S@s3.px.disagreementq50.behind}{2}
\@namedef{S@s3.px.disagreementq50.random}{11.9}
\@namedef{S@s3.px.disagreementq50.random.cov}{0.875}
\@namedef{S@s3.px.disagreementq50.random.early}{0.37}
\@namedef{S@s3.px.disagreementq50.random.rate}{0.34}
\@namedef{S@s3.px.disagreementq50.random.rate35}{0.33}
\@namedef{S@s3.px.disagreementq50.random.u10}{0.37}
\@namedef{S@s3.px.disagreementq50.rule}{13.6}
\@namedef{S@s3.px.disagreementq50.rule.cov}{0.887}
\@namedef{S@s3.px.disagreementq50.rule.early}{0.39}
\@namedef{S@s3.px.disagreementq50.rule.rate}{0.34}
\@namedef{S@s3.px.disagreementq50.rule.rate35}{0.32}
\@namedef{S@s3.px.disagreementq50.rule.u10}{0.38}
\@namedef{S@s3.px.disagreementq50.shuffle}{12.9}
\@namedef{S@s3.px.disagreementq50.shuffle.cov}{0.881}
\@namedef{S@s3.px.disagreementq50.shuffle.early}{0.39}
\@namedef{S@s3.px.disagreementq50.shuffle.rate}{0.32}
\@namedef{S@s3.px.disagreementq50.shuffle.rate35}{0.32}
\@namedef{S@s3.px.disagreementq50.shuffle.u10}{0.38}
\@namedef{S@s3.px.disagreementq75.ahead}{3}
\@namedef{S@s3.px.disagreementq75.aheadcov}{4}
\@namedef{S@s3.px.disagreementq75.aheadrandom}{5}
\@namedef{S@s3.px.disagreementq75.behind}{2}
\@namedef{S@s3.px.disagreementq75.random}{9.8}
\@namedef{S@s3.px.disagreementq75.random.cov}{0.862}
\@namedef{S@s3.px.disagreementq75.random.early}{0.26}
\@namedef{S@s3.px.disagreementq75.random.rate}{0.22}
\@namedef{S@s3.px.disagreementq75.random.rate35}{0.22}
\@namedef{S@s3.px.disagreementq75.random.u10}{0.25}
\@namedef{S@s3.px.disagreementq75.rule}{11.6}
\@namedef{S@s3.px.disagreementq75.rule.cov}{0.874}
\@namedef{S@s3.px.disagreementq75.rule.early}{0.28}
\@namedef{S@s3.px.disagreementq75.rule.rate}{0.23}
\@namedef{S@s3.px.disagreementq75.rule.rate35}{0.22}
\@namedef{S@s3.px.disagreementq75.rule.u10}{0.27}
\@namedef{S@s3.px.disagreementq75.shuffle}{10.8}
\@namedef{S@s3.px.disagreementq75.shuffle.cov}{0.866}
\@namedef{S@s3.px.disagreementq75.shuffle.early}{0.28}
\@namedef{S@s3.px.disagreementq75.shuffle.rate}{0.23}
\@namedef{S@s3.px.disagreementq75.shuffle.rate35}{0.22}
\@namedef{S@s3.px.disagreementq75.shuffle.u10}{0.27}
\@namedef{S@s3.px.disagreementq90.ahead}{2}
\@namedef{S@s3.px.disagreementq90.aheadcov}{3}
\@namedef{S@s3.px.disagreementq90.aheadrandom}{3}
\@namedef{S@s3.px.disagreementq90.behind}{3}
\@namedef{S@s3.px.disagreementq90.random}{9.8}
\@namedef{S@s3.px.disagreementq90.random.cov}{0.857}
\@namedef{S@s3.px.disagreementq90.random.early}{0.22}
\@namedef{S@s3.px.disagreementq90.random.rate}{0.19}
\@namedef{S@s3.px.disagreementq90.random.rate35}{0.19}
\@namedef{S@s3.px.disagreementq90.random.u10}{0.22}
\@namedef{S@s3.px.disagreementq90.rule}{10.2}
\@namedef{S@s3.px.disagreementq90.rule.cov}{0.861}
\@namedef{S@s3.px.disagreementq90.rule.early}{0.22}
\@namedef{S@s3.px.disagreementq90.rule.rate}{0.19}
\@namedef{S@s3.px.disagreementq90.rule.rate35}{0.19}
\@namedef{S@s3.px.disagreementq90.rule.u10}{0.22}
\@namedef{S@s3.px.disagreementq90.shuffle}{10.0}
\@namedef{S@s3.px.disagreementq90.shuffle.cov}{0.856}
\@namedef{S@s3.px.disagreementq90.shuffle.early}{0.22}
\@namedef{S@s3.px.disagreementq90.shuffle.rate}{0.19}
\@namedef{S@s3.px.disagreementq90.shuffle.rate35}{0.19}
\@namedef{S@s3.px.disagreementq90.shuffle.u10}{0.22}
\@namedef{S@s3.px.early.maxgap.random}{0.14}
\@namedef{S@s3.px.early.maxgap.shuffle}{0.01}
\@namedef{S@s3.px.errorq25.ahead}{3}
\@namedef{S@s3.px.errorq25.aheadcov}{5}
\@namedef{S@s3.px.errorq25.aheadrandom}{3}
\@namedef{S@s3.px.errorq25.behind}{2}
\@namedef{S@s3.px.errorq25.random}{14.6}
\@namedef{S@s3.px.errorq25.random.cov}{0.892}
\@namedef{S@s3.px.errorq25.random.early}{0.61}
\@namedef{S@s3.px.errorq25.random.rate}{0.59}
\@namedef{S@s3.px.errorq25.random.rate35}{0.58}
\@namedef{S@s3.px.errorq25.random.u10}{0.61}
\@namedef{S@s3.px.errorq25.rule}{15.4}
\@namedef{S@s3.px.errorq25.rule.cov}{0.903}
\@namedef{S@s3.px.errorq25.rule.early}{0.71}
\@namedef{S@s3.px.errorq25.rule.rate}{0.59}
\@namedef{S@s3.px.errorq25.rule.rate35}{0.55}
\@namedef{S@s3.px.errorq25.rule.u10}{0.69}
\@namedef{S@s3.px.errorq25.shuffle}{15.3}
\@namedef{S@s3.px.errorq25.shuffle.cov}{0.898}
\@namedef{S@s3.px.errorq25.shuffle.early}{0.70}
\@namedef{S@s3.px.errorq25.shuffle.rate}{0.56}
\@namedef{S@s3.px.errorq25.shuffle.rate35}{0.55}
\@namedef{S@s3.px.errorq25.shuffle.u10}{0.69}
\@namedef{S@s3.px.errorq50.ahead}{3}
\@namedef{S@s3.px.errorq50.aheadcov}{4}
\@namedef{S@s3.px.errorq50.aheadrandom}{4}
\@namedef{S@s3.px.errorq50.behind}{2}
\@namedef{S@s3.px.errorq50.random}{12.6}
\@namedef{S@s3.px.errorq50.random.cov}{0.880}
\@namedef{S@s3.px.errorq50.random.early}{0.41}
\@namedef{S@s3.px.errorq50.random.rate}{0.38}
\@namedef{S@s3.px.errorq50.random.rate35}{0.37}
\@namedef{S@s3.px.errorq50.random.u10}{0.41}
\@namedef{S@s3.px.errorq50.rule}{13.8}
\@namedef{S@s3.px.errorq50.rule.cov}{0.891}
\@namedef{S@s3.px.errorq50.rule.early}{0.45}
\@namedef{S@s3.px.errorq50.rule.rate}{0.38}
\@namedef{S@s3.px.errorq50.rule.rate35}{0.36}
\@namedef{S@s3.px.errorq50.rule.u10}{0.44}
\@namedef{S@s3.px.errorq50.shuffle}{13.4}
\@namedef{S@s3.px.errorq50.shuffle.cov}{0.885}
\@namedef{S@s3.px.errorq50.shuffle.early}{0.45}
\@namedef{S@s3.px.errorq50.shuffle.rate}{0.37}
\@namedef{S@s3.px.errorq50.shuffle.rate35}{0.36}
\@namedef{S@s3.px.errorq50.shuffle.u10}{0.44}
\@namedef{S@s3.px.errorq75.ahead}{2}
\@namedef{S@s3.px.errorq75.aheadcov}{4}
\@namedef{S@s3.px.errorq75.aheadrandom}{2}
\@namedef{S@s3.px.errorq75.behind}{3}
\@namedef{S@s3.px.errorq75.random}{10.7}
\@namedef{S@s3.px.errorq75.random.cov}{0.867}
\@namedef{S@s3.px.errorq75.random.early}{0.30}
\@namedef{S@s3.px.errorq75.random.rate}{0.26}
\@namedef{S@s3.px.errorq75.random.rate35}{0.26}
\@namedef{S@s3.px.errorq75.random.u10}{0.30}
\@namedef{S@s3.px.errorq75.rule}{10.8}
\@namedef{S@s3.px.errorq75.rule.cov}{0.874}
\@namedef{S@s3.px.errorq75.rule.early}{0.29}
\@namedef{S@s3.px.errorq75.rule.rate}{0.27}
\@namedef{S@s3.px.errorq75.rule.rate35}{0.26}
\@namedef{S@s3.px.errorq75.rule.u10}{0.29}
\@namedef{S@s3.px.errorq75.shuffle}{11.0}
\@namedef{S@s3.px.errorq75.shuffle.cov}{0.869}
\@namedef{S@s3.px.errorq75.shuffle.early}{0.29}
\@namedef{S@s3.px.errorq75.shuffle.rate}{0.26}
\@namedef{S@s3.px.errorq75.shuffle.rate35}{0.26}
\@namedef{S@s3.px.errorq75.shuffle.u10}{0.29}
\@namedef{S@s3.px.errorq90.ahead}{0}
\@namedef{S@s3.px.errorq90.aheadcov}{4}
\@namedef{S@s3.px.errorq90.aheadrandom}{1}
\@namedef{S@s3.px.errorq90.behind}{5}
\@namedef{S@s3.px.errorq90.random}{9.8}
\@namedef{S@s3.px.errorq90.random.cov}{0.858}
\@namedef{S@s3.px.errorq90.random.early}{0.23}
\@namedef{S@s3.px.errorq90.random.rate}{0.20}
\@namedef{S@s3.px.errorq90.random.rate35}{0.20}
\@namedef{S@s3.px.errorq90.random.u10}{0.23}
\@namedef{S@s3.px.errorq90.rule}{9.2}
\@namedef{S@s3.px.errorq90.rule.cov}{0.860}
\@namedef{S@s3.px.errorq90.rule.early}{0.23}
\@namedef{S@s3.px.errorq90.rule.rate}{0.21}
\@namedef{S@s3.px.errorq90.rule.rate35}{0.20}
\@namedef{S@s3.px.errorq90.rule.u10}{0.22}
\@namedef{S@s3.px.errorq90.shuffle}{9.8}
\@namedef{S@s3.px.errorq90.shuffle.cov}{0.857}
\@namedef{S@s3.px.errorq90.shuffle.early}{0.23}
\@namedef{S@s3.px.errorq90.shuffle.rate}{0.20}
\@namedef{S@s3.px.errorq90.shuffle.rate35}{0.20}
\@namedef{S@s3.px.errorq90.shuffle.u10}{0.22}
\@namedef{S@s3.px.final.F.ci}{+0.030 to +0.077}
\@namedef{S@s3.px.final.F.ci2}{+0.0296 to +0.0766}
\@namedef{S@s3.px.final.F.d}{+0.051}
\@namedef{S@s3.px.final.F.p}{<0.001}
\@namedef{S@s3.px.final.F.pp}{$p<0.001$}
\@namedef{S@s3.px.final.fixed1}{0.894}
\@namedef{S@s3.px.final.fixed4}{0.842}
\@namedef{S@s3.px.final95.F.ci}{+1.0 to +11.0}
\@namedef{S@s3.px.final95.F.ci2}{+1.00 to +11.00}
\@namedef{S@s3.px.final95.F.d}{+6.0}
\@namedef{S@s3.px.final95.F.p}{0.019}
\@namedef{S@s3.px.final95.F.pp}{$p=0.019$}
\@namedef{S@s3.px.final95.fixed1}{14.4}
\@namedef{S@s3.px.final95.fixed4}{8.4}
\@namedef{S@s3.px.geom.ahead}{1}
\@namedef{S@s3.px.geom.aheadcov}{2}
\@namedef{S@s3.px.geom.aheadrandom}{4}
\@namedef{S@s3.px.geom.behind}{4}
\@namedef{S@s3.px.geom.random}{10.7}
\@namedef{S@s3.px.geom.random.cov}{0.867}
\@namedef{S@s3.px.geom.random.early}{0.29}
\@namedef{S@s3.px.geom.random.rate}{0.26}
\@namedef{S@s3.px.geom.random.rate35}{0.26}
\@namedef{S@s3.px.geom.random.u10}{0.29}
\@namedef{S@s3.px.geom.rule}{11.8}
\@namedef{S@s3.px.geom.rule.cov}{0.888}
\@namedef{S@s3.px.geom.rule.early}{0.39}
\@namedef{S@s3.px.geom.rule.rate}{0.27}
\@namedef{S@s3.px.geom.rule.rate35}{0.26}
\@namedef{S@s3.px.geom.rule.u10}{0.39}
\@namedef{S@s3.px.geom.shuffle}{12.4}
\@namedef{S@s3.px.geom.shuffle.cov}{0.885}
\@namedef{S@s3.px.geom.shuffle.early}{0.39}
\@namedef{S@s3.px.geom.shuffle.rate}{0.27}
\@namedef{S@s3.px.geom.shuffle.rate35}{0.26}
\@namedef{S@s3.px.geom.shuffle.u10}{0.39}
\@namedef{S@s3.px.h8.min}{1.000}
\@namedef{S@s3.px.h8.nsig}{0}
\@namedef{S@s3.px.profmax}{1e-12}
\@namedef{S@s3.px.rate35.random.max}{+0.02}
\@namedef{S@s3.px.rate35.random.min}{\ensuremath{-}0.03}
\@namedef{S@s3.px.rr.contactq25.ci}{\ensuremath{-}2.8 to +2.5}
\@namedef{S@s3.px.rr.contactq25.ci2}{\ensuremath{-}2.75 to +2.46}
\@namedef{S@s3.px.rr.contactq25.d}{\ensuremath{-}0.2}
\@namedef{S@s3.px.rr.contactq25.p}{0.900}
\@namedef{S@s3.px.rr.contactq25.pp}{$p=0.900$}
\@namedef{S@s3.px.rr.contactq50.ci}{\ensuremath{-}3.6 to +3.3}
\@namedef{S@s3.px.rr.contactq50.ci2}{\ensuremath{-}3.60 to +3.28}
\@namedef{S@s3.px.rr.contactq50.d}{\ensuremath{-}0.1}
\@namedef{S@s3.px.rr.contactq50.p}{0.963}
\@namedef{S@s3.px.rr.contactq50.pp}{$p=0.963$}
\@namedef{S@s3.px.rr.contactq75.ci}{\ensuremath{-}3.9 to +2.8}
\@namedef{S@s3.px.rr.contactq75.ci2}{\ensuremath{-}3.90 to +2.82}
\@namedef{S@s3.px.rr.contactq75.d}{\ensuremath{-}0.5}
\@namedef{S@s3.px.rr.contactq75.p}{0.799}
\@namedef{S@s3.px.rr.contactq75.pp}{$p=0.799$}
\@namedef{S@s3.px.rr.contactq90.ci}{\ensuremath{-}1.9 to +4.6}
\@namedef{S@s3.px.rr.contactq90.ci2}{\ensuremath{-}1.89 to +4.58}
\@namedef{S@s3.px.rr.contactq90.d}{+1.2}
\@namedef{S@s3.px.rr.contactq90.p}{0.446}
\@namedef{S@s3.px.rr.contactq90.pp}{$p=0.446$}
\@namedef{S@s3.px.rr.disagreementq25.ci}{\ensuremath{-}2.6 to +4.2}
\@namedef{S@s3.px.rr.disagreementq25.ci2}{\ensuremath{-}2.64 to +4.16}
\@namedef{S@s3.px.rr.disagreementq25.d}{+0.7}
\@namedef{S@s3.px.rr.disagreementq25.p}{0.681}
\@namedef{S@s3.px.rr.disagreementq25.pp}{$p=0.681$}
\@namedef{S@s3.px.rr.disagreementq50.ci}{\ensuremath{-}1.4 to +5.1}
\@namedef{S@s3.px.rr.disagreementq50.ci2}{\ensuremath{-}1.40 to +5.11}
\@namedef{S@s3.px.rr.disagreementq50.d}{+1.7}
\@namedef{S@s3.px.rr.disagreementq50.p}{0.288}
\@namedef{S@s3.px.rr.disagreementq50.pp}{$p=0.288$}
\@namedef{S@s3.px.rr.disagreementq75.ci}{\ensuremath{-}0.9 to +4.8}
\@namedef{S@s3.px.rr.disagreementq75.ci2}{\ensuremath{-}0.94 to +4.83}
\@namedef{S@s3.px.rr.disagreementq75.d}{+1.8}
\@namedef{S@s3.px.rr.disagreementq75.p}{0.206}
\@namedef{S@s3.px.rr.disagreementq75.pp}{$p=0.206$}
\@namedef{S@s3.px.rr.disagreementq90.ci}{\ensuremath{-}1.3 to +2.4}
\@namedef{S@s3.px.rr.disagreementq90.ci2}{\ensuremath{-}1.30 to +2.44}
\@namedef{S@s3.px.rr.disagreementq90.d}{+0.3}
\@namedef{S@s3.px.rr.disagreementq90.p}{0.754}
\@namedef{S@s3.px.rr.disagreementq90.pp}{$p=0.754$}
\@namedef{S@s3.px.rr.errorq25.ci}{\ensuremath{-}3.2 to +4.9}
\@namedef{S@s3.px.rr.errorq25.ci2}{\ensuremath{-}3.17 to +4.91}
\@namedef{S@s3.px.rr.errorq25.d}{+0.8}
\@namedef{S@s3.px.rr.errorq25.p}{0.695}
\@namedef{S@s3.px.rr.errorq25.pp}{$p=0.695$}
\@namedef{S@s3.px.rr.errorq50.ci}{\ensuremath{-}2.2 to +4.8}
\@namedef{S@s3.px.rr.errorq50.ci2}{\ensuremath{-}2.18 to +4.84}
\@namedef{S@s3.px.rr.errorq50.d}{+1.2}
\@namedef{S@s3.px.rr.errorq50.p}{0.446}
\@namedef{S@s3.px.rr.errorq50.pp}{$p=0.446$}
\@namedef{S@s3.px.rr.errorq75.ci}{\ensuremath{-}2.5 to +2.8}
\@namedef{S@s3.px.rr.errorq75.ci2}{\ensuremath{-}2.52 to +2.79}
\@namedef{S@s3.px.rr.errorq75.d}{+0.1}
\@namedef{S@s3.px.rr.errorq75.p}{0.984}
\@namedef{S@s3.px.rr.errorq75.pp}{$p=0.984$}
\@namedef{S@s3.px.rr.errorq90.ci}{\ensuremath{-}2.0 to +0.9}
\@namedef{S@s3.px.rr.errorq90.ci2}{\ensuremath{-}1.99 to +0.90}
\@namedef{S@s3.px.rr.errorq90.d}{\ensuremath{-}0.6}
\@namedef{S@s3.px.rr.errorq90.p}{0.384}
\@namedef{S@s3.px.rr.errorq90.pp}{$p=0.384$}
\@namedef{S@s3.px.rr.geom.ci}{\ensuremath{-}2.6 to +4.7}
\@namedef{S@s3.px.rr.geom.ci2}{\ensuremath{-}2.58 to +4.71}
\@namedef{S@s3.px.rr.geom.d}{+1.1}
\@namedef{S@s3.px.rr.geom.p}{0.542}
\@namedef{S@s3.px.rr.geom.pp}{$p=0.542$}
\@namedef{S@s3.px.rrcov.contactq25.ci}{\ensuremath{-}0.001 to +0.008}
\@namedef{S@s3.px.rrcov.contactq25.ci2}{\ensuremath{-}0.0008 to +0.0079}
\@namedef{S@s3.px.rrcov.contactq25.d}{+0.003}
\@namedef{S@s3.px.rrcov.contactq25.p}{0.122}
\@namedef{S@s3.px.rrcov.contactq25.pp}{$p=0.122$}
\@namedef{S@s3.px.rrcov.contactq50.ci}{+0.0002 to +0.016}
\@namedef{S@s3.px.rrcov.contactq50.ci2}{+0.0002 to +0.0160}
\@namedef{S@s3.px.rrcov.contactq50.d}{+0.008}
\@namedef{S@s3.px.rrcov.contactq50.p}{0.044}
\@namedef{S@s3.px.rrcov.contactq50.pp}{$p=0.044$}
\@namedef{S@s3.px.rrcov.contactq75.ci}{\ensuremath{-}0.007 to +0.014}
\@namedef{S@s3.px.rrcov.contactq75.ci2}{\ensuremath{-}0.0075 to +0.0139}
\@namedef{S@s3.px.rrcov.contactq75.d}{+0.003}
\@namedef{S@s3.px.rrcov.contactq75.p}{0.545}
\@namedef{S@s3.px.rrcov.contactq75.pp}{$p=0.545$}
\@namedef{S@s3.px.rrcov.contactq90.ci}{\ensuremath{-}0.001 to +0.021}
\@namedef{S@s3.px.rrcov.contactq90.ci2}{\ensuremath{-}0.0011 to +0.0209}
\@namedef{S@s3.px.rrcov.contactq90.d}{+0.009}
\@namedef{S@s3.px.rrcov.contactq90.p}{0.084}
\@namedef{S@s3.px.rrcov.contactq90.pp}{$p=0.084$}
\@namedef{S@s3.px.rrcov.disagreementq25.ci}{+0.007 to +0.027}
\@namedef{S@s3.px.rrcov.disagreementq25.ci2}{+0.0073 to +0.0272}
\@namedef{S@s3.px.rrcov.disagreementq25.d}{+0.016}
\@namedef{S@s3.px.rrcov.disagreementq25.p}{0.001}
\@namedef{S@s3.px.rrcov.disagreementq25.pp}{$p=0.001$}
\@namedef{S@s3.px.rrcov.disagreementq50.ci}{+0.0002 to +0.023}
\@namedef{S@s3.px.rrcov.disagreementq50.ci2}{+0.0002 to +0.0233}
\@namedef{S@s3.px.rrcov.disagreementq50.d}{+0.011}
\@namedef{S@s3.px.rrcov.disagreementq50.p}{0.046}
\@namedef{S@s3.px.rrcov.disagreementq50.pp}{$p=0.046$}
\@namedef{S@s3.px.rrcov.disagreementq75.ci}{+0.001 to +0.026}
\@namedef{S@s3.px.rrcov.disagreementq75.ci2}{+0.0009 to +0.0257}
\@namedef{S@s3.px.rrcov.disagreementq75.d}{+0.013}
\@namedef{S@s3.px.rrcov.disagreementq75.p}{0.037}
\@namedef{S@s3.px.rrcov.disagreementq75.pp}{$p=0.037$}
\@namedef{S@s3.px.rrcov.disagreementq90.ci}{\ensuremath{-}0.005 to +0.019}
\@namedef{S@s3.px.rrcov.disagreementq90.ci2}{\ensuremath{-}0.0045 to +0.0186}
\@namedef{S@s3.px.rrcov.disagreementq90.d}{+0.004}
\@namedef{S@s3.px.rrcov.disagreementq90.p}{0.518}
\@namedef{S@s3.px.rrcov.disagreementq90.pp}{$p=0.518$}
\@namedef{S@s3.px.rrcov.errorq25.ci}{+0.003 to +0.019}
\@namedef{S@s3.px.rrcov.errorq25.ci2}{+0.0025 to +0.0189}
\@namedef{S@s3.px.rrcov.errorq25.d}{+0.011}
\@namedef{S@s3.px.rrcov.errorq25.p}{0.010}
\@namedef{S@s3.px.rrcov.errorq25.pp}{$p=0.010$}
\@namedef{S@s3.px.rrcov.errorq50.ci}{+0.001 to +0.022}
\@namedef{S@s3.px.rrcov.errorq50.ci2}{+0.0015 to +0.0224}
\@namedef{S@s3.px.rrcov.errorq50.d}{+0.011}
\@namedef{S@s3.px.rrcov.errorq50.p}{0.025}
\@namedef{S@s3.px.rrcov.errorq50.pp}{$p=0.025$}
\@namedef{S@s3.px.rrcov.errorq75.ci}{\ensuremath{-}0.004 to +0.017}
\@namedef{S@s3.px.rrcov.errorq75.ci2}{\ensuremath{-}0.0044 to +0.0171}
\@namedef{S@s3.px.rrcov.errorq75.d}{+0.006}
\@namedef{S@s3.px.rrcov.errorq75.p}{0.235}
\@namedef{S@s3.px.rrcov.errorq75.pp}{$p=0.235$}
\@namedef{S@s3.px.rrcov.errorq90.ci}{\ensuremath{-}0.007 to +0.011}
\@namedef{S@s3.px.rrcov.errorq90.ci2}{\ensuremath{-}0.0068 to +0.0111}
\@namedef{S@s3.px.rrcov.errorq90.d}{+0.002}
\@namedef{S@s3.px.rrcov.errorq90.p}{0.731}
\@namedef{S@s3.px.rrcov.errorq90.pp}{$p=0.731$}
\@namedef{S@s3.px.rrcov.geom.ci}{+0.008 to +0.037}
\@namedef{S@s3.px.rrcov.geom.ci2}{+0.0078 to +0.0372}
\@namedef{S@s3.px.rrcov.geom.d}{+0.021}
\@namedef{S@s3.px.rrcov.geom.p}{<0.001}
\@namedef{S@s3.px.rrcov.geom.pp}{$p<0.001$}
\@namedef{S@s3.px.rs.contactq25.ci}{\ensuremath{-}1.1 to +1.3}
\@namedef{S@s3.px.rs.contactq25.ci2}{\ensuremath{-}1.09 to +1.32}
\@namedef{S@s3.px.rs.contactq25.d}{+0.0}
\@namedef{S@s3.px.rs.contactq25.h13}{1.000}
\@namedef{S@s3.px.rs.contactq25.p}{0.983}
\@namedef{S@s3.px.rs.contactq25.pp}{$p=0.983$}
\@namedef{S@s3.px.rs.contactq50.ci}{\ensuremath{-}3.5 to +2.1}
\@namedef{S@s3.px.rs.contactq50.ci2}{\ensuremath{-}3.49 to +2.07}
\@namedef{S@s3.px.rs.contactq50.d}{\ensuremath{-}0.7}
\@namedef{S@s3.px.rs.contactq50.h13}{1.000}
\@namedef{S@s3.px.rs.contactq50.p}{0.582}
\@namedef{S@s3.px.rs.contactq50.pp}{$p=0.582$}
\@namedef{S@s3.px.rs.contactq75.ci}{\ensuremath{-}4.0 to +2.8}
\@namedef{S@s3.px.rs.contactq75.ci2}{\ensuremath{-}3.98 to +2.82}
\@namedef{S@s3.px.rs.contactq75.d}{\ensuremath{-}0.5}
\@namedef{S@s3.px.rs.contactq75.h13}{1.000}
\@namedef{S@s3.px.rs.contactq75.h8}{1.000}
\@namedef{S@s3.px.rs.contactq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rs.contactq75.p}{0.790}
\@namedef{S@s3.px.rs.contactq75.pp}{$p=0.790$}
\@namedef{S@s3.px.rs.contactq90.ci}{\ensuremath{-}3.3 to +3.4}
\@namedef{S@s3.px.rs.contactq90.ci2}{\ensuremath{-}3.28 to +3.36}
\@namedef{S@s3.px.rs.contactq90.d}{+0.0}
\@namedef{S@s3.px.rs.contactq90.h13}{1.000}
\@namedef{S@s3.px.rs.contactq90.p}{0.995}
\@namedef{S@s3.px.rs.contactq90.pp}{$p=0.995$}
\@namedef{S@s3.px.rs.disagreementq25.ci}{\ensuremath{-}4.2 to +2.1}
\@namedef{S@s3.px.rs.disagreementq25.ci2}{\ensuremath{-}4.24 to +2.10}
\@namedef{S@s3.px.rs.disagreementq25.d}{\ensuremath{-}1.0}
\@namedef{S@s3.px.rs.disagreementq25.h13}{1.000}
\@namedef{S@s3.px.rs.disagreementq25.p}{0.546}
\@namedef{S@s3.px.rs.disagreementq25.pp}{$p=0.546$}
\@namedef{S@s3.px.rs.disagreementq50.ci}{\ensuremath{-}2.6 to +4.3}
\@namedef{S@s3.px.rs.disagreementq50.ci2}{\ensuremath{-}2.55 to +4.26}
\@namedef{S@s3.px.rs.disagreementq50.d}{+0.7}
\@namedef{S@s3.px.rs.disagreementq50.h13}{1.000}
\@namedef{S@s3.px.rs.disagreementq50.p}{0.679}
\@namedef{S@s3.px.rs.disagreementq50.pp}{$p=0.679$}
\@namedef{S@s3.px.rs.disagreementq75.ci}{\ensuremath{-}1.7 to +3.7}
\@namedef{S@s3.px.rs.disagreementq75.ci2}{\ensuremath{-}1.74 to +3.72}
\@namedef{S@s3.px.rs.disagreementq75.d}{+0.8}
\@namedef{S@s3.px.rs.disagreementq75.h13}{1.000}
\@namedef{S@s3.px.rs.disagreementq75.h8}{1.000}
\@namedef{S@s3.px.rs.disagreementq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rs.disagreementq75.p}{0.547}
\@namedef{S@s3.px.rs.disagreementq75.pp}{$p=0.547$}
\@namedef{S@s3.px.rs.disagreementq90.ci}{\ensuremath{-}1.3 to +2.1}
\@namedef{S@s3.px.rs.disagreementq90.ci2}{\ensuremath{-}1.26 to +2.08}
\@namedef{S@s3.px.rs.disagreementq90.d}{+0.2}
\@namedef{S@s3.px.rs.disagreementq90.h13}{1.000}
\@namedef{S@s3.px.rs.disagreementq90.p}{0.839}
\@namedef{S@s3.px.rs.disagreementq90.pp}{$p=0.839$}
\@namedef{S@s3.px.rs.dmax}{+0.8}
\@namedef{S@s3.px.rs.dmin}{\ensuremath{-}1.0}
\@namedef{S@s3.px.rs.errorq25.ci}{\ensuremath{-}4.0 to +4.6}
\@namedef{S@s3.px.rs.errorq25.ci2}{\ensuremath{-}4.02 to +4.59}
\@namedef{S@s3.px.rs.errorq25.d}{+0.1}
\@namedef{S@s3.px.rs.errorq25.h13}{1.000}
\@namedef{S@s3.px.rs.errorq25.p}{0.971}
\@namedef{S@s3.px.rs.errorq25.pp}{$p=0.971$}
\@namedef{S@s3.px.rs.errorq50.ci}{\ensuremath{-}2.8 to +3.7}
\@namedef{S@s3.px.rs.errorq50.ci2}{\ensuremath{-}2.78 to +3.70}
\@namedef{S@s3.px.rs.errorq50.d}{+0.4}
\@namedef{S@s3.px.rs.errorq50.h13}{1.000}
\@namedef{S@s3.px.rs.errorq50.p}{0.797}
\@namedef{S@s3.px.rs.errorq50.pp}{$p=0.797$}
\@namedef{S@s3.px.rs.errorq75.ci}{\ensuremath{-}2.8 to +2.4}
\@namedef{S@s3.px.rs.errorq75.ci2}{\ensuremath{-}2.81 to +2.44}
\@namedef{S@s3.px.rs.errorq75.d}{\ensuremath{-}0.2}
\@namedef{S@s3.px.rs.errorq75.h13}{1.000}
\@namedef{S@s3.px.rs.errorq75.h8}{1.000}
\@namedef{S@s3.px.rs.errorq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rs.errorq75.p}{0.888}
\@namedef{S@s3.px.rs.errorq75.pp}{$p=0.888$}
\@namedef{S@s3.px.rs.errorq90.ci}{\ensuremath{-}1.8 to +0.6}
\@namedef{S@s3.px.rs.errorq90.ci2}{\ensuremath{-}1.83 to +0.55}
\@namedef{S@s3.px.rs.errorq90.d}{\ensuremath{-}0.6}
\@namedef{S@s3.px.rs.errorq90.h13}{1.000}
\@namedef{S@s3.px.rs.errorq90.p}{0.256}
\@namedef{S@s3.px.rs.errorq90.pp}{$p=0.256$}
\@namedef{S@s3.px.rs.geom.ci}{\ensuremath{-}3.2 to +1.9}
\@namedef{S@s3.px.rs.geom.ci2}{\ensuremath{-}3.24 to +1.95}
\@namedef{S@s3.px.rs.geom.d}{\ensuremath{-}0.7}
\@namedef{S@s3.px.rs.geom.h13}{1.000}
\@namedef{S@s3.px.rs.geom.h8}{1.000}
\@namedef{S@s3.px.rs.geom.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rs.geom.p}{0.624}
\@namedef{S@s3.px.rs.geom.pp}{$p=0.624$}
\@namedef{S@s3.px.rs.hi}{+4.6}
\@namedef{S@s3.px.rs.lo}{\ensuremath{-}4.2}
\@namedef{S@s3.px.rs.ndpos}{7}
\@namedef{S@s3.px.rs.nholm}{0}
\@namedef{S@s3.px.rs.nneg}{0}
\@namedef{S@s3.px.rs.npos}{0}
\@namedef{S@s3.px.rs.prim.dmax}{+0.8}
\@namedef{S@s3.px.rs.prim.dmin}{\ensuremath{-}0.7}
\@namedef{S@s3.px.rs.prim.hi}{+3.7}
\@namedef{S@s3.px.rs.prim.lo}{\ensuremath{-}4.0}
\@namedef{S@s3.px.rs.prim.npos}{0}
\@namedef{S@s3.px.rs.prim.nsig}{0}
\@namedef{S@s3.px.rscov.contactq25.ci}{\ensuremath{-}0.002 to +0.002}
\@namedef{S@s3.px.rscov.contactq25.ci2}{\ensuremath{-}0.0016 to +0.0021}
\@namedef{S@s3.px.rscov.contactq25.d}{+0.000}
\@namedef{S@s3.px.rscov.contactq25.h13}{1.000}
\@namedef{S@s3.px.rscov.contactq25.p}{0.940}
\@namedef{S@s3.px.rscov.contactq25.pp}{$p=0.940$}
\@namedef{S@s3.px.rscov.contactq50.ci}{\ensuremath{-}0.005 to +0.005}
\@namedef{S@s3.px.rscov.contactq50.ci2}{\ensuremath{-}0.0046 to +0.0048}
\@namedef{S@s3.px.rscov.contactq50.d}{+0.000}
\@namedef{S@s3.px.rscov.contactq50.h13}{1.000}
\@namedef{S@s3.px.rscov.contactq50.p}{0.842}
\@namedef{S@s3.px.rscov.contactq50.pp}{$p=0.842$}
\@namedef{S@s3.px.rscov.contactq75.ci}{\ensuremath{-}0.007 to +0.012}
\@namedef{S@s3.px.rscov.contactq75.ci2}{\ensuremath{-}0.0075 to +0.0125}
\@namedef{S@s3.px.rscov.contactq75.d}{+0.003}
\@namedef{S@s3.px.rscov.contactq75.h13}{1.000}
\@namedef{S@s3.px.rscov.contactq75.h8}{1.000}
\@namedef{S@s3.px.rscov.contactq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rscov.contactq75.p}{0.524}
\@namedef{S@s3.px.rscov.contactq75.pp}{$p=0.524$}
\@namedef{S@s3.px.rscov.contactq90.ci}{\ensuremath{-}0.009 to +0.013}
\@namedef{S@s3.px.rscov.contactq90.ci2}{\ensuremath{-}0.0089 to +0.0131}
\@namedef{S@s3.px.rscov.contactq90.d}{+0.002}
\@namedef{S@s3.px.rscov.contactq90.h13}{1.000}
\@namedef{S@s3.px.rscov.contactq90.p}{0.693}
\@namedef{S@s3.px.rscov.contactq90.pp}{$p=0.693$}
\@namedef{S@s3.px.rscov.disagreementq25.ci}{+0.001 to +0.015}
\@namedef{S@s3.px.rscov.disagreementq25.ci2}{+0.0006 to +0.0148}
\@namedef{S@s3.px.rscov.disagreementq25.d}{+0.007}
\@namedef{S@s3.px.rscov.disagreementq25.h13}{0.416}
\@namedef{S@s3.px.rscov.disagreementq25.p}{0.032}
\@namedef{S@s3.px.rscov.disagreementq25.pp}{$p=0.032$}
\@namedef{S@s3.px.rscov.disagreementq50.ci}{\ensuremath{-}0.003 to +0.017}
\@namedef{S@s3.px.rscov.disagreementq50.ci2}{\ensuremath{-}0.0034 to +0.0174}
\@namedef{S@s3.px.rscov.disagreementq50.d}{+0.006}
\@namedef{S@s3.px.rscov.disagreementq50.h13}{1.000}
\@namedef{S@s3.px.rscov.disagreementq50.p}{0.215}
\@namedef{S@s3.px.rscov.disagreementq50.pp}{$p=0.215$}
\@namedef{S@s3.px.rscov.disagreementq75.ci}{\ensuremath{-}0.004 to +0.021}
\@namedef{S@s3.px.rscov.disagreementq75.ci2}{\ensuremath{-}0.0043 to +0.0214}
\@namedef{S@s3.px.rscov.disagreementq75.d}{+0.008}
\@namedef{S@s3.px.rscov.disagreementq75.h13}{1.000}
\@namedef{S@s3.px.rscov.disagreementq75.h8}{1.000}
\@namedef{S@s3.px.rscov.disagreementq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rscov.disagreementq75.p}{0.200}
\@namedef{S@s3.px.rscov.disagreementq75.pp}{$p=0.200$}
\@namedef{S@s3.px.rscov.disagreementq90.ci}{\ensuremath{-}0.004 to +0.018}
\@namedef{S@s3.px.rscov.disagreementq90.ci2}{\ensuremath{-}0.0042 to +0.0175}
\@namedef{S@s3.px.rscov.disagreementq90.d}{+0.004}
\@namedef{S@s3.px.rscov.disagreementq90.h13}{1.000}
\@namedef{S@s3.px.rscov.disagreementq90.p}{0.440}
\@namedef{S@s3.px.rscov.disagreementq90.pp}{$p=0.440$}
\@namedef{S@s3.px.rscov.dmax}{+0.008}
\@namedef{S@s3.px.rscov.dmin}{+0.000}
\@namedef{S@s3.px.rscov.errorq25.ci}{\ensuremath{-}0.001 to +0.011}
\@namedef{S@s3.px.rscov.errorq25.ci2}{\ensuremath{-}0.0008 to +0.0114}
\@namedef{S@s3.px.rscov.errorq25.d}{+0.005}
\@namedef{S@s3.px.rscov.errorq25.h13}{1.000}
\@namedef{S@s3.px.rscov.errorq25.p}{0.087}
\@namedef{S@s3.px.rscov.errorq25.pp}{$p=0.087$}
\@namedef{S@s3.px.rscov.errorq50.ci}{\ensuremath{-}0.005 to +0.017}
\@namedef{S@s3.px.rscov.errorq50.ci2}{\ensuremath{-}0.0048 to +0.0167}
\@namedef{S@s3.px.rscov.errorq50.d}{+0.006}
\@namedef{S@s3.px.rscov.errorq50.h13}{1.000}
\@namedef{S@s3.px.rscov.errorq50.p}{0.261}
\@namedef{S@s3.px.rscov.errorq50.pp}{$p=0.261$}
\@namedef{S@s3.px.rscov.errorq75.ci}{\ensuremath{-}0.007 to +0.016}
\@namedef{S@s3.px.rscov.errorq75.ci2}{\ensuremath{-}0.0068 to +0.0160}
\@namedef{S@s3.px.rscov.errorq75.d}{+0.005}
\@namedef{S@s3.px.rscov.errorq75.h13}{1.000}
\@namedef{S@s3.px.rscov.errorq75.h8}{1.000}
\@namedef{S@s3.px.rscov.errorq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rscov.errorq75.p}{0.428}
\@namedef{S@s3.px.rscov.errorq75.pp}{$p=0.428$}
\@namedef{S@s3.px.rscov.errorq90.ci}{\ensuremath{-}0.006 to +0.013}
\@namedef{S@s3.px.rscov.errorq90.ci2}{\ensuremath{-}0.0064 to +0.0133}
\@namedef{S@s3.px.rscov.errorq90.d}{+0.002}
\@namedef{S@s3.px.rscov.errorq90.h13}{1.000}
\@namedef{S@s3.px.rscov.errorq90.p}{0.618}
\@namedef{S@s3.px.rscov.errorq90.pp}{$p=0.618$}
\@namedef{S@s3.px.rscov.geom.ci}{\ensuremath{-}0.007 to +0.016}
\@namedef{S@s3.px.rscov.geom.ci2}{\ensuremath{-}0.0070 to +0.0163}
\@namedef{S@s3.px.rscov.geom.d}{+0.003}
\@namedef{S@s3.px.rscov.geom.h13}{1.000}
\@namedef{S@s3.px.rscov.geom.h8}{1.000}
\@namedef{S@s3.px.rscov.geom.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.px.rscov.geom.p}{0.693}
\@namedef{S@s3.px.rscov.geom.pp}{$p=0.693$}
\@namedef{S@s3.px.rscov.hi}{+0.021}
\@namedef{S@s3.px.rscov.lo}{\ensuremath{-}0.009}
\@namedef{S@s3.px.rscov.ndpos}{13}
\@namedef{S@s3.px.rscov.nholm}{0}
\@namedef{S@s3.px.rscov.nneg}{0}
\@namedef{S@s3.px.rscov.npos}{1}
\@namedef{S@s3.px.rscov.prim.dmax}{+0.008}
\@namedef{S@s3.px.rscov.prim.dmin}{+0.003}
\@namedef{S@s3.px.rscov.prim.hi}{+0.021}
\@namedef{S@s3.px.rscov.prim.lo}{\ensuremath{-}0.007}
\@namedef{S@s3.px.rscov.prim.npos}{0}
\@namedef{S@s3.px.rscov.prim.nsig}{0}
\@namedef{S@s3.px.seeds}{5}
\@namedef{S@s3.px.sr.contactq25.ci}{\ensuremath{-}2.6 to +2.3}
\@namedef{S@s3.px.sr.contactq25.ci2}{\ensuremath{-}2.58 to +2.33}
\@namedef{S@s3.px.sr.contactq25.d}{\ensuremath{-}0.2}
\@namedef{S@s3.px.sr.contactq25.h13}{1.000}
\@namedef{S@s3.px.sr.contactq25.p}{0.869}
\@namedef{S@s3.px.sr.contactq25.pp}{$p=0.869$}
\@namedef{S@s3.px.sr.contactq50.ci}{\ensuremath{-}1.7 to +2.8}
\@namedef{S@s3.px.sr.contactq50.ci2}{\ensuremath{-}1.68 to +2.80}
\@namedef{S@s3.px.sr.contactq50.d}{+0.6}
\@namedef{S@s3.px.sr.contactq50.h13}{1.000}
\@namedef{S@s3.px.sr.contactq50.p}{0.588}
\@namedef{S@s3.px.sr.contactq50.pp}{$p=0.588$}
\@namedef{S@s3.px.sr.contactq75.ci}{\ensuremath{-}1.4 to +1.5}
\@namedef{S@s3.px.sr.contactq75.ci2}{\ensuremath{-}1.40 to +1.47}
\@namedef{S@s3.px.sr.contactq75.d}{+0.0}
\@namedef{S@s3.px.sr.contactq75.h13}{1.000}
\@namedef{S@s3.px.sr.contactq75.p}{0.959}
\@namedef{S@s3.px.sr.contactq75.pp}{$p=0.959$}
\@namedef{S@s3.px.sr.contactq90.ci}{+0.2 to +2.3}
\@namedef{S@s3.px.sr.contactq90.ci2}{+0.15 to +2.34}
\@namedef{S@s3.px.sr.contactq90.d}{+1.2}
\@namedef{S@s3.px.sr.contactq90.h13}{0.341}
\@namedef{S@s3.px.sr.contactq90.p}{0.026}
\@namedef{S@s3.px.sr.contactq90.pp}{$p=0.026$}
\@namedef{S@s3.px.sr.disagreementq25.ci}{\ensuremath{-}0.2 to +3.8}
\@namedef{S@s3.px.sr.disagreementq25.ci2}{\ensuremath{-}0.23 to +3.75}
\@namedef{S@s3.px.sr.disagreementq25.d}{+1.7}
\@namedef{S@s3.px.sr.disagreementq25.h13}{0.964}
\@namedef{S@s3.px.sr.disagreementq25.p}{0.088}
\@namedef{S@s3.px.sr.disagreementq25.pp}{$p=0.088$}
\@namedef{S@s3.px.sr.disagreementq50.ci}{\ensuremath{-}0.4 to +2.7}
\@namedef{S@s3.px.sr.disagreementq50.ci2}{\ensuremath{-}0.38 to +2.67}
\@namedef{S@s3.px.sr.disagreementq50.d}{+1.0}
\@namedef{S@s3.px.sr.disagreementq50.h13}{1.000}
\@namedef{S@s3.px.sr.disagreementq50.p}{0.172}
\@namedef{S@s3.px.sr.disagreementq50.pp}{$p=0.172$}
\@namedef{S@s3.px.sr.disagreementq75.ci}{\ensuremath{-}0.1 to +2.1}
\@namedef{S@s3.px.sr.disagreementq75.ci2}{\ensuremath{-}0.09 to +2.15}
\@namedef{S@s3.px.sr.disagreementq75.d}{+1.0}
\@namedef{S@s3.px.sr.disagreementq75.h13}{0.883}
\@namedef{S@s3.px.sr.disagreementq75.p}{0.074}
\@namedef{S@s3.px.sr.disagreementq75.pp}{$p=0.074$}
\@namedef{S@s3.px.sr.disagreementq90.ci}{\ensuremath{-}0.5 to +0.8}
\@namedef{S@s3.px.sr.disagreementq90.ci2}{\ensuremath{-}0.48 to +0.79}
\@namedef{S@s3.px.sr.disagreementq90.d}{+0.1}
\@namedef{S@s3.px.sr.disagreementq90.h13}{1.000}
\@namedef{S@s3.px.sr.disagreementq90.p}{0.682}
\@namedef{S@s3.px.sr.disagreementq90.pp}{$p=0.682$}
\@namedef{S@s3.px.sr.dmax}{+1.8}
\@namedef{S@s3.px.sr.dmin}{\ensuremath{-}0.2}
\@namedef{S@s3.px.sr.errorq25.ci}{\ensuremath{-}1.1 to +2.5}
\@namedef{S@s3.px.sr.errorq25.ci2}{\ensuremath{-}1.09 to +2.48}
\@namedef{S@s3.px.sr.errorq25.d}{+0.7}
\@namedef{S@s3.px.sr.errorq25.h13}{1.000}
\@namedef{S@s3.px.sr.errorq25.p}{0.456}
\@namedef{S@s3.px.sr.errorq25.pp}{$p=0.456$}
\@namedef{S@s3.px.sr.errorq50.ci}{\ensuremath{-}0.3 to +2.1}
\@namedef{S@s3.px.sr.errorq50.ci2}{\ensuremath{-}0.31 to +2.12}
\@namedef{S@s3.px.sr.errorq50.d}{+0.9}
\@namedef{S@s3.px.sr.errorq50.h13}{1.000}
\@namedef{S@s3.px.sr.errorq50.p}{0.143}
\@namedef{S@s3.px.sr.errorq50.pp}{$p=0.143$}
\@namedef{S@s3.px.sr.errorq75.ci}{\ensuremath{-}1.0 to +1.5}
\@namedef{S@s3.px.sr.errorq75.ci2}{\ensuremath{-}0.95 to +1.48}
\@namedef{S@s3.px.sr.errorq75.d}{+0.2}
\@namedef{S@s3.px.sr.errorq75.h13}{1.000}
\@namedef{S@s3.px.sr.errorq75.p}{0.721}
\@namedef{S@s3.px.sr.errorq75.pp}{$p=0.721$}
\@namedef{S@s3.px.sr.errorq90.ci}{\ensuremath{-}0.7 to +0.9}
\@namedef{S@s3.px.sr.errorq90.ci2}{\ensuremath{-}0.71 to +0.89}
\@namedef{S@s3.px.sr.errorq90.d}{+0.0}
\@namedef{S@s3.px.sr.errorq90.h13}{1.000}
\@namedef{S@s3.px.sr.errorq90.p}{0.980}
\@namedef{S@s3.px.sr.errorq90.pp}{$p=0.980$}
\@namedef{S@s3.px.sr.geom.ci}{\ensuremath{-}0.7 to +4.4}
\@namedef{S@s3.px.sr.geom.ci2}{\ensuremath{-}0.69 to +4.44}
\@namedef{S@s3.px.sr.geom.d}{+1.8}
\@namedef{S@s3.px.sr.geom.h13}{1.000}
\@namedef{S@s3.px.sr.geom.p}{0.162}
\@namedef{S@s3.px.sr.geom.pp}{$p=0.162$}
\@namedef{S@s3.px.sr.hi}{+4.4}
\@namedef{S@s3.px.sr.lo}{\ensuremath{-}2.6}
\@namedef{S@s3.px.sr.ndpos}{12}
\@namedef{S@s3.px.sr.nholm}{0}
\@namedef{S@s3.px.sr.nneg}{0}
\@namedef{S@s3.px.sr.npos}{1}
\@namedef{S@s3.px.sr.prim.dmax}{+1.8}
\@namedef{S@s3.px.sr.prim.dmin}{+0.0}
\@namedef{S@s3.px.sr.prim.hi}{+4.4}
\@namedef{S@s3.px.sr.prim.lo}{\ensuremath{-}1.4}
\@namedef{S@s3.px.sr.prim.npos}{0}
\@namedef{S@s3.px.sr.prim.nsig}{0}
\@namedef{S@s3.px.srcov.contactq25.ci}{\ensuremath{-}0.001 to +0.008}
\@namedef{S@s3.px.srcov.contactq25.ci2}{\ensuremath{-}0.0009 to +0.0078}
\@namedef{S@s3.px.srcov.contactq25.d}{+0.003}
\@namedef{S@s3.px.srcov.contactq25.h13}{0.805}
\@namedef{S@s3.px.srcov.contactq25.p}{0.134}
\@namedef{S@s3.px.srcov.contactq25.pp}{$p=0.134$}
\@namedef{S@s3.px.srcov.contactq50.ci}{+0.002 to +0.014}
\@namedef{S@s3.px.srcov.contactq50.ci2}{+0.0018 to +0.0140}
\@namedef{S@s3.px.srcov.contactq50.d}{+0.008}
\@namedef{S@s3.px.srcov.contactq50.h13}{0.095}
\@namedef{S@s3.px.srcov.contactq50.p}{0.011}
\@namedef{S@s3.px.srcov.contactq50.pp}{$p=0.011$}
\@namedef{S@s3.px.srcov.contactq75.ci}{\ensuremath{-}0.004 to +0.005}
\@namedef{S@s3.px.srcov.contactq75.ci2}{\ensuremath{-}0.0041 to +0.0045}
\@namedef{S@s3.px.srcov.contactq75.d}{+0.000}
\@namedef{S@s3.px.srcov.contactq75.h13}{1.000}
\@namedef{S@s3.px.srcov.contactq75.p}{0.927}
\@namedef{S@s3.px.srcov.contactq75.pp}{$p=0.927$}
\@namedef{S@s3.px.srcov.contactq90.ci}{+0.004 to +0.011}
\@namedef{S@s3.px.srcov.contactq90.ci2}{+0.0039 to +0.0106}
\@namedef{S@s3.px.srcov.contactq90.d}{+0.007}
\@namedef{S@s3.px.srcov.contactq90.h13}{0.001}
\@namedef{S@s3.px.srcov.contactq90.p}{<0.001}
\@namedef{S@s3.px.srcov.contactq90.pp}{$p<0.001$}
\@namedef{S@s3.px.srcov.disagreementq25.ci}{+0.003 to +0.018}
\@namedef{S@s3.px.srcov.disagreementq25.ci2}{+0.0031 to +0.0177}
\@namedef{S@s3.px.srcov.disagreementq25.d}{+0.009}
\@namedef{S@s3.px.srcov.disagreementq25.h13}{0.026}
\@namedef{S@s3.px.srcov.disagreementq25.p}{0.002}
\@namedef{S@s3.px.srcov.disagreementq25.pp}{$p=0.002$}
\@namedef{S@s3.px.srcov.disagreementq50.ci}{\ensuremath{-}0.003 to +0.014}
\@namedef{S@s3.px.srcov.disagreementq50.ci2}{\ensuremath{-}0.0029 to +0.0145}
\@namedef{S@s3.px.srcov.disagreementq50.d}{+0.005}
\@namedef{S@s3.px.srcov.disagreementq50.h13}{1.000}
\@namedef{S@s3.px.srcov.disagreementq50.p}{0.214}
\@namedef{S@s3.px.srcov.disagreementq50.pp}{$p=0.214$}
\@namedef{S@s3.px.srcov.disagreementq75.ci}{+0.001 to +0.010}
\@namedef{S@s3.px.srcov.disagreementq75.ci2}{+0.0006 to +0.0100}
\@namedef{S@s3.px.srcov.disagreementq75.d}{+0.005}
\@namedef{S@s3.px.srcov.disagreementq75.h13}{0.182}
\@namedef{S@s3.px.srcov.disagreementq75.p}{0.026}
\@namedef{S@s3.px.srcov.disagreementq75.pp}{$p=0.026$}
\@namedef{S@s3.px.srcov.disagreementq90.ci}{\ensuremath{-}0.004 to +0.002}
\@namedef{S@s3.px.srcov.disagreementq90.ci2}{\ensuremath{-}0.0036 to +0.0024}
\@namedef{S@s3.px.srcov.disagreementq90.d}{\ensuremath{-}0.000}
\@namedef{S@s3.px.srcov.disagreementq90.h13}{1.000}
\@namedef{S@s3.px.srcov.disagreementq90.p}{0.989}
\@namedef{S@s3.px.srcov.disagreementq90.pp}{$p=0.989$}
\@namedef{S@s3.px.srcov.dmax}{+0.018}
\@namedef{S@s3.px.srcov.dmin}{\ensuremath{-}0.001}
\@namedef{S@s3.px.srcov.errorq25.ci}{+0.001 to +0.010}
\@namedef{S@s3.px.srcov.errorq25.ci2}{+0.0014 to +0.0098}
\@namedef{S@s3.px.srcov.errorq25.d}{+0.005}
\@namedef{S@s3.px.srcov.errorq25.h13}{0.086}
\@namedef{S@s3.px.srcov.errorq25.p}{0.009}
\@namedef{S@s3.px.srcov.errorq25.pp}{$p=0.009$}
\@namedef{S@s3.px.srcov.errorq50.ci}{+0.001 to +0.012}
\@namedef{S@s3.px.srcov.errorq50.ci2}{+0.0009 to +0.0119}
\@namedef{S@s3.px.srcov.errorq50.d}{+0.005}
\@namedef{S@s3.px.srcov.errorq50.h13}{0.125}
\@namedef{S@s3.px.srcov.errorq50.p}{0.016}
\@namedef{S@s3.px.srcov.errorq50.pp}{$p=0.016$}
\@namedef{S@s3.px.srcov.errorq75.ci}{\ensuremath{-}0.003 to +0.007}
\@namedef{S@s3.px.srcov.errorq75.ci2}{\ensuremath{-}0.0031 to +0.0069}
\@namedef{S@s3.px.srcov.errorq75.d}{+0.002}
\@namedef{S@s3.px.srcov.errorq75.h13}{1.000}
\@namedef{S@s3.px.srcov.errorq75.p}{0.416}
\@namedef{S@s3.px.srcov.errorq75.pp}{$p=0.416$}
\@namedef{S@s3.px.srcov.errorq90.ci}{\ensuremath{-}0.004 to +0.002}
\@namedef{S@s3.px.srcov.errorq90.ci2}{\ensuremath{-}0.0040 to +0.0018}
\@namedef{S@s3.px.srcov.errorq90.d}{\ensuremath{-}0.001}
\@namedef{S@s3.px.srcov.errorq90.h13}{1.000}
\@namedef{S@s3.px.srcov.errorq90.p}{0.578}
\@namedef{S@s3.px.srcov.errorq90.pp}{$p=0.578$}
\@namedef{S@s3.px.srcov.geom.ci}{+0.010 to +0.028}
\@namedef{S@s3.px.srcov.geom.ci2}{+0.0095 to +0.0281}
\@namedef{S@s3.px.srcov.geom.d}{+0.018}
\@namedef{S@s3.px.srcov.geom.h13}{0.001}
\@namedef{S@s3.px.srcov.geom.p}{<0.001}
\@namedef{S@s3.px.srcov.geom.pp}{$p<0.001$}
\@namedef{S@s3.px.srcov.hi}{+0.028}
\@namedef{S@s3.px.srcov.lo}{\ensuremath{-}0.004}
\@namedef{S@s3.px.srcov.ndpos}{11}
\@namedef{S@s3.px.srcov.nholm}{3}
\@namedef{S@s3.px.srcov.nneg}{0}
\@namedef{S@s3.px.srcov.npos}{7}
\@namedef{S@s3.px.srcov.prim.dmax}{+0.018}
\@namedef{S@s3.px.srcov.prim.dmin}{+0.000}
\@namedef{S@s3.px.srcov.prim.hi}{+0.028}
\@namedef{S@s3.px.srcov.prim.lo}{\ensuremath{-}0.004}
\@namedef{S@s3.px.srcov.prim.npos}{2}
\@namedef{S@s3.px.srcov.prim.nsig}{2}
\@namedef{S@s3.sh.0.02.errorq75}{2.4}
\@namedef{S@s3.sh.0.05.errorq75}{1.2}
\@namedef{S@s3.sh.0.1.errorq75}{3.2}
\@namedef{S@s3.sh.0.25.errorq75}{2.0}
\@namedef{S@s3.sh.0.85.errorq75}{3.4}
\@namedef{S@s3.st.cells}{640}
\@namedef{S@s3.st.contactq25.ahead}{7}
\@namedef{S@s3.st.contactq25.aheadcov}{8}
\@namedef{S@s3.st.contactq25.aheadrandom}{7}
\@namedef{S@s3.st.contactq25.behind}{3}
\@namedef{S@s3.st.contactq25.random}{32.3}
\@namedef{S@s3.st.contactq25.random.cov}{0.934}
\@namedef{S@s3.st.contactq25.random.early}{0.84}
\@namedef{S@s3.st.contactq25.random.rate}{0.82}
\@namedef{S@s3.st.contactq25.random.rate35}{0.82}
\@namedef{S@s3.st.contactq25.random.u10}{0.83}
\@namedef{S@s3.st.contactq25.rule}{33.4}
\@namedef{S@s3.st.contactq25.rule.cov}{0.936}
\@namedef{S@s3.st.contactq25.rule.early}{0.97}
\@namedef{S@s3.st.contactq25.rule.rate}{0.82}
\@namedef{S@s3.st.contactq25.rule.rate35}{0.74}
\@namedef{S@s3.st.contactq25.rule.u10}{0.96}
\@namedef{S@s3.st.contactq25.shuffle}{33.0}
\@namedef{S@s3.st.contactq25.shuffle.cov}{0.935}
\@namedef{S@s3.st.contactq25.shuffle.early}{0.97}
\@namedef{S@s3.st.contactq25.shuffle.rate}{0.78}
\@namedef{S@s3.st.contactq25.shuffle.rate35}{0.74}
\@namedef{S@s3.st.contactq25.shuffle.u10}{0.96}
\@namedef{S@s3.st.contactq50.ahead}{9}
\@namedef{S@s3.st.contactq50.aheadcov}{10}
\@namedef{S@s3.st.contactq50.aheadrandom}{10}
\@namedef{S@s3.st.contactq50.behind}{1}
\@namedef{S@s3.st.contactq50.random}{29.1}
\@namedef{S@s3.st.contactq50.random.cov}{0.927}
\@namedef{S@s3.st.contactq50.random.early}{0.65}
\@namedef{S@s3.st.contactq50.random.rate}{0.62}
\@namedef{S@s3.st.contactq50.random.rate35}{0.62}
\@namedef{S@s3.st.contactq50.random.u10}{0.64}
\@namedef{S@s3.st.contactq50.rule}{33.0}
\@namedef{S@s3.st.contactq50.rule.cov}{0.935}
\@namedef{S@s3.st.contactq50.rule.early}{0.84}
\@namedef{S@s3.st.contactq50.rule.rate}{0.63}
\@namedef{S@s3.st.contactq50.rule.rate35}{0.52}
\@namedef{S@s3.st.contactq50.rule.u10}{0.82}
\@namedef{S@s3.st.contactq50.shuffle}{31.5}
\@namedef{S@s3.st.contactq50.shuffle.cov}{0.932}
\@namedef{S@s3.st.contactq50.shuffle.early}{0.83}
\@namedef{S@s3.st.contactq50.shuffle.rate}{0.57}
\@namedef{S@s3.st.contactq50.shuffle.rate35}{0.52}
\@namedef{S@s3.st.contactq50.shuffle.u10}{0.82}
\@namedef{S@s3.st.contactq75.ahead}{4}
\@namedef{S@s3.st.contactq75.aheadcov}{10}
\@namedef{S@s3.st.contactq75.aheadrandom}{3}
\@namedef{S@s3.st.contactq75.behind}{6}
\@namedef{S@s3.st.contactq75.random}{21.4}
\@namedef{S@s3.st.contactq75.random.cov}{0.909}
\@namedef{S@s3.st.contactq75.random.early}{0.37}
\@namedef{S@s3.st.contactq75.random.rate}{0.34}
\@namedef{S@s3.st.contactq75.random.rate35}{0.33}
\@namedef{S@s3.st.contactq75.random.u10}{0.37}
\@namedef{S@s3.st.contactq75.rule}{19.7}
\@namedef{S@s3.st.contactq75.rule.cov}{0.913}
\@namedef{S@s3.st.contactq75.rule.early}{0.44}
\@namedef{S@s3.st.contactq75.rule.rate}{0.34}
\@namedef{S@s3.st.contactq75.rule.rate35}{0.32}
\@namedef{S@s3.st.contactq75.rule.u10}{0.44}
\@namedef{S@s3.st.contactq75.shuffle}{21.3}
\@namedef{S@s3.st.contactq75.shuffle.cov}{0.907}
\@namedef{S@s3.st.contactq75.shuffle.early}{0.44}
\@namedef{S@s3.st.contactq75.shuffle.rate}{0.32}
\@namedef{S@s3.st.contactq75.shuffle.rate35}{0.32}
\@namedef{S@s3.st.contactq75.shuffle.u10}{0.44}
\@namedef{S@s3.st.contactq90.ahead}{4}
\@namedef{S@s3.st.contactq90.aheadcov}{7}
\@namedef{S@s3.st.contactq90.aheadrandom}{6}
\@namedef{S@s3.st.contactq90.behind}{6}
\@namedef{S@s3.st.contactq90.random}{15.6}
\@namedef{S@s3.st.contactq90.random.cov}{0.895}
\@namedef{S@s3.st.contactq90.random.early}{0.26}
\@namedef{S@s3.st.contactq90.random.rate}{0.23}
\@namedef{S@s3.st.contactq90.random.rate35}{0.22}
\@namedef{S@s3.st.contactq90.random.u10}{0.26}
\@namedef{S@s3.st.contactq90.rule}{16.6}
\@namedef{S@s3.st.contactq90.rule.cov}{0.900}
\@namedef{S@s3.st.contactq90.rule.early}{0.32}
\@namedef{S@s3.st.contactq90.rule.rate}{0.23}
\@namedef{S@s3.st.contactq90.rule.rate35}{0.22}
\@namedef{S@s3.st.contactq90.rule.u10}{0.32}
\@namedef{S@s3.st.contactq90.shuffle}{17.7}
\@namedef{S@s3.st.contactq90.shuffle.cov}{0.899}
\@namedef{S@s3.st.contactq90.shuffle.early}{0.32}
\@namedef{S@s3.st.contactq90.shuffle.rate}{0.23}
\@namedef{S@s3.st.contactq90.shuffle.rate35}{0.22}
\@namedef{S@s3.st.contactq90.shuffle.u10}{0.32}
\@namedef{S@s3.st.disagreementq25.ahead}{6}
\@namedef{S@s3.st.disagreementq25.aheadcov}{9}
\@namedef{S@s3.st.disagreementq25.aheadrandom}{10}
\@namedef{S@s3.st.disagreementq25.behind}{4}
\@namedef{S@s3.st.disagreementq25.random}{26.0}
\@namedef{S@s3.st.disagreementq25.random.cov}{0.921}
\@namedef{S@s3.st.disagreementq25.random.early}{0.51}
\@namedef{S@s3.st.disagreementq25.random.rate}{0.48}
\@namedef{S@s3.st.disagreementq25.random.rate35}{0.47}
\@namedef{S@s3.st.disagreementq25.random.u10}{0.50}
\@namedef{S@s3.st.disagreementq25.rule}{29.5}
\@namedef{S@s3.st.disagreementq25.rule.cov}{0.931}
\@namedef{S@s3.st.disagreementq25.rule.early}{0.62}
\@namedef{S@s3.st.disagreementq25.rule.rate}{0.48}
\@namedef{S@s3.st.disagreementq25.rule.rate35}{0.43}
\@namedef{S@s3.st.disagreementq25.rule.u10}{0.59}
\@namedef{S@s3.st.disagreementq25.shuffle}{28.7}
\@namedef{S@s3.st.disagreementq25.shuffle.cov}{0.927}
\@namedef{S@s3.st.disagreementq25.shuffle.early}{0.61}
\@namedef{S@s3.st.disagreementq25.shuffle.rate}{0.46}
\@namedef{S@s3.st.disagreementq25.shuffle.rate35}{0.43}
\@namedef{S@s3.st.disagreementq25.shuffle.u10}{0.59}
\@namedef{S@s3.st.disagreementq50.ahead}{6}
\@namedef{S@s3.st.disagreementq50.aheadcov}{10}
\@namedef{S@s3.st.disagreementq50.aheadrandom}{7}
\@namedef{S@s3.st.disagreementq50.behind}{4}
\@namedef{S@s3.st.disagreementq50.random}{21.3}
\@namedef{S@s3.st.disagreementq50.random.cov}{0.909}
\@namedef{S@s3.st.disagreementq50.random.early}{0.37}
\@namedef{S@s3.st.disagreementq50.random.rate}{0.33}
\@namedef{S@s3.st.disagreementq50.random.rate35}{0.33}
\@namedef{S@s3.st.disagreementq50.random.u10}{0.37}
\@namedef{S@s3.st.disagreementq50.rule}{23.6}
\@namedef{S@s3.st.disagreementq50.rule.cov}{0.921}
\@namedef{S@s3.st.disagreementq50.rule.early}{0.43}
\@namedef{S@s3.st.disagreementq50.rule.rate}{0.33}
\@namedef{S@s3.st.disagreementq50.rule.rate35}{0.31}
\@namedef{S@s3.st.disagreementq50.rule.u10}{0.41}
\@namedef{S@s3.st.disagreementq50.shuffle}{23.4}
\@namedef{S@s3.st.disagreementq50.shuffle.cov}{0.914}
\@namedef{S@s3.st.disagreementq50.shuffle.early}{0.42}
\@namedef{S@s3.st.disagreementq50.shuffle.rate}{0.32}
\@namedef{S@s3.st.disagreementq50.shuffle.rate35}{0.31}
\@namedef{S@s3.st.disagreementq50.shuffle.u10}{0.41}
\@namedef{S@s3.st.disagreementq75.ahead}{5}
\@namedef{S@s3.st.disagreementq75.aheadcov}{10}
\@namedef{S@s3.st.disagreementq75.aheadrandom}{9}
\@namedef{S@s3.st.disagreementq75.behind}{5}
\@namedef{S@s3.st.disagreementq75.random}{16.1}
\@namedef{S@s3.st.disagreementq75.random.cov}{0.895}
\@namedef{S@s3.st.disagreementq75.random.early}{0.26}
\@namedef{S@s3.st.disagreementq75.random.rate}{0.23}
\@namedef{S@s3.st.disagreementq75.random.rate35}{0.23}
\@namedef{S@s3.st.disagreementq75.random.u10}{0.26}
\@namedef{S@s3.st.disagreementq75.rule}{17.7}
\@namedef{S@s3.st.disagreementq75.rule.cov}{0.908}
\@namedef{S@s3.st.disagreementq75.rule.early}{0.29}
\@namedef{S@s3.st.disagreementq75.rule.rate}{0.23}
\@namedef{S@s3.st.disagreementq75.rule.rate35}{0.22}
\@namedef{S@s3.st.disagreementq75.rule.u10}{0.28}
\@namedef{S@s3.st.disagreementq75.shuffle}{17.6}
\@namedef{S@s3.st.disagreementq75.shuffle.cov}{0.899}
\@namedef{S@s3.st.disagreementq75.shuffle.early}{0.29}
\@namedef{S@s3.st.disagreementq75.shuffle.rate}{0.23}
\@namedef{S@s3.st.disagreementq75.shuffle.rate35}{0.22}
\@namedef{S@s3.st.disagreementq75.shuffle.u10}{0.28}
\@namedef{S@s3.st.disagreementq90.ahead}{3}
\@namedef{S@s3.st.disagreementq90.aheadcov}{9}
\@namedef{S@s3.st.disagreementq90.aheadrandom}{7}
\@namedef{S@s3.st.disagreementq90.behind}{7}
\@namedef{S@s3.st.disagreementq90.random}{14.1}
\@namedef{S@s3.st.disagreementq90.random.cov}{0.889}
\@namedef{S@s3.st.disagreementq90.random.early}{0.22}
\@namedef{S@s3.st.disagreementq90.random.rate}{0.19}
\@namedef{S@s3.st.disagreementq90.random.rate35}{0.19}
\@namedef{S@s3.st.disagreementq90.random.u10}{0.22}
\@namedef{S@s3.st.disagreementq90.rule}{14.8}
\@namedef{S@s3.st.disagreementq90.rule.cov}{0.895}
\@namedef{S@s3.st.disagreementq90.rule.early}{0.23}
\@namedef{S@s3.st.disagreementq90.rule.rate}{0.19}
\@namedef{S@s3.st.disagreementq90.rule.rate35}{0.19}
\@namedef{S@s3.st.disagreementq90.rule.u10}{0.22}
\@namedef{S@s3.st.disagreementq90.shuffle}{14.7}
\@namedef{S@s3.st.disagreementq90.shuffle.cov}{0.892}
\@namedef{S@s3.st.disagreementq90.shuffle.early}{0.23}
\@namedef{S@s3.st.disagreementq90.shuffle.rate}{0.19}
\@namedef{S@s3.st.disagreementq90.shuffle.rate35}{0.19}
\@namedef{S@s3.st.disagreementq90.shuffle.u10}{0.22}
\@namedef{S@s3.st.early.maxgap.random}{0.19}
\@namedef{S@s3.st.early.maxgap.shuffle}{0.01}
\@namedef{S@s3.st.errorq25.ahead}{6}
\@namedef{S@s3.st.errorq25.aheadcov}{6}
\@namedef{S@s3.st.errorq25.aheadrandom}{10}
\@namedef{S@s3.st.errorq25.behind}{4}
\@namedef{S@s3.st.errorq25.random}{27.8}
\@namedef{S@s3.st.errorq25.random.cov}{0.925}
\@namedef{S@s3.st.errorq25.random.early}{0.59}
\@namedef{S@s3.st.errorq25.random.rate}{0.56}
\@namedef{S@s3.st.errorq25.random.rate35}{0.56}
\@namedef{S@s3.st.errorq25.random.u10}{0.58}
\@namedef{S@s3.st.errorq25.rule}{31.5}
\@namedef{S@s3.st.errorq25.rule.cov}{0.933}
\@namedef{S@s3.st.errorq25.rule.early}{0.75}
\@namedef{S@s3.st.errorq25.rule.rate}{0.56}
\@namedef{S@s3.st.errorq25.rule.rate35}{0.48}
\@namedef{S@s3.st.errorq25.rule.u10}{0.72}
\@namedef{S@s3.st.errorq25.shuffle}{31.1}
\@namedef{S@s3.st.errorq25.shuffle.cov}{0.932}
\@namedef{S@s3.st.errorq25.shuffle.early}{0.75}
\@namedef{S@s3.st.errorq25.shuffle.rate}{0.53}
\@namedef{S@s3.st.errorq25.shuffle.rate35}{0.48}
\@namedef{S@s3.st.errorq25.shuffle.u10}{0.72}
\@namedef{S@s3.st.errorq50.ahead}{4}
\@namedef{S@s3.st.errorq50.aheadcov}{7}
\@namedef{S@s3.st.errorq50.aheadrandom}{10}
\@namedef{S@s3.st.errorq50.behind}{6}
\@namedef{S@s3.st.errorq50.random}{22.2}
\@namedef{S@s3.st.errorq50.random.cov}{0.912}
\@namedef{S@s3.st.errorq50.random.early}{0.40}
\@namedef{S@s3.st.errorq50.random.rate}{0.36}
\@namedef{S@s3.st.errorq50.random.rate35}{0.36}
\@namedef{S@s3.st.errorq50.random.u10}{0.39}
\@namedef{S@s3.st.errorq50.rule}{27.1}
\@namedef{S@s3.st.errorq50.rule.cov}{0.927}
\@namedef{S@s3.st.errorq50.rule.early}{0.52}
\@namedef{S@s3.st.errorq50.rule.rate}{0.36}
\@namedef{S@s3.st.errorq50.rule.rate35}{0.32}
\@namedef{S@s3.st.errorq50.rule.u10}{0.49}
\@namedef{S@s3.st.errorq50.shuffle}{27.1}
\@namedef{S@s3.st.errorq50.shuffle.cov}{0.924}
\@namedef{S@s3.st.errorq50.shuffle.early}{0.51}
\@namedef{S@s3.st.errorq50.shuffle.rate}{0.35}
\@namedef{S@s3.st.errorq50.shuffle.rate35}{0.32}
\@namedef{S@s3.st.errorq50.shuffle.u10}{0.49}
\@namedef{S@s3.st.errorq75.ahead}{2}
\@namedef{S@s3.st.errorq75.aheadcov}{6}
\@namedef{S@s3.st.errorq75.aheadrandom}{7}
\@namedef{S@s3.st.errorq75.behind}{8}
\@namedef{S@s3.st.errorq75.random}{16.0}
\@namedef{S@s3.st.errorq75.random.cov}{0.895}
\@namedef{S@s3.st.errorq75.random.early}{0.26}
\@namedef{S@s3.st.errorq75.random.rate}{0.23}
\@namedef{S@s3.st.errorq75.random.rate35}{0.23}
\@namedef{S@s3.st.errorq75.random.u10}{0.26}
\@namedef{S@s3.st.errorq75.rule}{18.0}
\@namedef{S@s3.st.errorq75.rule.cov}{0.907}
\@namedef{S@s3.st.errorq75.rule.early}{0.31}
\@namedef{S@s3.st.errorq75.rule.rate}{0.23}
\@namedef{S@s3.st.errorq75.rule.rate35}{0.22}
\@namedef{S@s3.st.errorq75.rule.u10}{0.30}
\@namedef{S@s3.st.errorq75.shuffle}{19.0}
\@namedef{S@s3.st.errorq75.shuffle.cov}{0.904}
\@namedef{S@s3.st.errorq75.shuffle.early}{0.31}
\@namedef{S@s3.st.errorq75.shuffle.rate}{0.23}
\@namedef{S@s3.st.errorq75.shuffle.rate35}{0.22}
\@namedef{S@s3.st.errorq75.shuffle.u10}{0.30}
\@namedef{S@s3.st.errorq90.ahead}{5}
\@namedef{S@s3.st.errorq90.aheadcov}{5}
\@namedef{S@s3.st.errorq90.aheadrandom}{5}
\@namedef{S@s3.st.errorq90.behind}{5}
\@namedef{S@s3.st.errorq90.random}{13.9}
\@namedef{S@s3.st.errorq90.random.cov}{0.889}
\@namedef{S@s3.st.errorq90.random.early}{0.22}
\@namedef{S@s3.st.errorq90.random.rate}{0.19}
\@namedef{S@s3.st.errorq90.random.rate35}{0.19}
\@namedef{S@s3.st.errorq90.random.u10}{0.21}
\@namedef{S@s3.st.errorq90.rule}{13.7}
\@namedef{S@s3.st.errorq90.rule.cov}{0.891}
\@namedef{S@s3.st.errorq90.rule.early}{0.23}
\@namedef{S@s3.st.errorq90.rule.rate}{0.19}
\@namedef{S@s3.st.errorq90.rule.rate35}{0.19}
\@namedef{S@s3.st.errorq90.rule.u10}{0.22}
\@namedef{S@s3.st.errorq90.shuffle}{14.2}
\@namedef{S@s3.st.errorq90.shuffle.cov}{0.891}
\@namedef{S@s3.st.errorq90.shuffle.early}{0.23}
\@namedef{S@s3.st.errorq90.shuffle.rate}{0.19}
\@namedef{S@s3.st.errorq90.shuffle.rate35}{0.19}
\@namedef{S@s3.st.errorq90.shuffle.u10}{0.22}
\@namedef{S@s3.st.final.F.ci}{+0.037 to +0.077}
\@namedef{S@s3.st.final.F.ci2}{+0.0366 to +0.0769}
\@namedef{S@s3.st.final.F.d}{+0.055}
\@namedef{S@s3.st.final.F.p}{<0.001}
\@namedef{S@s3.st.final.F.pp}{$p<0.001$}
\@namedef{S@s3.st.final.fixed1}{0.932}
\@namedef{S@s3.st.final.fixed4}{0.878}
\@namedef{S@s3.st.final95.F.ci}{+13.0 to +24.0}
\@namedef{S@s3.st.final95.F.ci2}{+13.00 to +24.00}
\@namedef{S@s3.st.final95.F.d}{+18.4}
\@namedef{S@s3.st.final95.F.p}{<0.001}
\@namedef{S@s3.st.final95.F.pp}{$p<0.001$}
\@namedef{S@s3.st.final95.fixed1}{32.2}
\@namedef{S@s3.st.final95.fixed4}{13.8}
\@namedef{S@s3.st.geom.ahead}{0}
\@namedef{S@s3.st.geom.aheadcov}{3}
\@namedef{S@s3.st.geom.aheadrandom}{10}
\@namedef{S@s3.st.geom.behind}{10}
\@namedef{S@s3.st.geom.random}{17.4}
\@namedef{S@s3.st.geom.random.cov}{0.898}
\@namedef{S@s3.st.geom.random.early}{0.28}
\@namedef{S@s3.st.geom.random.rate}{0.25}
\@namedef{S@s3.st.geom.random.rate35}{0.25}
\@namedef{S@s3.st.geom.random.u10}{0.28}
\@namedef{S@s3.st.geom.rule}{20.1}
\@namedef{S@s3.st.geom.rule.cov}{0.913}
\@namedef{S@s3.st.geom.rule.early}{0.37}
\@namedef{S@s3.st.geom.rule.rate}{0.26}
\@namedef{S@s3.st.geom.rule.rate35}{0.24}
\@namedef{S@s3.st.geom.rule.u10}{0.37}
\@namedef{S@s3.st.geom.shuffle}{22.8}
\@namedef{S@s3.st.geom.shuffle.cov}{0.915}
\@namedef{S@s3.st.geom.shuffle.early}{0.37}
\@namedef{S@s3.st.geom.shuffle.rate}{0.26}
\@namedef{S@s3.st.geom.shuffle.rate35}{0.24}
\@namedef{S@s3.st.geom.shuffle.u10}{0.37}
\@namedef{S@s3.st.h8.min}{0.062}
\@namedef{S@s3.st.h8.nsig}{0}
\@namedef{S@s3.st.profmax}{1e-12}
\@namedef{S@s3.st.rate35.random.max}{+0.00}
\@namedef{S@s3.st.rate35.random.min}{\ensuremath{-}0.10}
\@namedef{S@s3.st.rr.contactq25.ci}{\ensuremath{-}1.0 to +3.1}
\@namedef{S@s3.st.rr.contactq25.ci2}{\ensuremath{-}1.02 to +3.11}
\@namedef{S@s3.st.rr.contactq25.d}{+1.1}
\@namedef{S@s3.st.rr.contactq25.p}{0.292}
\@namedef{S@s3.st.rr.contactq25.pp}{$p=0.292$}
\@namedef{S@s3.st.rr.contactq50.ci}{+1.5 to +6.5}
\@namedef{S@s3.st.rr.contactq50.ci2}{+1.48 to +6.51}
\@namedef{S@s3.st.rr.contactq50.d}{+3.9}
\@namedef{S@s3.st.rr.contactq50.p}{0.002}
\@namedef{S@s3.st.rr.contactq50.pp}{$p=0.002$}
\@namedef{S@s3.st.rr.contactq75.ci}{\ensuremath{-}5.7 to +2.3}
\@namedef{S@s3.st.rr.contactq75.ci2}{\ensuremath{-}5.74 to +2.31}
\@namedef{S@s3.st.rr.contactq75.d}{\ensuremath{-}1.6}
\@namedef{S@s3.st.rr.contactq75.p}{0.416}
\@namedef{S@s3.st.rr.contactq75.pp}{$p=0.416$}
\@namedef{S@s3.st.rr.contactq90.ci}{\ensuremath{-}2.0 to +4.2}
\@namedef{S@s3.st.rr.contactq90.ci2}{\ensuremath{-}1.98 to +4.20}
\@namedef{S@s3.st.rr.contactq90.d}{+1.0}
\@namedef{S@s3.st.rr.contactq90.p}{0.537}
\@namedef{S@s3.st.rr.contactq90.pp}{$p=0.537$}
\@namedef{S@s3.st.rr.disagreementq25.ci}{+0.5 to +6.6}
\@namedef{S@s3.st.rr.disagreementq25.ci2}{+0.55 to +6.61}
\@namedef{S@s3.st.rr.disagreementq25.d}{+3.5}
\@namedef{S@s3.st.rr.disagreementq25.p}{0.023}
\@namedef{S@s3.st.rr.disagreementq25.pp}{$p=0.023$}
\@namedef{S@s3.st.rr.disagreementq50.ci}{\ensuremath{-}1.2 to +6.1}
\@namedef{S@s3.st.rr.disagreementq50.ci2}{\ensuremath{-}1.17 to +6.11}
\@namedef{S@s3.st.rr.disagreementq50.d}{+2.3}
\@namedef{S@s3.st.rr.disagreementq50.p}{0.202}
\@namedef{S@s3.st.rr.disagreementq50.pp}{$p=0.202$}
\@namedef{S@s3.st.rr.disagreementq75.ci}{\ensuremath{-}1.3 to +4.5}
\@namedef{S@s3.st.rr.disagreementq75.ci2}{\ensuremath{-}1.26 to +4.54}
\@namedef{S@s3.st.rr.disagreementq75.d}{+1.6}
\@namedef{S@s3.st.rr.disagreementq75.p}{0.282}
\@namedef{S@s3.st.rr.disagreementq75.pp}{$p=0.282$}
\@namedef{S@s3.st.rr.disagreementq90.ci}{\ensuremath{-}1.3 to +2.8}
\@namedef{S@s3.st.rr.disagreementq90.ci2}{\ensuremath{-}1.26 to +2.79}
\@namedef{S@s3.st.rr.disagreementq90.d}{+0.7}
\@namedef{S@s3.st.rr.disagreementq90.p}{0.523}
\@namedef{S@s3.st.rr.disagreementq90.pp}{$p=0.523$}
\@namedef{S@s3.st.rr.errorq25.ci}{+0.9 to +6.4}
\@namedef{S@s3.st.rr.errorq25.ci2}{+0.94 to +6.44}
\@namedef{S@s3.st.rr.errorq25.d}{+3.7}
\@namedef{S@s3.st.rr.errorq25.p}{0.008}
\@namedef{S@s3.st.rr.errorq25.pp}{$p=0.008$}
\@namedef{S@s3.st.rr.errorq50.ci}{+1.8 to +8.1}
\@namedef{S@s3.st.rr.errorq50.ci2}{+1.84 to +8.14}
\@namedef{S@s3.st.rr.errorq50.d}{+4.9}
\@namedef{S@s3.st.rr.errorq50.p}{0.002}
\@namedef{S@s3.st.rr.errorq50.pp}{$p=0.002$}
\@namedef{S@s3.st.rr.errorq75.ci}{\ensuremath{-}1.1 to +5.5}
\@namedef{S@s3.st.rr.errorq75.ci2}{\ensuremath{-}1.14 to +5.52}
\@namedef{S@s3.st.rr.errorq75.d}{+2.0}
\@namedef{S@s3.st.rr.errorq75.p}{0.223}
\@namedef{S@s3.st.rr.errorq75.pp}{$p=0.223$}
\@namedef{S@s3.st.rr.errorq90.ci}{\ensuremath{-}1.9 to +1.6}
\@namedef{S@s3.st.rr.errorq90.ci2}{\ensuremath{-}1.93 to +1.58}
\@namedef{S@s3.st.rr.errorq90.d}{\ensuremath{-}0.2}
\@namedef{S@s3.st.rr.errorq90.p}{0.860}
\@namedef{S@s3.st.rr.errorq90.pp}{$p=0.860$}
\@namedef{S@s3.st.rr.geom.ci}{\ensuremath{-}1.3 to +6.8}
\@namedef{S@s3.st.rr.geom.ci2}{\ensuremath{-}1.33 to +6.83}
\@namedef{S@s3.st.rr.geom.d}{+2.7}
\@namedef{S@s3.st.rr.geom.p}{0.187}
\@namedef{S@s3.st.rr.geom.pp}{$p=0.187$}
\@namedef{S@s3.st.rrcov.contactq25.ci}{\ensuremath{-}0.0004 to +0.005}
\@namedef{S@s3.st.rrcov.contactq25.ci2}{\ensuremath{-}0.0004 to +0.0048}
\@namedef{S@s3.st.rrcov.contactq25.d}{+0.002}
\@namedef{S@s3.st.rrcov.contactq25.p}{0.104}
\@namedef{S@s3.st.rrcov.contactq25.pp}{$p=0.104$}
\@namedef{S@s3.st.rrcov.contactq50.ci}{+0.004 to +0.011}
\@namedef{S@s3.st.rrcov.contactq50.ci2}{+0.0036 to +0.0114}
\@namedef{S@s3.st.rrcov.contactq50.d}{+0.007}
\@namedef{S@s3.st.rrcov.contactq50.p}{<0.001}
\@namedef{S@s3.st.rrcov.contactq50.pp}{$p<0.001$}
\@namedef{S@s3.st.rrcov.contactq75.ci}{\ensuremath{-}0.004 to +0.013}
\@namedef{S@s3.st.rrcov.contactq75.ci2}{\ensuremath{-}0.0042 to +0.0128}
\@namedef{S@s3.st.rrcov.contactq75.d}{+0.004}
\@namedef{S@s3.st.rrcov.contactq75.p}{0.371}
\@namedef{S@s3.st.rrcov.contactq75.pp}{$p=0.371$}
\@namedef{S@s3.st.rrcov.contactq90.ci}{\ensuremath{-}0.0002 to +0.013}
\@namedef{S@s3.st.rrcov.contactq90.ci2}{\ensuremath{-}0.0002 to +0.0127}
\@namedef{S@s3.st.rrcov.contactq90.d}{+0.006}
\@namedef{S@s3.st.rrcov.contactq90.p}{0.060}
\@namedef{S@s3.st.rrcov.contactq90.pp}{$p=0.060$}
\@namedef{S@s3.st.rrcov.disagreementq25.ci}{+0.006 to +0.015}
\@namedef{S@s3.st.rrcov.disagreementq25.ci2}{+0.0058 to +0.0152}
\@namedef{S@s3.st.rrcov.disagreementq25.d}{+0.010}
\@namedef{S@s3.st.rrcov.disagreementq25.p}{<0.001}
\@namedef{S@s3.st.rrcov.disagreementq25.pp}{$p<0.001$}
\@namedef{S@s3.st.rrcov.disagreementq50.ci}{+0.006 to +0.020}
\@namedef{S@s3.st.rrcov.disagreementq50.ci2}{+0.0056 to +0.0196}
\@namedef{S@s3.st.rrcov.disagreementq50.d}{+0.012}
\@namedef{S@s3.st.rrcov.disagreementq50.p}{0.001}
\@namedef{S@s3.st.rrcov.disagreementq50.pp}{$p=0.001$}
\@namedef{S@s3.st.rrcov.disagreementq75.ci}{+0.005 to +0.021}
\@namedef{S@s3.st.rrcov.disagreementq75.ci2}{+0.0054 to +0.0213}
\@namedef{S@s3.st.rrcov.disagreementq75.d}{+0.013}
\@namedef{S@s3.st.rrcov.disagreementq75.p}{<0.001}
\@namedef{S@s3.st.rrcov.disagreementq75.pp}{$p<0.001$}
\@namedef{S@s3.st.rrcov.disagreementq90.ci}{\ensuremath{-}0.001 to +0.012}
\@namedef{S@s3.st.rrcov.disagreementq90.ci2}{\ensuremath{-}0.0015 to +0.0122}
\@namedef{S@s3.st.rrcov.disagreementq90.d}{+0.005}
\@namedef{S@s3.st.rrcov.disagreementq90.p}{0.127}
\@namedef{S@s3.st.rrcov.disagreementq90.pp}{$p=0.127$}
\@namedef{S@s3.st.rrcov.errorq25.ci}{+0.004 to +0.013}
\@namedef{S@s3.st.rrcov.errorq25.ci2}{+0.0038 to +0.0133}
\@namedef{S@s3.st.rrcov.errorq25.d}{+0.008}
\@namedef{S@s3.st.rrcov.errorq25.p}{<0.001}
\@namedef{S@s3.st.rrcov.errorq25.pp}{$p<0.001$}
\@namedef{S@s3.st.rrcov.errorq50.ci}{+0.010 to +0.022}
\@namedef{S@s3.st.rrcov.errorq50.ci2}{+0.0097 to +0.0218}
\@namedef{S@s3.st.rrcov.errorq50.d}{+0.015}
\@namedef{S@s3.st.rrcov.errorq50.p}{<0.001}
\@namedef{S@s3.st.rrcov.errorq50.pp}{$p<0.001$}
\@namedef{S@s3.st.rrcov.errorq75.ci}{+0.005 to +0.019}
\@namedef{S@s3.st.rrcov.errorq75.ci2}{+0.0052 to +0.0194}
\@namedef{S@s3.st.rrcov.errorq75.d}{+0.012}
\@namedef{S@s3.st.rrcov.errorq75.p}{<0.001}
\@namedef{S@s3.st.rrcov.errorq75.pp}{$p<0.001$}
\@namedef{S@s3.st.rrcov.errorq90.ci}{\ensuremath{-}0.003 to +0.009}
\@namedef{S@s3.st.rrcov.errorq90.ci2}{\ensuremath{-}0.0026 to +0.0090}
\@namedef{S@s3.st.rrcov.errorq90.d}{+0.003}
\@namedef{S@s3.st.rrcov.errorq90.p}{0.338}
\@namedef{S@s3.st.rrcov.errorq90.pp}{$p=0.338$}
\@namedef{S@s3.st.rrcov.geom.ci}{+0.008 to +0.023}
\@namedef{S@s3.st.rrcov.geom.ci2}{+0.0078 to +0.0227}
\@namedef{S@s3.st.rrcov.geom.d}{+0.015}
\@namedef{S@s3.st.rrcov.geom.p}{<0.001}
\@namedef{S@s3.st.rrcov.geom.pp}{$p<0.001$}
\@namedef{S@s3.st.rs.contactq25.ci}{\ensuremath{-}0.9 to +1.8}
\@namedef{S@s3.st.rs.contactq25.ci2}{\ensuremath{-}0.87 to +1.79}
\@namedef{S@s3.st.rs.contactq25.d}{+0.4}
\@namedef{S@s3.st.rs.contactq25.h13}{1.000}
\@namedef{S@s3.st.rs.contactq25.p}{0.498}
\@namedef{S@s3.st.rs.contactq25.pp}{$p=0.498$}
\@namedef{S@s3.st.rs.contactq50.ci}{\ensuremath{-}0.7 to +3.8}
\@namedef{S@s3.st.rs.contactq50.ci2}{\ensuremath{-}0.66 to +3.80}
\@namedef{S@s3.st.rs.contactq50.d}{+1.5}
\@namedef{S@s3.st.rs.contactq50.h13}{1.000}
\@namedef{S@s3.st.rs.contactq50.p}{0.168}
\@namedef{S@s3.st.rs.contactq50.pp}{$p=0.168$}
\@namedef{S@s3.st.rs.contactq75.ci}{\ensuremath{-}5.1 to +2.0}
\@namedef{S@s3.st.rs.contactq75.ci2}{\ensuremath{-}5.11 to +1.98}
\@namedef{S@s3.st.rs.contactq75.d}{\ensuremath{-}1.6}
\@namedef{S@s3.st.rs.contactq75.h13}{1.000}
\@namedef{S@s3.st.rs.contactq75.h8}{1.000}
\@namedef{S@s3.st.rs.contactq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.st.rs.contactq75.p}{0.374}
\@namedef{S@s3.st.rs.contactq75.pp}{$p=0.374$}
\@namedef{S@s3.st.rs.contactq90.ci}{\ensuremath{-}4.3 to +2.0}
\@namedef{S@s3.st.rs.contactq90.ci2}{\ensuremath{-}4.28 to +2.01}
\@namedef{S@s3.st.rs.contactq90.d}{\ensuremath{-}1.1}
\@namedef{S@s3.st.rs.contactq90.h13}{1.000}
\@namedef{S@s3.st.rs.contactq90.p}{0.475}
\@namedef{S@s3.st.rs.contactq90.pp}{$p=0.475$}
\@namedef{S@s3.st.rs.disagreementq25.ci}{\ensuremath{-}2.0 to +3.5}
\@namedef{S@s3.st.rs.disagreementq25.ci2}{\ensuremath{-}2.02 to +3.52}
\@namedef{S@s3.st.rs.disagreementq25.d}{+0.8}
\@namedef{S@s3.st.rs.disagreementq25.h13}{1.000}
\@namedef{S@s3.st.rs.disagreementq25.p}{0.533}
\@namedef{S@s3.st.rs.disagreementq25.pp}{$p=0.533$}
\@namedef{S@s3.st.rs.disagreementq50.ci}{\ensuremath{-}3.2 to +3.7}
\@namedef{S@s3.st.rs.disagreementq50.ci2}{\ensuremath{-}3.17 to +3.67}
\@namedef{S@s3.st.rs.disagreementq50.d}{+0.2}
\@namedef{S@s3.st.rs.disagreementq50.h13}{1.000}
\@namedef{S@s3.st.rs.disagreementq50.p}{0.928}
\@namedef{S@s3.st.rs.disagreementq50.pp}{$p=0.928$}
\@namedef{S@s3.st.rs.disagreementq75.ci}{\ensuremath{-}2.7 to +2.9}
\@namedef{S@s3.st.rs.disagreementq75.ci2}{\ensuremath{-}2.72 to +2.87}
\@namedef{S@s3.st.rs.disagreementq75.d}{+0.1}
\@namedef{S@s3.st.rs.disagreementq75.h13}{1.000}
\@namedef{S@s3.st.rs.disagreementq75.h8}{1.000}
\@namedef{S@s3.st.rs.disagreementq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.st.rs.disagreementq75.p}{0.935}
\@namedef{S@s3.st.rs.disagreementq75.pp}{$p=0.935$}
\@namedef{S@s3.st.rs.disagreementq90.ci}{\ensuremath{-}2.0 to +2.4}
\@namedef{S@s3.st.rs.disagreementq90.ci2}{\ensuremath{-}1.95 to +2.42}
\@namedef{S@s3.st.rs.disagreementq90.d}{+0.1}
\@namedef{S@s3.st.rs.disagreementq90.h13}{1.000}
\@namedef{S@s3.st.rs.disagreementq90.p}{0.968}
\@namedef{S@s3.st.rs.disagreementq90.pp}{$p=0.968$}
\@namedef{S@s3.st.rs.dmax}{+1.5}
\@namedef{S@s3.st.rs.dmin}{\ensuremath{-}2.6}
\@namedef{S@s3.st.rs.errorq25.ci}{\ensuremath{-}2.0 to +2.8}
\@namedef{S@s3.st.rs.errorq25.ci2}{\ensuremath{-}1.97 to +2.85}
\@namedef{S@s3.st.rs.errorq25.d}{+0.4}
\@namedef{S@s3.st.rs.errorq25.h13}{1.000}
\@namedef{S@s3.st.rs.errorq25.p}{0.753}
\@namedef{S@s3.st.rs.errorq25.pp}{$p=0.753$}
\@namedef{S@s3.st.rs.errorq50.ci}{\ensuremath{-}2.8 to +2.7}
\@namedef{S@s3.st.rs.errorq50.ci2}{\ensuremath{-}2.81 to +2.68}
\@namedef{S@s3.st.rs.errorq50.d}{+0.0}
\@namedef{S@s3.st.rs.errorq50.h13}{1.000}
\@namedef{S@s3.st.rs.errorq50.p}{0.965}
\@namedef{S@s3.st.rs.errorq50.pp}{$p=0.965$}
\@namedef{S@s3.st.rs.errorq75.ci}{\ensuremath{-}4.1 to +2.2}
\@namedef{S@s3.st.rs.errorq75.ci2}{\ensuremath{-}4.10 to +2.21}
\@namedef{S@s3.st.rs.errorq75.d}{\ensuremath{-}1.0}
\@namedef{S@s3.st.rs.errorq75.h13}{1.000}
\@namedef{S@s3.st.rs.errorq75.h8}{1.000}
\@namedef{S@s3.st.rs.errorq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.st.rs.errorq75.p}{0.528}
\@namedef{S@s3.st.rs.errorq75.pp}{$p=0.528$}
\@namedef{S@s3.st.rs.errorq90.ci}{\ensuremath{-}2.2 to +1.3}
\@namedef{S@s3.st.rs.errorq90.ci2}{\ensuremath{-}2.21 to +1.34}
\@namedef{S@s3.st.rs.errorq90.d}{\ensuremath{-}0.5}
\@namedef{S@s3.st.rs.errorq90.h13}{1.000}
\@namedef{S@s3.st.rs.errorq90.p}{0.600}
\@namedef{S@s3.st.rs.errorq90.pp}{$p=0.600$}
\@namedef{S@s3.st.rs.geom.ci}{\ensuremath{-}5.5 to \ensuremath{-}0.04}
\@namedef{S@s3.st.rs.geom.ci2}{\ensuremath{-}5.47 to \ensuremath{-}0.04}
\@namedef{S@s3.st.rs.geom.d}{\ensuremath{-}2.6}
\@namedef{S@s3.st.rs.geom.h13}{0.627}
\@namedef{S@s3.st.rs.geom.h8}{0.337}
\@namedef{S@s3.st.rs.geom.hh8}{$p_{\mathrm{Holm}}=0.337$}
\@namedef{S@s3.st.rs.geom.p}{0.048}
\@namedef{S@s3.st.rs.geom.pp}{$p=0.048$}
\@namedef{S@s3.st.rs.hi}{+3.8}
\@namedef{S@s3.st.rs.lo}{\ensuremath{-}5.5}
\@namedef{S@s3.st.rs.ndpos}{8}
\@namedef{S@s3.st.rs.nholm}{0}
\@namedef{S@s3.st.rs.nneg}{1}
\@namedef{S@s3.st.rs.npos}{0}
\@namedef{S@s3.st.rs.prim.dmax}{+0.1}
\@namedef{S@s3.st.rs.prim.dmin}{\ensuremath{-}2.6}
\@namedef{S@s3.st.rs.prim.hi}{+2.9}
\@namedef{S@s3.st.rs.prim.lo}{\ensuremath{-}5.5}
\@namedef{S@s3.st.rs.prim.npos}{0}
\@namedef{S@s3.st.rs.prim.nsig}{1}
\@namedef{S@s3.st.rscov.contactq25.ci}{\ensuremath{-}0.001 to +0.002}
\@namedef{S@s3.st.rscov.contactq25.ci2}{\ensuremath{-}0.0007 to +0.0018}
\@namedef{S@s3.st.rscov.contactq25.d}{+0.001}
\@namedef{S@s3.st.rscov.contactq25.h13}{1.000}
\@namedef{S@s3.st.rscov.contactq25.p}{0.302}
\@namedef{S@s3.st.rscov.contactq25.pp}{$p=0.302$}
\@namedef{S@s3.st.rscov.contactq50.ci}{\ensuremath{-}0.0000 to +0.004}
\@namedef{S@s3.st.rscov.contactq50.ci2}{\ensuremath{-}0.00003 to +0.0044}
\@namedef{S@s3.st.rscov.contactq50.d}{+0.002}
\@namedef{S@s3.st.rscov.contactq50.h13}{0.534}
\@namedef{S@s3.st.rscov.contactq50.p}{0.053}
\@namedef{S@s3.st.rscov.contactq50.pp}{$p=0.053$}
\@namedef{S@s3.st.rscov.contactq75.ci}{\ensuremath{-}0.002 to +0.014}
\@namedef{S@s3.st.rscov.contactq75.ci2}{\ensuremath{-}0.0017 to +0.0144}
\@namedef{S@s3.st.rscov.contactq75.d}{+0.006}
\@namedef{S@s3.st.rscov.contactq75.h13}{1.000}
\@namedef{S@s3.st.rscov.contactq75.h8}{0.842}
\@namedef{S@s3.st.rscov.contactq75.hh8}{$p_{\mathrm{Holm}}=0.842$}
\@namedef{S@s3.st.rscov.contactq75.p}{0.140}
\@namedef{S@s3.st.rscov.contactq75.pp}{$p=0.140$}
\@namedef{S@s3.st.rscov.contactq90.ci}{\ensuremath{-}0.004 to +0.008}
\@namedef{S@s3.st.rscov.contactq90.ci2}{\ensuremath{-}0.0043 to +0.0082}
\@namedef{S@s3.st.rscov.contactq90.d}{+0.002}
\@namedef{S@s3.st.rscov.contactq90.h13}{1.000}
\@namedef{S@s3.st.rscov.contactq90.p}{0.600}
\@namedef{S@s3.st.rscov.contactq90.pp}{$p=0.600$}
\@namedef{S@s3.st.rscov.disagreementq25.ci}{+0.0004 to +0.008}
\@namedef{S@s3.st.rscov.disagreementq25.ci2}{+0.0004 to +0.0079}
\@namedef{S@s3.st.rscov.disagreementq25.d}{+0.004}
\@namedef{S@s3.st.rscov.disagreementq25.h13}{0.377}
\@namedef{S@s3.st.rscov.disagreementq25.p}{0.031}
\@namedef{S@s3.st.rscov.disagreementq25.pp}{$p=0.031$}
\@namedef{S@s3.st.rscov.disagreementq50.ci}{+0.001 to +0.013}
\@namedef{S@s3.st.rscov.disagreementq50.ci2}{+0.0005 to +0.0135}
\@namedef{S@s3.st.rscov.disagreementq50.d}{+0.007}
\@namedef{S@s3.st.rscov.disagreementq50.h13}{0.418}
\@namedef{S@s3.st.rscov.disagreementq50.p}{0.038}
\@namedef{S@s3.st.rscov.disagreementq50.pp}{$p=0.038$}
\@namedef{S@s3.st.rscov.disagreementq75.ci}{+0.002 to +0.016}
\@namedef{S@s3.st.rscov.disagreementq75.ci2}{+0.0021 to +0.0162}
\@namedef{S@s3.st.rscov.disagreementq75.d}{+0.009}
\@namedef{S@s3.st.rscov.disagreementq75.h13}{0.101}
\@namedef{S@s3.st.rscov.disagreementq75.h8}{0.062}
\@namedef{S@s3.st.rscov.disagreementq75.hh8}{$p_{\mathrm{Holm}}=0.062$}
\@namedef{S@s3.st.rscov.disagreementq75.p}{0.008}
\@namedef{S@s3.st.rscov.disagreementq75.pp}{$p=0.008$}
\@namedef{S@s3.st.rscov.disagreementq90.ci}{\ensuremath{-}0.003 to +0.009}
\@namedef{S@s3.st.rscov.disagreementq90.ci2}{\ensuremath{-}0.0035 to +0.0094}
\@namedef{S@s3.st.rscov.disagreementq90.d}{+0.003}
\@namedef{S@s3.st.rscov.disagreementq90.h13}{1.000}
\@namedef{S@s3.st.rscov.disagreementq90.p}{0.337}
\@namedef{S@s3.st.rscov.disagreementq90.pp}{$p=0.337$}
\@namedef{S@s3.st.rscov.dmax}{+0.009}
\@namedef{S@s3.st.rscov.dmin}{\ensuremath{-}0.002}
\@namedef{S@s3.st.rscov.errorq25.ci}{\ensuremath{-}0.002 to +0.004}
\@namedef{S@s3.st.rscov.errorq25.ci2}{\ensuremath{-}0.0020 to +0.0043}
\@namedef{S@s3.st.rscov.errorq25.d}{+0.001}
\@namedef{S@s3.st.rscov.errorq25.h13}{1.000}
\@namedef{S@s3.st.rscov.errorq25.p}{0.481}
\@namedef{S@s3.st.rscov.errorq25.pp}{$p=0.481$}
\@namedef{S@s3.st.rscov.errorq50.ci}{\ensuremath{-}0.001 to +0.008}
\@namedef{S@s3.st.rscov.errorq50.ci2}{\ensuremath{-}0.0009 to +0.0077}
\@namedef{S@s3.st.rscov.errorq50.d}{+0.003}
\@namedef{S@s3.st.rscov.errorq50.h13}{1.000}
\@namedef{S@s3.st.rscov.errorq50.p}{0.119}
\@namedef{S@s3.st.rscov.errorq50.pp}{$p=0.119$}
\@namedef{S@s3.st.rscov.errorq75.ci}{\ensuremath{-}0.003 to +0.010}
\@namedef{S@s3.st.rscov.errorq75.ci2}{\ensuremath{-}0.0034 to +0.0096}
\@namedef{S@s3.st.rscov.errorq75.d}{+0.003}
\@namedef{S@s3.st.rscov.errorq75.h13}{1.000}
\@namedef{S@s3.st.rscov.errorq75.h8}{1.000}
\@namedef{S@s3.st.rscov.errorq75.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.st.rscov.errorq75.p}{0.358}
\@namedef{S@s3.st.rscov.errorq75.pp}{$p=0.358$}
\@namedef{S@s3.st.rscov.errorq90.ci}{\ensuremath{-}0.005 to +0.007}
\@namedef{S@s3.st.rscov.errorq90.ci2}{\ensuremath{-}0.0050 to +0.0068}
\@namedef{S@s3.st.rscov.errorq90.d}{+0.001}
\@namedef{S@s3.st.rscov.errorq90.h13}{1.000}
\@namedef{S@s3.st.rscov.errorq90.p}{0.910}
\@namedef{S@s3.st.rscov.errorq90.pp}{$p=0.910$}
\@namedef{S@s3.st.rscov.geom.ci}{\ensuremath{-}0.005 to +0.002}
\@namedef{S@s3.st.rscov.geom.ci2}{\ensuremath{-}0.0053 to +0.0017}
\@namedef{S@s3.st.rscov.geom.d}{\ensuremath{-}0.002}
\@namedef{S@s3.st.rscov.geom.h13}{1.000}
\@namedef{S@s3.st.rscov.geom.h8}{1.000}
\@namedef{S@s3.st.rscov.geom.hh8}{$p_{\mathrm{Holm}}=1.000$}
\@namedef{S@s3.st.rscov.geom.p}{0.290}
\@namedef{S@s3.st.rscov.geom.pp}{$p=0.290$}
\@namedef{S@s3.st.rscov.hi}{+0.016}
\@namedef{S@s3.st.rscov.lo}{\ensuremath{-}0.005}
\@namedef{S@s3.st.rscov.ndpos}{12}
\@namedef{S@s3.st.rscov.nholm}{0}
\@namedef{S@s3.st.rscov.nneg}{0}
\@namedef{S@s3.st.rscov.npos}{3}
\@namedef{S@s3.st.rscov.prim.dmax}{+0.009}
\@namedef{S@s3.st.rscov.prim.dmin}{\ensuremath{-}0.002}
\@namedef{S@s3.st.rscov.prim.hi}{+0.016}
\@namedef{S@s3.st.rscov.prim.lo}{\ensuremath{-}0.005}
\@namedef{S@s3.st.rscov.prim.npos}{1}
\@namedef{S@s3.st.rscov.prim.nsig}{1}
\@namedef{S@s3.st.seeds}{10}
\@namedef{S@s3.st.sr.contactq25.ci}{\ensuremath{-}0.9 to +2.3}
\@namedef{S@s3.st.sr.contactq25.ci2}{\ensuremath{-}0.95 to +2.25}
\@namedef{S@s3.st.sr.contactq25.d}{+0.7}
\@namedef{S@s3.st.sr.contactq25.h13}{1.000}
\@namedef{S@s3.st.sr.contactq25.p}{0.405}
\@namedef{S@s3.st.sr.contactq25.pp}{$p=0.405$}
\@namedef{S@s3.st.sr.contactq50.ci}{+0.6 to +4.3}
\@namedef{S@s3.st.sr.contactq50.ci2}{+0.61 to +4.30}
\@namedef{S@s3.st.sr.contactq50.d}{+2.4}
\@namedef{S@s3.st.sr.contactq50.h13}{0.052}
\@namedef{S@s3.st.sr.contactq50.p}{0.009}
\@namedef{S@s3.st.sr.contactq50.pp}{$p=0.009$}
\@namedef{S@s3.st.sr.contactq75.ci}{\ensuremath{-}1.6 to +1.4}
\@namedef{S@s3.st.sr.contactq75.ci2}{\ensuremath{-}1.59 to +1.45}
\@namedef{S@s3.st.sr.contactq75.d}{\ensuremath{-}0.1}
\@namedef{S@s3.st.sr.contactq75.h13}{1.000}
\@namedef{S@s3.st.sr.contactq75.p}{0.877}
\@namedef{S@s3.st.sr.contactq75.pp}{$p=0.877$}
\@namedef{S@s3.st.sr.contactq90.ci}{+0.9 to +3.5}
\@namedef{S@s3.st.sr.contactq90.ci2}{+0.86 to +3.50}
\@namedef{S@s3.st.sr.contactq90.d}{+2.1}
\@namedef{S@s3.st.sr.contactq90.h13}{0.011}
\@namedef{S@s3.st.sr.contactq90.p}{0.001}
\@namedef{S@s3.st.sr.contactq90.pp}{$p=0.001$}
\@namedef{S@s3.st.sr.disagreementq25.ci}{+1.2 to +4.3}
\@namedef{S@s3.st.sr.disagreementq25.ci2}{+1.19 to +4.33}
\@namedef{S@s3.st.sr.disagreementq25.d}{+2.7}
\@namedef{S@s3.st.sr.disagreementq25.h13}{0.007}
\@namedef{S@s3.st.sr.disagreementq25.p}{<0.001}
\@namedef{S@s3.st.sr.disagreementq25.pp}{$p<0.001$}
\@namedef{S@s3.st.sr.disagreementq50.ci}{+0.9 to +3.5}
\@namedef{S@s3.st.sr.disagreementq50.ci2}{+0.89 to +3.49}
\@namedef{S@s3.st.sr.disagreementq50.d}{+2.1}
\@namedef{S@s3.st.sr.disagreementq50.h13}{0.007}
\@namedef{S@s3.st.sr.disagreementq50.p}{<0.001}
\@namedef{S@s3.st.sr.disagreementq50.pp}{$p<0.001$}
\@namedef{S@s3.st.sr.disagreementq75.ci}{+0.1 to +2.9}
\@namedef{S@s3.st.sr.disagreementq75.ci2}{+0.10 to +2.90}
\@namedef{S@s3.st.sr.disagreementq75.d}{+1.5}
\@namedef{S@s3.st.sr.disagreementq75.h13}{0.168}
\@namedef{S@s3.st.sr.disagreementq75.p}{0.034}
\@namedef{S@s3.st.sr.disagreementq75.pp}{$p=0.034$}
\@namedef{S@s3.st.sr.disagreementq90.ci}{\ensuremath{-}0.4 to +1.5}
\@namedef{S@s3.st.sr.disagreementq90.ci2}{\ensuremath{-}0.39 to +1.53}
\@namedef{S@s3.st.sr.disagreementq90.d}{+0.6}
\@namedef{S@s3.st.sr.disagreementq90.h13}{0.914}
\@namedef{S@s3.st.sr.disagreementq90.p}{0.229}
\@namedef{S@s3.st.sr.disagreementq90.pp}{$p=0.229$}
\@namedef{S@s3.st.sr.dmax}{+5.4}
\@namedef{S@s3.st.sr.dmin}{\ensuremath{-}0.1}
\@namedef{S@s3.st.sr.errorq25.ci}{+1.6 to +5.1}
\@namedef{S@s3.st.sr.errorq25.ci2}{+1.59 to +5.13}
\@namedef{S@s3.st.sr.errorq25.d}{+3.3}
\@namedef{S@s3.st.sr.errorq25.h13}{0.002}
\@namedef{S@s3.st.sr.errorq25.p}{<0.001}
\@namedef{S@s3.st.sr.errorq25.pp}{$p<0.001$}
\@namedef{S@s3.st.sr.errorq50.ci}{+3.1 to +6.8}
\@namedef{S@s3.st.sr.errorq50.ci2}{+3.11 to +6.82}
\@namedef{S@s3.st.sr.errorq50.d}{+4.9}
\@namedef{S@s3.st.sr.errorq50.h13}{0.001}
\@namedef{S@s3.st.sr.errorq50.p}{<0.001}
\@namedef{S@s3.st.sr.errorq50.pp}{$p<0.001$}
\@namedef{S@s3.st.sr.errorq75.ci}{+1.3 to +4.8}
\@namedef{S@s3.st.sr.errorq75.ci2}{+1.31 to +4.80}
\@namedef{S@s3.st.sr.errorq75.d}{+3.0}
\@namedef{S@s3.st.sr.errorq75.h13}{0.011}
\@namedef{S@s3.st.sr.errorq75.p}{0.001}
\@namedef{S@s3.st.sr.errorq75.pp}{$p=0.001$}
\@namedef{S@s3.st.sr.errorq90.ci}{\ensuremath{-}0.6 to +1.1}
\@namedef{S@s3.st.sr.errorq90.ci2}{\ensuremath{-}0.55 to +1.15}
\@namedef{S@s3.st.sr.errorq90.d}{+0.3}
\@namedef{S@s3.st.sr.errorq90.h13}{1.000}
\@namedef{S@s3.st.sr.errorq90.p}{0.476}
\@namedef{S@s3.st.sr.errorq90.pp}{$p=0.476$}
\@namedef{S@s3.st.sr.geom.ci}{+2.3 to +8.7}
\@namedef{S@s3.st.sr.geom.ci2}{+2.25 to +8.67}
\@namedef{S@s3.st.sr.geom.d}{+5.4}
\@namedef{S@s3.st.sr.geom.h13}{0.007}
\@namedef{S@s3.st.sr.geom.p}{<0.001}
\@namedef{S@s3.st.sr.geom.pp}{$p<0.001$}
\@namedef{S@s3.st.sr.hi}{+8.7}
\@namedef{S@s3.st.sr.lo}{\ensuremath{-}1.6}
\@namedef{S@s3.st.sr.ndpos}{12}
\@namedef{S@s3.st.sr.nholm}{7}
\@namedef{S@s3.st.sr.nneg}{0}
\@namedef{S@s3.st.sr.npos}{9}
\@namedef{S@s3.st.sr.prim.dmax}{+5.4}
\@namedef{S@s3.st.sr.prim.dmin}{\ensuremath{-}0.1}
\@namedef{S@s3.st.sr.prim.hi}{+8.7}
\@namedef{S@s3.st.sr.prim.lo}{\ensuremath{-}1.6}
\@namedef{S@s3.st.sr.prim.npos}{3}
\@namedef{S@s3.st.sr.prim.nsig}{3}
\@namedef{S@s3.st.srcov.contactq25.ci}{\ensuremath{-}0.001 to +0.004}
\@namedef{S@s3.st.srcov.contactq25.ci2}{\ensuremath{-}0.0007 to +0.0040}
\@namedef{S@s3.st.srcov.contactq25.d}{+0.002}
\@namedef{S@s3.st.srcov.contactq25.h13}{0.366}
\@namedef{S@s3.st.srcov.contactq25.p}{0.183}
\@namedef{S@s3.st.srcov.contactq25.pp}{$p=0.183$}
\@namedef{S@s3.st.srcov.contactq50.ci}{+0.002 to +0.009}
\@namedef{S@s3.st.srcov.contactq50.ci2}{+0.0016 to +0.0092}
\@namedef{S@s3.st.srcov.contactq50.d}{+0.005}
\@namedef{S@s3.st.srcov.contactq50.h13}{0.026}
\@namedef{S@s3.st.srcov.contactq50.p}{0.004}
\@namedef{S@s3.st.srcov.contactq50.pp}{$p=0.004$}
\@namedef{S@s3.st.srcov.contactq75.ci}{\ensuremath{-}0.006 to +0.001}
\@namedef{S@s3.st.srcov.contactq75.ci2}{\ensuremath{-}0.0057 to +0.0014}
\@namedef{S@s3.st.srcov.contactq75.d}{\ensuremath{-}0.002}
\@namedef{S@s3.st.srcov.contactq75.h13}{0.366}
\@namedef{S@s3.st.srcov.contactq75.p}{0.259}
\@namedef{S@s3.st.srcov.contactq75.pp}{$p=0.259$}
\@namedef{S@s3.st.srcov.contactq90.ci}{+0.002 to +0.007}
\@namedef{S@s3.st.srcov.contactq90.ci2}{+0.0021 to +0.0065}
\@namedef{S@s3.st.srcov.contactq90.d}{+0.004}
\@namedef{S@s3.st.srcov.contactq90.h13}{0.001}
\@namedef{S@s3.st.srcov.contactq90.p}{<0.001}
\@namedef{S@s3.st.srcov.contactq90.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.disagreementq25.ci}{+0.004 to +0.009}
\@namedef{S@s3.st.srcov.disagreementq25.ci2}{+0.0035 to +0.0092}
\@namedef{S@s3.st.srcov.disagreementq25.d}{+0.006}
\@namedef{S@s3.st.srcov.disagreementq25.h13}{0.001}
\@namedef{S@s3.st.srcov.disagreementq25.p}{<0.001}
\@namedef{S@s3.st.srcov.disagreementq25.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.disagreementq50.ci}{+0.003 to +0.009}
\@namedef{S@s3.st.srcov.disagreementq50.ci2}{+0.0025 to +0.0093}
\@namedef{S@s3.st.srcov.disagreementq50.d}{+0.006}
\@namedef{S@s3.st.srcov.disagreementq50.h13}{0.001}
\@namedef{S@s3.st.srcov.disagreementq50.p}{<0.001}
\@namedef{S@s3.st.srcov.disagreementq50.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.disagreementq75.ci}{+0.001 to +0.008}
\@namedef{S@s3.st.srcov.disagreementq75.ci2}{+0.0010 to +0.0076}
\@namedef{S@s3.st.srcov.disagreementq75.d}{+0.004}
\@namedef{S@s3.st.srcov.disagreementq75.h13}{0.037}
\@namedef{S@s3.st.srcov.disagreementq75.p}{0.007}
\@namedef{S@s3.st.srcov.disagreementq75.pp}{$p=0.007$}
\@namedef{S@s3.st.srcov.disagreementq90.ci}{+0.0004 to +0.004}
\@namedef{S@s3.st.srcov.disagreementq90.ci2}{+0.0004 to +0.0039}
\@namedef{S@s3.st.srcov.disagreementq90.d}{+0.002}
\@namedef{S@s3.st.srcov.disagreementq90.h13}{0.055}
\@namedef{S@s3.st.srcov.disagreementq90.p}{0.018}
\@namedef{S@s3.st.srcov.disagreementq90.pp}{$p=0.018$}
\@namedef{S@s3.st.srcov.dmax}{+0.017}
\@namedef{S@s3.st.srcov.dmin}{\ensuremath{-}0.002}
\@namedef{S@s3.st.srcov.errorq25.ci}{+0.004 to +0.011}
\@namedef{S@s3.st.srcov.errorq25.ci2}{+0.0041 to +0.0107}
\@namedef{S@s3.st.srcov.errorq25.d}{+0.007}
\@namedef{S@s3.st.srcov.errorq25.h13}{0.001}
\@namedef{S@s3.st.srcov.errorq25.p}{<0.001}
\@namedef{S@s3.st.srcov.errorq25.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.errorq50.ci}{+0.009 to +0.016}
\@namedef{S@s3.st.srcov.errorq50.ci2}{+0.0086 to +0.0164}
\@namedef{S@s3.st.srcov.errorq50.d}{+0.012}
\@namedef{S@s3.st.srcov.errorq50.h13}{0.001}
\@namedef{S@s3.st.srcov.errorq50.p}{<0.001}
\@namedef{S@s3.st.srcov.errorq50.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.errorq75.ci}{+0.005 to +0.012}
\@namedef{S@s3.st.srcov.errorq75.ci2}{+0.0054 to +0.0125}
\@namedef{S@s3.st.srcov.errorq75.d}{+0.009}
\@namedef{S@s3.st.srcov.errorq75.h13}{0.001}
\@namedef{S@s3.st.srcov.errorq75.p}{<0.001}
\@namedef{S@s3.st.srcov.errorq75.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.errorq90.ci}{+0.001 to +0.004}
\@namedef{S@s3.st.srcov.errorq90.ci2}{+0.0005 to +0.0042}
\@namedef{S@s3.st.srcov.errorq90.d}{+0.002}
\@namedef{S@s3.st.srcov.errorq90.h13}{0.042}
\@namedef{S@s3.st.srcov.errorq90.p}{0.011}
\@namedef{S@s3.st.srcov.errorq90.pp}{$p=0.011$}
\@namedef{S@s3.st.srcov.geom.ci}{+0.010 to +0.024}
\@namedef{S@s3.st.srcov.geom.ci2}{+0.0103 to +0.0239}
\@namedef{S@s3.st.srcov.geom.d}{+0.017}
\@namedef{S@s3.st.srcov.geom.h13}{0.001}
\@namedef{S@s3.st.srcov.geom.p}{<0.001}
\@namedef{S@s3.st.srcov.geom.pp}{$p<0.001$}
\@namedef{S@s3.st.srcov.hi}{+0.024}
\@namedef{S@s3.st.srcov.lo}{\ensuremath{-}0.006}
\@namedef{S@s3.st.srcov.ndpos}{12}
\@namedef{S@s3.st.srcov.nholm}{10}
\@namedef{S@s3.st.srcov.nneg}{0}
\@namedef{S@s3.st.srcov.npos}{11}
\@namedef{S@s3.st.srcov.prim.dmax}{+0.017}
\@namedef{S@s3.st.srcov.prim.dmin}{\ensuremath{-}0.002}
\@namedef{S@s3.st.srcov.prim.hi}{+0.024}
\@namedef{S@s3.st.srcov.prim.lo}{\ensuremath{-}0.006}
\@namedef{S@s3.st.srcov.prim.npos}{3}
\@namedef{S@s3.st.srcov.prim.nsig}{3}
\makeatother

